CStream: Parallel Data Stream Compression on Multicore Edge Devices

In the burgeoning realm of Internet of Things (IoT) applications on edge devices, data stream compression has become increasingly pertinent. The integration of added compression overhead and limited hardware resources on these devices calls for a nuanced software-hardware co-design. This paper introduces CStream, a pioneering framework crafted for parallelizing stream compression on multicore edge devices. CStream grapples with the distinct challenges of delivering a high compression ratio, high throughput, low latency, and low energy consumption. Notably, CStream distinguishes itself by accommodating an array of stream compression algorithms, a variety of hardware architectures and configurations, and an innovative set of parallelization strategies, some of which are proposed herein for the first time. Our evaluation showcases the efficacy of a thoughtful co-design involving a lossy compression algorithm, asymmetric multicore processors, and our novel, hardware-conscious parallelization strategies. This approach achieves a 2.8x compression ratio with only marginal information loss, 4.3x throughput, 65% latency reduction and 89% energy consumption reduction, compared to designs lacking such strategic integration.

==> Sections/Authors.tex <==
%%
%% The "author" command and its associated commands are used to define the authors and their affiliations. 

%% This is an example of author command

%\author{Lars Th{\o}rv{\"a}ld}
%\orcid{0000-0002-1825-0097}
%\affiliation{%
  %\institution{The Th{\o}rv{\"a}ld Group}
  %\city{Hekla}
 % \country{Iceland}
%}
%\email{larst@affiliation.org}


%%
%% The "author" command and its associated commands are used to define the authors and their affiliations.

\author{Xianzhi Zeng}
\affiliation{%
  \institution{Singapore University of Technology and Design}
  \streetaddress{ 8 Somapah Rd, Singapore}
  %\city{Singapore}
  \state{Singapore}
  \postcode{487372}
}
\email{xianzhi_zeng@sutd.edu.sg}
\author{Shuhao Zhang}
\affiliation{%
  \institution{Singapore University of Technology and Design}
  \streetaddress{ 8 Somapah Rd, Singapore}
 % \city{Singapore}
  \state{Singapore}
  \postcode{487372}
}
\email{shuhao_zhang@sutd.edu.sg}

% \author{Valerie B\'eranger}
% \orcid{0000-0001-5109-3700}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }
% \email{vb@rocquencourt.com}


==> Sections/Co-Design/Versatility.tex <==
\subsection{Scalability and Versatility}
\label{subsec:scalability_versatility}
\design's design is inherently scalable and versatile, with its broad range of compression algorithms, adaptive scheduling, and efficient resource management enabling it to handle diverse data types, workloads, and hardware configurations. 

One of the major strengths of \design lies in its ability to process different kinds of data. Whether it is structured or unstructured, numeric or textual, \design's diverse set of compression algorithms can adapt to the specific properties of the data. This adaptability extends to various IoT data types, making \design an ideal solution for a wide range of IoT applications at the edge.

Scalability is another hallmark of \design. Its design leverages the inherent parallelism in stream compression tasks, effectively utilizing the available hardware resources. This ability is further boosted by its asymmetric-aware scheduling and smart workload partitioning, allowing it to handle larger volumes of data by distributing the load across available cores. Moreover, \design scales with the hardware, seamlessly integrating additional cores or adjusting to different core configurations.

The versatile nature of \design also extends to its power adaptability. Recognizing the energy constraints prevalent in edge computing environments, \design's design places a strong emphasis on energy efficiency. Its energy metering component measures the power consumption of its operations in real-time, enabling dynamic adjustments and optimizations to keep power usage within acceptable bounds. Furthermore, its intelligent task scheduling considers both the computational needs and energy efficiency, striking a balanced allocation that maximizes throughput while minimizing power consumption.

In summary, the scalability and versatility of \design lie in its ability to adapt to the diverse and dynamic nature of edge computing environments, demonstrating its potential as an effective and efficient solution for stream compression in IoT applications.


==> Sections/backup/0_Abstract.tex <==
\begin{abstract}
Modern stream applications are increasingly deployed near the data source on edge devices, which are now commonly equipped with \emph{asymmetric multicore processors (AMPs)} balancing compute power and energy efficiency. 
Meanwhile, the \emph{streaming lossless compression (\compress)} has became a key operation widely used in stream applications, but prior work primarily targets improving its efficiency on a single core or symmetric multicores.
% Specifically, we adapt CPU-assisted prefetching to minimize
% cache misses in GPU query co-processing and CPU-assisted
% decompression to improve query execution performance. Furthermore, we develop a cost model guided adaptation mechanism for distributing the workload of prefetching, decompression, and query execution between CPU and GPU. We implement a system prototype and evaluate it on two recent
% AMD APUs A8 and A10. The experimental results show
% that 1) in-cache query co-processing can effectively improve
% the performance of the state-of-the-art GPU co-processing
% paradigm by up to 30% and 33% on A8 and A10, respectively, and 2) our workload distribution adaption mechanism
% can significantly improve the query performance by up to
% 36% and 40% on A8 and A10, respectively.
In this paper, we propose a novel parallelization framework namely \design for parallelizing \compress algorithms on AMPs. 
% This paper introduces \design, a new data stream compression algorithm
Specifically, \design holistically exploits both task pipeline and data partitioning schemes during compression, which results in a list of fine-grained execution tasks. 
Furthermore, we develop a cost model to guide the scheduling of those tasks among asymmetric multicores to satisfy processing latency constraints with minimum energy consumption considering both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores}.
To validate our proposal, we implement a system prototype with five alternative approaches. 
%  several anti-interference co-design, us 
Our extensive experimental study of parallelizing three popular \compress algorithms 
with three real-world datasets show that (1) \design outperforms alternative approaches by up to 53\%; and (2) our cost-model can successfully guide \design to minimize energy consumption while sustaining different latency constraints.
% Query co-processing on graphics processors (GPUs) has become an effective means to improve the performance of main
% memory databases. However, the relatively low bandwidth
% and high latency of the PCI-e bus are usually bottleneck
% issues for co-processing. Recently, coupled CPU-GPU architectures have received a lot of attention, e.g. AMD APUs
% with the CPU and the GPU integrated into a single chip.
% That opens up new opportunities for optimizing query coprocessing. 
\begin{comment}
Modern stream applications are increasingly popular near the data source on edge devices, and they are now commonly equipped with \emph{asymmetric multicore processors (AMPs)} balancing compute power and energy efficiency. 
Meanwhile, the \emph{streaming lossless compression (\compress)} has became a key operation widely used in stream applications.
However,
prior works primarily focus on improving its efficiency on a single core or symmetric multicores,
while ignoring \compress on AMPs.
%
%Modern stream applications are increasingly deployed near the data source on edge devices, which are now commonly equipped with \emph{asymmetric multicore processors (AMPs)} balancing compute power and energy efficiency. 
%Meanwhile, the \emph{streaming lossless compression (\compress)} has became a key operation widely used in stream applications, but prior work primarily targets improving its efficiency on a single core or symmetric multicores.
% Specifically, we adapt CPU-assisted prefetching to minimize
% cache misses in GPU query co-processing and CPU-assisted
% decompression to improve query execution performance. Furthermore, we develop a cost model guided adaptation mechanism for distributing the workload of prefetching, decompression, and query execution between CPU and GPU. We implement a system prototype and evaluate it on two recent
% AMD APUs A8 and A10. The experimental results show
% that 1) in-cache query co-processing can effectively improve
% the performance of the state-of-the-art GPU co-processing
% paradigm by up to 30% and 33% on A8 and A10, respectively, and 2) our workload distribution adaption mechanism
% can significantly improve the query performance by up to
% 36% and 40% on A8 and A10, respectively.

In this paper, we develop a novel energy-efficient framework, called \design, to parallelize \compress on AMPs.
%\xianzhi{in an energy efficient manner}.
%Specifically, 
First,
\design holistically exploits both task pipeline and data partitioning schemes during compression, which results in a list of fine-grained execution tasks. 
%Furthermore,
Second,
we develop a cost model called \model to guide the scheduling of those tasks among asymmetric multicores.
With our model, \design can satisfy processing latency constraints with minimum energy consumption considering both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores}.
%To validate our proposal, we implement the system prototype with five alternative approaches. 
Third,
For the smooth execution of \compress, we  develop an executor with anti-interference co-design in the \design  prototype.

%\xianzhi{For the smooth running of \compress, we also develop an executor with anti-interference co-design in the \design system prototype.}


\iffalse
In this paper, we propose a novel parallelization framework namely \design for parallelizing \compress algorithms on AMPs. 
% This paper introduces \design, a new data stream compression algorithm
Specifically, \design holistically exploits both task pipeline and data partitioning schemes during compression, which results in a list of fine-grained execution tasks. 
Furthermore, we develop a cost model to guide the scheduling of those tasks among asymmetric multicores to satisfy processing latency constraints with minimum energy consumption considering both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores}.
To validate our proposal, we implement a system prototype with five alternative approaches. 
%  several anti-interference co-design, us 
\fi


We use three popular \compress algorithms 
with three real-world diverse datasets to validate its performance and compare \design with five alternative approaches.
Experiments show that 1) \design outperforms the state-of-the-art approaches by up to 53\%, and 2) our cost-model can successfully guide \design to minimize energy consumption while sustaining different latency constraints.


\iffalse
Our extensive experimental study of parallelizing three popular \compress algorithms 
with three real-world datasets show that (1) \design outperforms alternative approaches by up to 53\%; and (2) our cost-model can successfully guide \design to minimize energy consumption while sustaining different latency constraints.
\fi


% and evaluate it on a recent AMPs xxx. 
% and then schedules those tasks based on a novel cost model  with a goal of minimizing 
% latency while sustaining a given energy budget. 
% energy consumption while sustaining a given compressing latency requirement.
% The key contribution of \design is an affinity
% varying core affinities and  asymmetriccore communication cost
% Based on a novel cost model, \design schedules those tasks on asymmetric multicore processors 
% For evaluation, we implement three stream-based compression algorithms in \system.


% In this paper, we experimentally revisit hash
% joins, one of the most important join algorithms for main
% memory databases, on a coupled CPU-GPU architecture.
% Particularly, we study the fine-grained co-processing mechanisms on hash joins with and without partitioning. The
% co-processing outlines an interesting design space. We extend existing cost models to automatically guide decisions
% on the design space. Our experimental results on a recent
% AMD APU show that (1) the coupled architecture enables
% fine-grained co-processing and cache reuses, which are inefficient on discrete CPU-GPU architectures; (2) the cost model can automatically guide the design and tuning knobs in
% the design space; (3) fine-grained co-processing achieves up
% to 53%, 35% and 28% performance improvement over CPUonly, GPU-only and conventional CPU-GPU co-processing,
% respectively. We believe that the insights and implications
% from this study are initial yet important for further research
% on query co-processing on coupled CPU-GPU architectures.

% In this paper, we propose \system, a novel data stream compression framework
% % This paper introduces \design, a new data stream compression algorithm
% specifically designed for asymmetric multicore processors. 
% During compressing, \system holistically exploits both task pipeline and data partitioning schemes resulting in a list of fine-grained tasks and then schedules those tasks based on a novel cost model considering both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores} with a goal of minimizing 
% % latency while sustaining a given energy budget. 
% energy consumption while sustaining a given compressing latency requirement.
% % The key contribution of \design is an affinity
% % varying core affinities and  asymmetriccore communication cost
% % Based on a novel cost model, \design schedules those tasks on asymmetric multicore processors 
% For evaluation, we implement three stream-based compression algorithms in \system.
% Our extensive experimental study based on both real-world and synthetic dataset show that (1) \design outperforms alternative approaches by xxx; and (2) the cost model can successfully guide \design to select the optimal scheduling plan.

% A key contribution of \design is a novel AMP-aware cost-model that guides the scheduling of fine-grained tasks of DSC on AMPs with a goal of minimizing the energy consumption while sustaining a given latency requirement.

 % Particularly, we study the fine-grained co-processing mechanisms on hash joins with and without partitioning. The
% co-processing outlines an interesting design space. We extend existing cost models to automatically guide decisions
% on the design space. Our experimental results on a recent
% AMD APU show that (1) the coupled architecture enables
% fine-grained co-processing and cache reuses, which are inefficient on discrete CPU-GPU architectures; (2) the cost model can automatically guide the design and tuning knobs in
% the design space; (3) fine-grained co-processing achieves up
% to 53%, 35% and 28% performance improvement over CPUonly, GPU-only and conventional CPU-GPU co-processing,
% respectively. We believe that the insights and implications
% from this study are initial yet important for further research
% on query co-processing on coupled CPU-GPU architectures.


% we introduce a novel stream-based data compression algorithm called \design optimized for the asymmetric multicore architecture.

% To achieve the goal, we propose the {\design} scheduling strategy. {\design} uses the AMP-adapted \emph{roof line model} and compression-specific algorithm analysis to address core affinity, and has the \emph{slope mode} to deal with asymmetric core communication cost. Therefore, it can select the optimal scheduling plan by precise estimation. Besides, {\design} use the dynamic programming to simplify the searching and enumeration of plans. 
% %
% We implemented {\design} on customized embedded system {\system}, and
% our extensive experiment on concrete AMP device confirms the superiority of {\design}.



% Due to the increasing volume of data streams, 
% The asymmetric multicore architecture increasingly adopted by edge devices makes it compelling to process data streams near the cloud edge to reduce data transmission overhead. 
% However, such an approach is constrained by compute power, memory limits and energy budget. 
% In such a setting, the \emph{stream-based data compression}, that compresses continuous data streams is attractive to be applied to further reduce data footprints as edge devices are often constrained by

% The \emph{stream-based data compression}, that compresses continuous data streams, receives much attention
% is a widely studied technique to reduce data footprints of modern data intensive applications. 
% However, compression does not necessarily lead to performance improvement, especially when applications are deployed 

% Many previous works have attempted at improving its performance by adopting parallel multicore 
\end{comment}
\begin{comment}
%The appealing properties of NVM including high performance,
%persistence, and byte-addressability, and a recent active
%thread of building remote memory systems with RDMA,
%have produced considerable interest in combining them for
%fast and persistent remote memory systems.
The appealing properties of \emph{asymmetric multicore processors (AMPs)} including
% satisfying compute power and 
high performance and energy efficiency, 
and a recent popularity of the \emph{streaming lossless compression (\compress)}, 
have produced considerable interest and benefits in combining them for
more efficient stream processing at the network edge. 
% at the edge of Internet of Things (IoT).
%The \emph{asymmetric multicore processors (AMPs)} which balance compute power and energy efficiency is gaining increasing popularity in edge computing, which is a thriving new field for modern stream applications. Meanwhile, the \emph{streaming lossless compression (\compress)} has became a key operation widely used in stream applications. 
However,
prior works primarily focus on improving its efficiency on a single core or symmetric multicores,
while ignoring \compress on AMPs.
In this paper, we develop a novel energy-efficient parallelization framework, called \design, to parallelize \compress on AMPs.
%
First, \design involves library and algorithms for a fine-grained and hybrid parallelization of \compress .
%
Second, \design integrates a cost model called \model to guide the scheduling of parallel \compress tasks, which considers both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores}.
%
Third, \design maintains an executor with anti-interference co-design 
for the smooth execution of \compress.
%

We implement \design and five alternative approaches on real AMP.
Experiments involving diverse data sets show that 1) \design outperforms the state-of-the-art approaches by up to 53\%, and 2) the \model can successfully guide \design to minimize energy consumption while sustaining different latency constraints. The superiority of \design can be confirmed further in simulation towards future AMP.
\end{comment}

\end{abstract}

==> Sections/backup/1_Introduction.tex <==
\section{Introduction}
\label{sec::introdction}
\begin{comment}
% Modern stream applications are increasingly deployed near the data source on edge devices.
% To balance compute power and energy efficiency, those edge devices are commonly equipped with \emph{asymmetric multicore processors (AMPs)}. 
\xianzhi{
With the development of 5G~\cite{fiveg_survey} and Internet of Things (IoT)~\cite{IoT_survey2019},
edge computing emerges as an attractive
manner to host computation tasks as close as
possible to the data sources and end users~\cite{edge_2020}.
%it has became more and more compelling to deploy various applications~\cite{sp_def} near the data source on edge devices~\cite{nebulastream}.
According to a 2018 survey~\cite{edge_survey}, modern ARM machines are typical choices for edge devices, which are often equipped with \emph{asymmetric multicore processors (AMPs)}~\cite{amp_iot}. The AMPs couple relatively batter-saving and slower cores~\cite{amp_A53ug} with relatively more powerful and power-hungry cores~\cite{amp_A72ug} under the same Instruction Set Architecture (ISA), and they can effectively balance computational power and energy consumption~\cite{amp_survey_2016}.

% Meanwhile, the \emph{streaming lossless compression (\compress)} has became a key operation widely used in stream applications. However, none exploits AMP to its full potential due to the unawareness of its asymmetry in terms of both core and communication.
Meanwhile, the data compression has been widely adopted in edge computing applications~\cite{comp_edge_energy}, as it can significantly reduce the data redundancy and help addressing the storage limitations of edge devices. 
Moreover, the stringent response time requirements and energy constrains 
%in edge computing 
have created significant interest in accelerating compression~\cite{comp_acc} and reducing its energy dissipation~\cite{comp_energy_2006}. It is therefore natural and profitable to parallelize and optimize data compression on AMPs for edge computing.
}
\end{comment}


\begin{comment}
Unfortunately, literature gap makes effective data compression on AMPs still unachieved. In particular,
% none of existing work can achieve energy efficient parallelization of \compress on AMP.
existing work on compression emphasize on improving the theoretical compressibility~\cite{comp_7z}, 
reducing compressing complexity on single core~\cite{comp_survey_2017,comp_survey_huffman}, 
parallel compressing performance on symmetric multicores~\cite{comp_ndzip,comp_para_bzip2}, 
or heterogeneous hardware devices like GPU~\cite{comp_pipeline_gpu,comp_cuda_compare} or FPGA~\cite{comp_lz4_fpga}.
Due to their unawareness of AMPs' asymmetry in terms of core~\cite{amp_2003,amp_2004} and communication~\cite{amp_partition_2019}, their approaches incur both higher latency and more energy dissipation as shown in our experiments.
Therefore, we need a new solution for parallelizing data compression on AMPs, which shall
give answers to three key challenging questions as follows.
\begin{myitemize}
    \item [C1] \textbf{Which compression algorithm to be applied?} Many compression algorithms are applicable with diverse trade-offs (e.g., speed and compression ratio~\cite{comp_exp_review}), and the specific use case can further influence the algorithm choice.
    %For instance, the critical data like id in stream processing~\cite{comp_tersecades} or VM statuts in computation offloading~\cite{comp_mobile_vm} prefers lossless and fast-complete algorithms much more than massive sensor data~\cite{comp_wsn}. 
    \item [C2] \textbf{How to parallelize compression algorithms on AMPs?} Unlike conventional symmetric multicore processors (SMPs), AMPs contain cores under different micro-architecture (e.g., Out-of-Order and In-Order), which have varying affinity to even the same data compression. Therefore, a proper parallelization of compression should consider all micro-architectures involved.
    \item [C3] \textbf{How to schedule parallel compression tasks on AMPs?} Multiple task will be created after the parallelization of compression, and they should be finally scheduled to AMP cores. The scheduling is not only among asymmetric cores, but also faced with the asymmetric communication. Specifically, communication costs vary depending on 1) the relative location of mapped cores and 2) the direction of communication. This is even more complicated than NUMA architecture, which involves the so-called 'NUMA-distance'~\cite{sp_briskstream} but is not direction-related. 
\end{myitemize}
\end{comment}


\begin{comment}
% Figure 1 shows the evaluation of xxx on AMP. It shows that 
% To the best of our knowledge, little work has studied how to best parallelize \compress on AMPs.
%Meanwhile, existing works of improving scheduling on AMPs are typically in OS level~\cite{amp_DVFS2,amp_scheduling_2018,amp_scheduling_2021} (i.e., viewing the all work load as equal black-box). 
% In this paper, we propose a novel parallelization framework namely \design for parallelizing \compress algorithms on AMPs. \design is primarily based on the holistic exploration of both task pipeline and data partitioning parallelism during compression. 
In this paper, we propose the \design (Parallel Compression on Asymmetric Multicore Processors) framework to parallelize \compress algorithms on AMPs. 
To address C1, \design consists an extensible algorithm library to enable the suitable selection of compression algorithm on demand.
%and it integrates a tailored run time as well as energy measurement functions for efficient execution on AMP. 
To address C2, \design decomposes compression algorithms into multiple fine-grained tasks, and each of them can be independently scheduled based on its core-preference. To address C3, \design is guided by a novel asymmetric-aware cost model considering both asymmetric cores and asymmetric communication to determine the optimal scheduling plan.
\end{comment}
 
\begin{comment}
The process of compressing a batch or tuple is called a \emph{compression job}.
For handling each compression job, \design explores two common parallelizing approaches. 
1) \emph{Task pipelining:} 
     a job can be decomposed into a list of execution \emph{stages}. 
     Each stage can run independently by exchanging intermediate results via message passing.
2) \emph{Data parallelism:} 
     each \emph{stage} may be further replicated into multiple \emph{replicas} handling subsets of input data concurrently.
% which results in a list of fine-grained execution tasks.
In this way, the parallelization of each compression job results in a list of \emph{execution tasks}, i.e., replicas of stages.
% This allows it to extract fine-grained execution tasks with varying task-core affinity to better utilize AMPs.
This allows us to schedule execution tasks to their suitable cores in a more fine-grained manner compared to existing works mostly only exploit data parallelism~\cite{comp_para_bzip2}.

% The scheduling of the resulting execution tasks on AMPs is still non-trivial. 
An \emph{scheduling plan} determines the number of replicas of each stage, as well as the way of allocating each replica to
the underlying cores. 
Identifying an optimal plan on AMPs is still non-trivial due to two key challenges. 
Challenge 1: 
each task may favor~\cite{amp_scheduling_2021} different types of cores on AMPs, due to their involved different Instruction Level Parallelism (ILP) and Memory Level Parallelism (MLP). 
% in energy consumption and execution latency.
Challenge 2: 
there is a asymmetric core communication pattern among tasks scheduled to different cores on AMPs. 
This is even more complicated than NUMA-architecture~\cite{sp_briskstream}, which has varying communication costs due to distance but no asymmetry.
% 
% there is a varying and polar penalty for core communication on AMP.

% We develop a cost model to guide the proper scheduling by taking both \emph{asymmetric cores} and \emph{asymmetric communication cost} into consideration.
We develop a cost model to guide \design to search for the optimal scheduling plan.
Inspired by the boat-hull adoption~\cite{roofline_boat}, we predict the performance and energy of how a given software runs on AMP by roofline model. 
To address the first challenge, we harnesses the ILP and MLP of each task through roof line   xxx
To address the second challenge, the relative location (i.e., AMP-distance with asymmetric core communication) of consecutive \emph{stages} into consideration. xxx
In this way, it is able to determine the correlation between a solution and its
objective value, i.e., to predict the \textbf{E}nergy consumption and \textbf{L}atency of each compression job. 
\end{comment}

% Modern stream applications are increasingly deployed near the
% data source on edge devices, which are now commonly equipped
% with asymmetric multicore processors (AMPs) balancing compute
% power and energy efficiency.
%Optimizing the performance of stream processing systems
%hot research topic due to the rigid requirement
%on the event processing latency and throughput
%has been a hot research topic due to the rigid requirement
%on the event processing latency and throughput.
\iffalse

Utilizing new hardware to optimize stream operations has been a hot research topic because of the rigid requirement and trade-off between performance and energy consumption.
With the development of 5G and Internet of Things (IoT)~\cite{IoT_survey2019}, it has became more and more compelling to deploy modern stream applications~\cite{sp_def} near the data source on edge devices.
In this way, we can minimize data transmission overhead to cope with the fast increasing volumes of data streams~\cite{nebulastream}.
In the edge scenarios,
we usually adopt modern ARM devices~\cite{edge_survey}.
These devices are often equipped with \emph{asymmetric multicore processors (AMPs)},
 coupling relatively batter-saving and slower cores~\cite{amp_A53ug} with relatively more powerful and power-hungry cores~\cite{amp_A72ug}.
 These cores share the same Instruction Set Architecture (ISA), aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.
Meanwhile, \emph{streaming lossless compression (\compress)} has been widely adopted in modern stream applications~\cite{comp_tersecades},
which can reduce computational workloads and memory footprints without affecting the accuracy of results. 
Different from traditional batch-based compression algorithms, \compress needs to compress data as soon as they arrive. 
Accordingly, the time-consuming data compression and stringent response time requirements pose urgent need
in accelerating \compress.
\begin{comment}
Moreover, the limited energy budget on stream processing devices under edge or mobile computing makes reducing the energy dissipation of \compress another major concern. 
\end{comment}



\xianzhi{Optimizing stream operations by utilizing new hardware has been a hot research topic due to the rigid requirement and trad-off between performance and energy consumption.}
Due to the raise of 5G and Internet of Things (IoT)~\cite{IoT_survey2019}, it has became more and more compelling to deploy modern stream applications~\cite{sp_def} near the data source on edge devices minimizing data transmission overhead to cope with the fast increasing volume of data streams~\cite{nebulastream}.
According to a 2018 survey~\cite{edge_survey}, modern ARM machines are typical choices for edge devices, which are often equipped with \emph{asymmetric multicore processors (AMPs)} coupling relatively batter-saving and slower cores~\cite{amp_A53ug} with relatively more powerful and power-hungry cores~\cite{amp_A72ug} sharing the same Instruction Set Architecture (ISA), aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.
Meanwhile, the \emph{streaming lossless compression (\compress)} has been widely adopted in modern stream applications~\cite{comp_tersecades} to reduce computational workloads and memory footprints without affecting the accuracy of results. 
Different from traditional batch-based compression algorithms, \compress needs to compress data as soon as they arrive. 
The costly nature of data compressing and the stringent response time requirements have created significant interest in accelerating \compress and \xianzhi{reducing its energy dissipation.}

\fi



Utilizing new hardware to optimize stream operations has been a hot research topic because of the rigid requirement and trade-off between performance and energy consumption. 
%On the one hand, it has became more and more compelling to deploy modern stream applications~\cite{sp_def} near the data source on edge devices~\cite{nebulastream} with the raise of 5G and Internet of Things (IoT)~\cite{IoT_survey2019}, and the \emph{asymmetric multicore processors (AMPs)} coupling both high performance cores~\cite{amp_A72ug} and high energy efficiency cores~\cite{amp_A53ug} are typical choices~\cite{amp_survey_2016} for these edge devices.
On the one hand, the \emph{asymmetric multicore processors (AMPs)} coupling both high performance cores~\cite{amp_A72ug} and high energy efficiency cores~\cite{amp_A53ug} are typical choices~\cite{amp_survey_2016} for edge computing devices~\cite{edge_survey}, which are the new compelling places to deploy modern stream applications~\cite{sp_def} near the data source~\cite{nebulastream}.
On the other hand, the \emph{streaming lossless compression (\compress)} has been widely adopted in modern stream applications~\cite{comp_tersecades}. It is therefore natural to consider implement and optimize \compress on AMP for stream processing at the edge.

This paper aims to parallelize  \compress under an energy efficient constraint on AMP. Specifically, we focus on minimizing the
energy consumption of parallel \compress while still meeting the cut-off constraint of latency and avoiding core overload. 
%benefits
By achieving the energy-efficient parallelization of \compress on AMP, stream analytics on
 edge devices  benefits from the following three aspects:
First, parallelization with AMP can meet the stringent response time requirements of \compress, against its costly nature of compressing data as soon as they arrive. 
Second,
%Next, 
deploying \compress to AMP-based stream processing systems can significantly reduce computational workloads and memory footprints without affecting the accuracy of results. 
Third,
most importantly, by synthetically utilizing the asymmetry of AMP, we can achieve lower power consumption levels and satisfying high performance simultaneously in \compress.

\begin{comment}
For the parallelization, 
 we explore two common approaches including 
1) task pipelining, where the compressing process can be decomposed into a list of execution \emph{stages}, which can run independently by exchanging intermediate results via message passing;
and 2) to further increase parallelism, each step may be replicated into multiple \emph{replicas} running in parallel threads handling subsets of input data concurrently.
Subsequently, we schedule the resulting lists of fine-grained execution tasks to AMPs to gain performance improvement and energy reduction.
\end{comment}
% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.

% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.

% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.

% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.


% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.


% a low-end processor~\cite{amp_A53ug} and a high-end processor~\cite{amp_A72ug} sharing the same instruction set, aiming to balance computational power and energy consumption~\cite{amp_survey_2016}.

%First introduce sp
% Stream processing (SP) is gaining popularity for continuous near real-time monitoring and analytics~\cite{sp_def}. For the consideration of higher capacity and lower latency, it is a new tendency to place SP at embedded edge devices instead of at the data center ~\cite{nebulastream} , as this kind of placement is closer to the data source. Typically, these embedded edge devices are faced with limited energy budget, and they should be implemented with energy-efficient new hardware with necessary computing power. The asymmetric multicore processors (AMPs) can just come to the aid, as they are intended to improve energy efficiency~\cite{amp_2003}, as well as guarantee or even improve the performance ~\cite{amp_2004}. Nowadays, top processor vendors like to apply the idea of AMP to build their flag-ship processors for edge and mobile computing (e.g. the rk3399(2016)~\cite{amp_rk3399} by Rockchip, the snapdragon-888(2020-2021)~\cite{amp_sd888} by Qualcomm and the kirin-9000(2020-2021)~\cite{amp_kirin9000} by Hisilicon) as AMPs have shown great success in fulfilling their original intention. 
%introduce AMP?
% Generally speaking, AMP means 1) identical instruction set architecture (ISA), 2) asymmetric cores (e.g., the In-Order A53~\cite{amp_A53ug} cores and Out-of-Order A72~\cite{amp_A72ug} cores)  with different performance and power and 3) asymmetric cache-memory structure to couple the asymmetric cores. Due to the wide application~\cite{amp_iot} and insightful design~\cite{amp_survey_2016}, it's natural and explicit to use AMP for stream applications at the edge on embedded systems.

% Meanwhile, the lossless data stream
% compression has became a key operation widely used in modern
% stream applications, but prior work primarily targets single core
% or symmetric multicores.
% Hence, many prior works focus on improving the compressing speed of \compress, but 

Unfortunately, none of existing work can achieve energy efficient parallelization of \compress on AMP.
Most of them are emphasized on improving the theoretical compressibility~\cite{comp_7z}, reducing compressing complexity on single core~\cite{comp_survey_2017,comp_survey_huffman},  parallel compressing performance on symmetric multicores~\cite{comp_ndzip,comp_para_bzip2}, or heterogeneous hardware devices~\cite{comp_cuda_compare,comp_lz4_fpga,comp_para_gpu}. 
To the best of our knowledge, little work has studied how to best parallelize \compress on AMPs, which gains many attention recently due to its increasingly deployment in IoT~\cite{amp_iot,nebulastream}. 
Meanwhile, existing works of improving scheduling on AMPs are typically in OS level~\cite{amp_DVFS2,amp_scheduling_2018,amp_scheduling_2021} (i.e., viewing the all work load as equal black-box). Thus, those literature gap motivates this work.

%\xianzhi{ 
Energy-efficiently parallelizing \compress on AMPs is non-trivial due to three key challenges. 
%\textbf{Challenge 1: }
First,
exposing and realizing the various Instruction Level Parallelism (ILP) and Memory Level Parallelism (MLP), while also considering Thread Level Parallelism (TLP), is important in both energy reduction and performance gain~\cite{amp_scheduling_2021,amp_impacts_2005}.
Howerver, there is no parallel-\compress-aware solution yet.
%First, to expose and realize the different Instruction Level Parallelism (ILP) and Memory Level Parallelism (MLP) while also consider the Thread Level Parallelism (TLP) is important in both energy reduction and performance gain~\cite{amp_scheduling_2021,amp_impacts_2005}, but there is no parallel-\compress-aware solution yet.
Second,
%\textbf{Challenge 2: }
different ILP and MLP leads to different task-core affinity in energy consumption and execution latency, and
another open question is how to synthetically estimate their impacts on different types of cores.
%Next, different ILP and MLP leads to different task-core affinity in energy consumption and execution latency, and how to synthetically estimate their impacts on different types of cores is another opening question.
%Finally, 
Third,
%\textbf{Challenge 3: }
there is a varying and polar penalty for core communication on AMP. In other words, the cost of communication varies with distance between cores and can be asymmetric between two cores. This is more complicated than NUMA-architecture~\cite{sp_briskstream}, which has varying communication costs due to distance but no asymmetry.
%the core communication on AMP has varying and polar penalty. In another word, the communication cost varies due to distance between cores and the cost may be asymmetric between two cores. This is even more complicated than NUMA-architecture~\cite{sp_briskstream}, which involves varying communication cost due to distance but there is no asymmetry.
%}
%\end{comment}

\begin{comment}
Next, the penalty of core communications between \emph{stages} \shuhao{cores?} is asymmetric, with both varying distance and polarity.\shuhao{, where the communication cost varies due to distance between cores and the cost may be asymmetric between two cores.} This is even more complicated than NUMA-architecture~\cite{sp_briskstream} which has socket-distance but is without polarity. 
\shuhao{ which involves varying communication cost due to distance but there is no asymmetry.}
\end{comment}


\begin{comment}
brisk stream:
Witnessing this problem, we present a novel NUMA-aware streaming execution plan optimization paradigm, called \emph{Relative-Location Aware Scheduling} (RLAS).
RLAS takes the relative location  (i.e., NUMA distance) of each pair of producer-consumer into consideration during optimization. 

tstream:
This paper presents TStream, a novel DSPS supporting
efficient concurrent state access in the context of main memory
multicore architectures. TStream follows previous work [7],
[9] of employing transactional semantics to handle concurrent
state access but achieves much better scalability. The design
of TStream is inspired by our careful analysis of existing
applications. Stream processing usually consists of a set
of operations that are repeated for every input event, and
concurrent state access (if applied) often turns out to be a
performance bottleneck. This pattern guides us to abstract
the processing as a three-step procedure: preprocess, state
access, and postprocess. While this formulation may appear to
limit the flexibility of programming, it unlocks the potential
for simple and effective optimization opportunities, which we
exploit to improve scalability.

amp_scheduling_2021:
In this paper, we introduce COLAB, an OS scheduling
policy for asymmetric multicore processors that makes
coordinated decisions targeting all three main factors in
thread scheduling - core sensitivity, thread critically and
fairness. Our scheduler uses three collaborating heuristics
to drive decisions about mapping threads to cores, each of
the heuristics foucing primarly on optimisation of one of
the factors. Collectively, these multi-factor heuristics result
in better thread schedules compared to the Linux and
WASH schedulers, therefore improving both performance
and energy consumption.

price_theory:
The novelty of our power management approach is that
it incorporates all the objectives outlined earlier within a
unified and scalable framework based on the foundations
of price theory [21] from economics. We implement our
approach within the Linux fair scheduler with minimal
modifications to the kernel. Moreover, our evaluations are
performed on a real heterogenous multi-core chip ARM
big.LITTLE.

amp_web:
In this paper, we demonstrate the benefits of big/little heterogeneous
systems in achieving an ideal performance and
energy trade-off via scheduling. We harness the key insight
that different webpages contain strong variances in load time
and energy consumption. Leveraging this fact, we propose
webpage-aware scheduling, a mechanism that explores the
webpage variance and intelligently schedules webpages using
different core and frequency configurations for minimizing the
energy while still meeting the cut-off constraint.

amp_QOS:
In this paper, we design and prototype Octopus-Man,
a QoS-aware task management system that addresses these
challenges and dynamically manages tasks on heterogeneous
multicores. Driven by runtime QoS measurements, Octopus-
Man exploits load changes to allocate latency-sensitive tasks to
the least power-hungry processing resources that are sufficient
to meet the QoS requirements. By continuously monitoring
QoS changes and carefully expanding, contracting and migrating
between wimpy/brawny core resources, Octopus-Man
is able to meet tail latency requirements, while minimizing
power consumption and improving server energy efficiency.
Octopus-Man requires no extra hardware support beyond the
heterogeneous multicore substrate and no modification to the
host OS.

amp_game:
In this paper, we propose a novel method for finegrained
classification of game scenes, and incorporate it in
a real-time predictive governing framework. This framework
can evaluate game workloads more accurately, and
has a better mapping between game scenes and individual
hardware configurations (including the appropriate type
of CPU cores, CPU working frequency and GPU working
frequency). Our work is based on several observations.
First, modern online 3D games may have thousands of
scenes, which we call the functional scenes, or F-scenes. Many
F-scenes with comparable complexities may have similar
computational demands. Second, mobile 3D games heavily
rely on OpenGL ES for user interface (UI) rendering. We
observe that the numbers of calls on different OpenGL
APIs are a relevant indicator for computational demands
and combining these different types of APIs can classify
thousands of F-scenes into a small number of scenes with
similar complexities.


abstract:
Specifically, \design holistically exploits both task pipeline and data partitioning schemes during compression, which results in a list of fine-grained execution tasks. 
Furthermore, we develop a cost model to guide the scheduling of those tasks among asymmetric multicores to satisfy processing latency constraints with minimum energy consumption considering both \emph{varying task-core preference} and \emph{asymmetric communication cost among cores}.
To validate our proposal, we implement a system prototype with five alternative approaches. 
%  several anti-interference co-design, us 
Our extensive experimental study of parallelizing three popular \compress algorithms 
with three real-world datasets show that (1) \design outperforms alternative approaches by up to 53\%; and (2) our cost-model can successfully guide \design to minimize energy consumption while sustaining different latency constraints.
\end{comment}
 
 We propose the \emph{Asymmetric Compressing} (\design) system prototype in this work. The core idea of \design is parallel-\compress-awareness and AMP-awareness.
To address the first challenge, \design explores two common approaches including 
1) task pipelining, where the whole \compress process called \emph{\compress job} can be decomposed into a list of execution \emph{stages}
, which can run independently by exchanging intermediate results via message passing;
and 2) data parallelism, each \emph{stage} may be replicated into multiple \emph{replicas} running in parallel threads handling subsets of input data concurrently. The per-\emph{stage} view is a fine-grained manner to 
fully expose the ILP and MLP of \compress, and mutiple \emph{replicas} can help to relieve the bottle neck by exploiting TLP. Then for the second challenge, we develop a cost model called \model in \design, which harnesses the ILP and MLP of each \emph{stage} and \emph{replica} to predict the \textbf{E}nergy consumption, \textbf{L}atency, and \textbf{C}ore load of the whole \compress job. To overcome the last challenge, \model takes the relative location  (i.e., AMP-distance with asymmetric core communication) of consecutive \emph{stages} into consideration. By fine-grained and hybrid parallelization as well as the \model model, \design can achieve both performance improvement and energy reduction by properly allocating the hardware resource of AMP to the \compress software. 
In addition to the fine-grained parallelization and \model model, 
%\xianzhi{Besides the fine-grained parallelization and \model model}, 
\design is equipped with an executor to provide a clean environment and the low overhead energy measurement to support the running of \compress.

\begin{comment}
We have implemented \design and five alternative approaches on our optimized test bed called \system, which involves a recent AMP platform \emph{rockpi 4a~\cite{amp_rockpi4}}, has a \emph{clean} software environment and provides accurate measurement of energy. \shuhao{Now, you see this seems very much less important. Consider remove it? Or Combine with the next paragraph, so leave it as just some minor experimental setup details.}
\end{comment}



%\xianzhi{We have implemented \design along with five alternative approaches, and conducted comprehensive experiments of \design and its competitors.}


We develop \design on the AMP processor rk3399, and conduct comprehensive experiments to evaluate \design and its competitors.
Specifically, we have examined both real world and synthetic data set. 
The results on concrete AMP processor rk3399 show that \design can achieve up to 53 \% energy reduction and always meet the latency requirements adaptively without core overload, as it has an accurate modeling of parallel \compress software and AMP hardware. Besides, our simulation indicates even more profits can be
gained by deploying \design on future AMP.

\emph{In summary, this paper makes the following contributions:}
\begin{myitemize}
    \item 
        We propose a system protype called \design to parallelize \compress with energy efficiency. (section ~\ref{sec:overview}) 
    \item 
        We exploit fine-grained parallelization of \compress on AMPs and presents a formal problem formulation of the parallelization optimization problem (section~\ref{sec:problem}). 
        % present a formal problem formulation of the scheduling optimization of \compress on AMPs (section \ref{sec:problem}). 
    \item 
        We propose a novel cost model called {\model} in \design to better schedule \compress on AMP, which can precisely estimate the energy, latency and core workload of \compress on AMP.  (section~\ref{sec:models}). 
    \item 
         We design the executor in \design, which has an anti-interference co-design and provide low-overhead accurate energy measurement to run the \compress (section~\ref{sec:implementation}).
    \item 
         We conduct a comprehensive evaluation on \design, which demonstrates that {\design} outperforms alternative solutions on varying \compress methods, stream data sets, system settings and hardware configurations(section \ref{sec:evaluation}).
\end{myitemize}
%challenges
% The appropriate scheduling to our goal is difficult due to following two major challenges:


% Like parallelizing other things (e.g., the stream processing engine~\cite{flink,storm}), parallel lossless stream compression (PLSC) includes 1) pipelined processing, i.e., to decompose the whole compression job into \emph{stages} and arrange them in a chain and 2) stage replications, i.e., each stage can have multiple \emph{replicas} running at the same time which only deals with a partition of all data. 


% On concrete devices, each \emph{stage} of PLSC and its all \emph{replicas} should be assigned with specific computational hardware resource for the real execution, and this process is scheduling or core-mapping for multicore systems including AMP. The goal this paper is to schedule the PLSC on AMP for least energy consumption, with acceptable latency and no CPU overload.

% Besides energy efficiency, saving the limited hardware resource like memory space is another concern for embedded and edge-based SP. Therefore,
%LSC is important, especially for embedded SP
% lossless compression (LC) on large volume of stream data, or lossless stream compression (LSC) for short, is introduced to reduce the inner redundancy of the data without breaking any information it carried on. This operation is of great help to boost stream processing(SP)~\cite{comp_tersecades} as it can provide more opportunities of in-memory-processing and save the bandwidth. 
%  Due to the stark contradiction between limited memory and infinite data, this operation is of particular importance. 
%we have PLSC, but not for energy-efficiency at  embedded IoT systems. 

% Starting in 1985~\cite{comp_1985} and thriving in this century,
% many have explored the parallelization of LSC or generic LC to improve the performance~\cite{comp_para_bzip2,comp_ndzip,comp_para_gpu,comp_para_lzss,comp_lz4_fpga}. However, since low latency or high throughput are their major concerns, they have not give enough attention to energy-efficiency, especially that at embedded IoT systems. 


% While it is compelling to process large streams of IoT data on the cloud edge
% The Internet of Things (IoT) combines large data centers with (mobile, networked) edge devices that are constrained both in compute power and energy budget. 
% is gaining popularity for continuous near real-time monitoring and analytics~\cite{sp_def}. 
% IHS Markit forecasts that 125 billion IoT devices will be in service by 2030, up from 27 billion in 2018~\cite{IoT_survey2019}. 
% Consequently, data is generated in high volume, velocity and variety. 
% Applications
% with time constraints are increasingly implemented in
% modern stream applications 

% ranging from machine-type communications to mission-critical communications in smart health care,
% smart homes, smart factory, autonomous driving, immersive entertainment, and smart city. 
% the IoT application is becoming one of the major sources of big data processing.
%

%Then introduce AMP
\begin{comment}


\shuhao{To address the aforementioned challenges, we propose the \emph{Asymmetric Compressing} (\design) in this work. 
In particular, \design considers xxx to address $C1$. To address $C2$, \design xxx.}

Witnessing this problem, we present a novel AMP-aware PLSC scheduling strategy as the first, which is named as \emph{Affinity and Cache Aware Mapping} (ACAM). 
Specifically, {\design} considers 
the core affinity according to a certain replica of specific compression stage handling specific data set (denoted as the \emph{execution unit})  by compression-specific analysis of algorithms along with synthetic adoption of the \emph{roof line model}~\cite{roofline_1st} on AMP, which is a fine-grained manner compared to black-box view of compression threads. In addition, we propose and use the \emph{slope model} in {\design} to address the variable and polar CC in AMP. If we define one of the ways to map \emph{stages} and their \emph{repliacas} of a PLSC algorithm to AMP cores as a \emph{scheduling plan}, {\design} can decide the best one as it can suitably determine the correlation between a \emph{scheduling plan} and its
objective value(e.g., , latency or energy). To reduce the cost of enumerate and analyzing each plan, we combine {\design}  with the dynamic programming~\cite{algo_dp_1954}.


\shuhao{
We have implemented \design from scratch and resolve a list of implementation and evaluation challenges. Specifically, xxx.
}

We implemented the {\design} on a customized embedded system, called the {\system}.
The key design of {\system} are 1)to only include and run the software that are \emph{in need} and 2) to achieve precise and non-invasive energy measurement by special hardware. Therefore, {\system} has a software-hardware co-design which can provide {\design} with necessary support in terms of run-time libraries and power measurement methods, without adding interference or overhead to {\design}.



\shuhao{We evaluate \design on a recent AMP platform \emph{rockpi 4a~\cite{amp_rockpi4}}, xxx}

Based on {\system}, we conduct evaluation on AMP platform rockpi 4a~\cite{amp_rockpi4}, where we use {\design} to schedule several classic PLSC algorithms against four data sets including full-text data, binary stream data and synthetic data in experimental studies comparing with competitors. The results show that {\design} can achieve 20 \% to 40 \%
saving in energy, while always meeting the assigned maximum latency and preventing each core from overloading.


\shuhao{
\emph{In summary, this paper makes the following contributions:}
\begin{myitemize}
    \item 
        We exploits fine-grained parallelization of \compress on AMPs and presents a formal problem formulation of the parallelization optimization problem (section~\ref{sec:problem}). 
        % present a formal problem formulation of the scheduling optimization of \compress on AMPs (section \ref{sec:problem}). 
    \item 
        We propose a novel parallelization paradigm called {\design} to better schedule \compress on AMP, by precisely estimating the energy, latency and core workload of them on AMP with a performance-model (section~\ref{sec:models}). 
    \item 
         We implement \design in a system prototype with several alternative approaches and address a list of issues in implementation, which has an anti-interference co-design and provide low-overhead energy measurement (section~\ref{sec:implementation}).
    \item 
         We conduct a comprehensive evaluation on the AMP platform, which demonstrates that {\design} outperforms alternative solutions on varying PLSC methods and stream datasets (section \ref{sec:evaluation}).
\end{myitemize}
}
\end{comment}



==> Sections/backup/2.5_Overview.tex <==

\section{Background
%\shuhao{why no discussion about the asymmetric communication cost??}
}
\label{sec:background}
%In this section, we introduce modern AMP (especially its asymmetric core communication) and provide an overview of the \compress.



\subsection{Modern AMP}
\label{subsec:amp_intro}
%\textbf{Purposes and Properties}.
%Initially, AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
%AMP was intended to improve energy efficiency and provide higher performance (i.e., by increased area efficiency) from the first beginning~\cite{amp_2003,amp_2004,amp_impacts_2005}.
 %To achieve these goals, AMP has two key characteristics. First, it involves different types of cores~\cite{amp_survey_2016}, which trade off performance with power to different degrees. 
 %Second, the different types of cores are formed within the same instruction set architectures (ISA).
% To reach the goals, there are two key factors of the AMP. First, it involves cores of different types~\cite{amp_survey_2016}, which trade off performance with power to different degrees. Next, the different types of cores are formed within the same instruction set architectures (ISA).
%Therefore, AMP embraces heterogeneity as a first principle, but still have convenient management methods and unified programming models by virtue of identical ISA.

We use the rk3399 processor~\cite{amp_rk3399} as an example to show the architecture characteristics of AMP,
as shown in Figure~\ref{fig:rk3399},
which has three key properties.

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/AMP.pdf}
    \caption{The 6-core AMP rk3399.}  \label{fig:rk3399}   
\end{figure}
%\textbf{Overview}.
%\label{subsec:amp}
%The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}. 

%Figure \ref{fig:rk3399} shows a concrete example of AMP, the rk3399 processor~\cite{amp_rk3399}. Three key properties of AMP can be observed in this processor as listed below. 

\begin{myitemize}
    \item \textbf{Asymmetric cores}. AMP couples different kinds of cores. This design can trade off performance with power to different degrees on the same processor under the same instruction set architectures (ISA). For rk3399, it couples both the in-order A53~\cite{amp_A53ug} cores and out-of-order A72~\cite{amp_A72ug} cores.
    
    \item \textbf{Asymmetric cache-memory structure}. The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the equivalent clock frequency setting.
    In contrast, the micro-architecture and frequency for cores from different \emph{clusters} are not identical.
    For instance, the A53 and A72 cores are placed at \emph{cluster0} and \emph{cluster1}, respectively in rk3399.
    
    \item \textbf{On-chip peripherals}. AMP for embedded systems has many peripherals to complete their embedded tasks (e.g., the I2C and the USB protocols~\cite{amp_i2c}). 
    The peripherals are arranged in unified addressing ways in RISC architectures like ARM~\cite{amp_arm}.
    In rk3399, I2C and other peripherals share the inter connection hardware CCI500~\cite{amp_CCI500} with cores, caches, and memory.
\end{myitemize}

In this paper, we focus on two major AMP effects according to the above properties.

\textbf{Energy reduction and performance improvement}.
The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
Specifically, the core asymmetry of AMP can exploit the fact that applications’ resource
requirements are different. The reason is that both high energy-efficient cores and high-performance cores are integrated on the same processor, and by the same contract between hardware and software. Accordingly, by deciding ``the right kind of core''~\cite{amp_scheduling_2021} to satisfy the application requirements, we can achieve either saving in energy or boosting in speed, and even both of them.
%AMP couples relatively battery-saving and slower cores with relatively more powerful and power-hungry cores within the ISA, which offers a large space for optimization.
%AMP integrates both high energy efficiency cores and high performance cores on the same processor and by the same contract between hardware and software, which offers a large space for optimization.
%The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
%Specifically, it exploits the fact that applications’ resource
%requirements are different~\cite{amp_latency_2015} by coupling different kinds of cores which trade off performance with power to different degrees on the same processor\ under the same instruction set architectures (ISA).
%software-hardware contract (e.g., the ARMv8 ISA).
%Thus, by deciding 'the right kind of core'~\cite{amp_scheduling_2021} to satisfy the requirements, we can achieve either saving in energy or boost in speed, and even both of them.
%This is totally different from symmetric multicore processors (SMPs), which must do the trade-off between performance and energy within the same type of cores.
\begin{comment}
\textbf{Applications}. AMP has been gaining much popularity these years~\cite{amp_iot}. Nowadays, top processor vendors like to apply the idea of AMP to build their flag-ship processors for edge and mobile computing: the rk3399(2016)~\cite{amp_rk3399} by Rockchip, the kirin 9000(2020)~\cite{amp_kirin9000} by Hisilicon and the snapdragon 8 Gen 1(2021)~\cite{amp_sd8g1} by Qualcomm; as they can enhance battery life, reduce the cost of cooling and overall improve system’s scalability and reliability in these scenarios specifically. Moreover, the application filed of AMP  will extend to personal computers and even data center, according to Intel's recent release of 12th generation \emph{Core} Processor~\cite{amp_i9_12} and AMD's new plans~\cite{amp_amd}.
\end{comment}

\textbf{Asymmetric core communication}.
%The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. 
The asymmetric   cache-memory   structure of AMP leads to asymmetric core communication.
%Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the same clock frequency setting, while these for cores from different \emph{clusters} are different. 
Following existing work~\cite{amp_partition_2019}, we define 
the communication between cores in the same cluster as \emph{intra-cluster} communication (red lines in Figure \ref{fig:rk3399}), and between cores in different clusters as \emph{inter-cluster} communication~\cite{amp_partition_2019} (blue lines). 
%This kind of organization forms the asymmetry in core communication.
The \emph{intra-cluster} communication can be achieved directly by cache sharing (e.g., L2 cache for rk3399), and it is bidirectional symmetric for the simple bridging of identical cores. The \emph{inter-cluster} communication on the other hand, is much more complicated for two reasons: First, it leads to more overhead, as it is achieved by special inter connection hardware like the CCI500~\cite{amp_CCI500}, which is often much lower than direct cache sharing. Second, it is \textbf{polar}, as data sink core resides at higher performance \emph{cluster} (e.g., core4) has to \emph{wait for} the data source if the source core belongs to a poorer performance \emph{cluster} (e.g., core0). This can increase the total communication overhead in hardware level of \emph{hand-shaking}, \emph{acknowledgement}, and \emph{synchronization}. However, the reverse process, i.e., from core in higher performance \emph{cluster} to core in poorer performance \emph{cluster}, suffers less
in waiting and synchronization, and leads to less overhead. Even worse, frequently addressing the on-chip peripherals can add more uncertainties and overhead to the \emph{inter-cluster} communication. 

%Besides, as the on-chip peripherals or protocols with relative low speed also share the hardware interconnection with the cores, frequently addressing them can add more uncertainties and overhead to the \emph{inter-cluster} communication. 



%The AMP have \emph{clusters} or \emph{cluster-like structures} to organize cores. 


\begin{comment}
\xianzhi{The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. }
\shuhao{maintains a cluster-like structure?}
%Typically, the same \emph{cluster} have cores under identical micro-architecture and within the same frequency domain, 
\xianzhi{Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the same clock frequency setting, while cores from different \emph{clusters} typically follow different micro-architectures, clock frequency settings or even both.}
\shuhao{Typically, cores within the same follow identical micro-architecture and share the same clock frequency setting?}
%while different \emph{clusters} contain cores different in micro-architecture, frequency domain or even both. 
\shuhao{Typically, cores within the same cluster follow an identical micro-architecture and share the same clock frequency setting, while cores from different clusters typically follow different micro-architectures, clock frequency settings or even both. Nevertheless, those cores share memory subsystem and adopt the same ISA.}
%Therefore \shuhao{Nevertheless?}, 
\xianzhi{Nevertheless,}
the two kinds of asymmetry in core and cache-memory structure are formed within the same ISA. 


\shuhao{those cores share memory subsystem and adopt the same ISA?}
The rk3399 processor~\cite{amp_rk3399} shown in Figure \ref{fig:rk3399} is a concrete example for AMP.

 This processor has two kinds of cores under ARMV8 64-bit ISA: the in-order A53~\cite{amp_A53ug} running under maximum frequency 1.416GHz (core0 to core3)  and the out-of-order (OoO) A72~\cite{amp_A72ug} running under maximum frequency 1.8GHz (core4 to core5), and they are placed in \emph{cluster0} and \emph{cluster1} respectively. The communication between cores in the same cluster (e.g., core0 and core1) is \emph{intra-cluster}, and between cores in different clusters (e.g., core0 and core4) is \emph{inter-cluster}. While the \emph{intra-cluster} communication is carried on directly by shared L2 cache of the \emph{cluster}, the \emph{inter-cluster} communication requires data transferring through the CCI500~\cite{amp_CCI500}, which is a cross-bar inter connection hardware with snoop filter entries for the coherent between \emph{clusters}. 
\shuhao{shows a the rk3399 processor which is a concrete example of AMP. This processor has two kinds of cores under ARMV8 64-bit ISA: the in-order A53 with a maximum frequency of 1.416GHz (core0~core3) and the out-of-order (OoO) A72 with a maximum frequency of 1.8GHz (core4~core5), and they are placed in cluster0 and cluster1 respectively. The  intra-cluster communication is carried on directly by shared L2 cache of the cluster, while the inter-cluster communication requires data transferring through the CCI500, which is a cross-bar inter connection hardware with snoop filter entries for the coherent between clusters.}


The L2-based  \emph{intra-cluster} and the CCI500-based \emph{inter-cluster}  data sharing form the asymmetry of core communication, and they are drawn as red lines and blue lines respectively in Figure \ref{fig:rk3399}.
For the \emph{intra-cluster} communication, it does not need to go through the slower CCI500 so has less overhead, and it is also  without polarity due to its simple bridging of the symmetric cores within the same \emph{cluster}.  The \emph{inter-cluster} communication is on the contrary, with both more overhead and the communication polarity.
 To illustrate the \emph{inter-cluster} communication further, let's now consider an data transferring from core0 (A53) to core4 (A72), and allow both of them to run at maximum
frequency (1.416GHz and 1.8GHz respectively). In this case, core4 will always have to \emph{wait for} core0 due to 1) its higher frequency and 2) its OoO nature with more greedy cache line fetching, which increase the total communication overhead in hardware level of \emph{hand-shaking}, \emph{acknowledgement} and \emph{synchronization}, etc. So this communication process has to \emph{go through the narrow and slower path} in Figure \ref{fig:rk3399}. However, the reverse process, i.e., from core4 to core0, is faster, as slower and less greedy core0 for data sink will lead to less suffering in waiting and synchronization.
\end{comment}

\begin{comment}
The formulation of The asymmetric core communication is demonstrated in subsection \ref{subsec:latency}, and experiments in subsection \ref{sucsec:confirmation} will do the confirmation.


In addition to the cache and memory, AMP for embedded systems have many peripherals to finish their embedded tasks (e.g., the I2C and the USB protocols~\cite{amp_i2c}), and they are arranged in unified addressing ways in some RISC architectures like ARM~\cite{amp_arm}. As these peripherals or protocols with relative low speed also share the hardware interconnection with cores, frequently addressing them can add more uncertainties and overhead to the \emph{inter-cluster} communication. 

\end{comment}


\subsection{Streaming Lossless Compression}
% In this work, we limit our scope to lossless data stream compression. To further extending our work to lossy data stream compression is important but left as a future work.
\textbf{Principles of \compress}. By analyzing existing works, we observe that lossless data stream compression can be achieved  by 1) using \emph{dictionary} to represent the repeated sequence~\cite{comp_lzFamily},   2) cutting off unnecessary bits ~\cite{comp_elias,comp_baseDelta}, and 3) variable length coding approaching the entropy~\cite{comp_huffman}. 
Moreover, the complexity of lossless data stream compression must be \emph{relatively low} within an acceptable time overhead. 
Complicated algorithms like the original huffman encoding or the original LZ77 cannot be applicable,
as discussed in ~\cite{comp_tersecades,db_comp0,db_comp1}.


%according existing work in stream~\cite{comp_tersecades} and in-memory database compression~\cite{db_comp0,db_comp1}. 

\textbf{Algorithms used in this paper}. 
We introduce and adopt three compression algorithms for \compress in this paper as follows. All of them are with relatively low overhead.
We use these algorithms because they are representative and can cover all of the three common approaches for \compress. Furthermore, 
the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.

\begin{myitemize}
    \item \textbf{lz4}~\cite{comp_lz4} is a widely-used  LZ77-based~\cite{comp_lzFamily} compression. It uses a hash table to replace the traditional \emph{dictionary} of LZ77, so it is much faster than LZ77.
    \item \textbf{tcomp32} is a simplification of elias encoding~\cite{comp_elias}, which is already claimed as 'light-weight' in cutting off bits by existing works~\cite{db_comp0}. We change its encoding methods with a fixed length-indicator, so it is more stable in dealing with stream data with more variety.  
    
    \item \textbf{tdic32} is a simplified variable length coding by the hybridization of two above, as it borrows the hash table from lz4 and uses a memory I/O pattern similar to tcomp32 (i.e., per 32-bit single symbol). The frequently-showed symbols are encoded with their hash index (which is always shorter). Those not found in hash table are  encoded by their original values together a one-bit indicator (which means longer encoding).  
\end{myitemize}

%The specific algorithm of lz4, tcomp32 and tdic32 are presented in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of \emph{a segment of code lines} (or \emph{code segment} for short), and the {//} for \emph{a certain line of code}. These algorithms are representative enough for this work, as they cover all of the three common approaches for \compress. Therefore, the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.

\textbf{AMP-aware opportunity}.
 None of existing work has parallelized \compress on AMP, though this combination is feasible and can achieve significant reduction in time and energy overhead. 
 %\xianzhi{extend this part?}
 On the one hand, \compress involves varying data transformation (e.g., replace a data sequence by its \emph{lz4 token}) and memory addressing (i.e., read and write data by aligned or unaligned memory I/O), which leads to diverse ILP and MLP among different algorithms, and even within the same one.
 According to existing work in parallelization~\cite{comp_paralz_2013,comp_lzss_cuda}, it can be further accelerated by TLP (i.e., by running multiple threads which only handle a part of the whole data). On the other hand, the \textbf{a}symmetric cores in AMP provide flexible support to optimize the execution for different ILP and MLP, and the  
  \textbf{m}ulticores in AMP can directly support the TLP. The rest part of this paper can illustrate how to achieve the combination and optimization.
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/fstages.pdf}
    \caption{The \compress pipeline of $s0$, $s1$ and $s2$ .}  \label{fig:chain}   
\end{figure}

==> Sections/backup/2_20220525.tex <==
\section{Design Aspects of Stream Compression at the Edge}
\label{sec:preliminaries}
We first classify and summarize the algorithms of stream compression. 
Then, we introduce the edge computing hardware, especially the in asymmetric multicore processors (AMPs). Finally, we discuss the impacts of workload characteristics the edge-based stream compression. 

% and then review the related work on AMP-aware task scheduling and parallel data compression.
\subsection{Stream Compression Algorithms}

 \begin{figure}[t]
    \centering
    \includegraphics*[width=0.32\textwidth]{figures/overView_sc.pdf}
    \caption{Overview of stream compression algorithms.}
    %\shuhao{(Mark ``big'' and ``little'' cores in figure)}}  
    \label{fig:sc_comp_overview}   
\end{figure}
 
 Stream compression, different from file compression~\cite{comp_zlib} and  data base compression~\cite{db_comp0}, is distinguished by three major aspects as illustrated in Figure~\ref{fig:sc_comp_overview}. 
 First, it is an incremental procedure due to the incremental nature of streams. That's to say, the compression on \emph{current tuple} (i.e., that arrives most recently) can rely on 1) its self and 2) the \emph{past tuples} (i.e., those arrives earlier than the current tuple), and has no reference to the \emph{future tuples} which haven't arrived yet.
 Second, it should be ultra-low latency compression as the streams are also time-sensitive.
 Therefore, parallelization is typically required and multiple execution units (e.g., CPU/GPU cores, FPGA logic arraies, etc.) are running together.
 Third, it is conducted in cache and memory and typically without disk I/O. To improve the performance, the \emph{micro-batching} procedure
accumulating tuples in cache or memory is also introduced just as the spark~\cite{sp_spark} streaming engine does.
 We classify the algorithms and summarize their tuning factors based on the principles above.
 
 \subsubsection{Utilization of the State}
 \label{subsec:intro_state}
 A lot of compression methods have been proposed since 1950s~\cite{comp_huffman}, including
improving the theoretical compressibility~\cite{comp_7z} and
reducing compressing complexity on single core~\cite{comp_survey_2017,comp_survey_huffman}.  
 We classify those applicable for stream compression as \emph{stateless} and \emph{stateful} according to their different policies towards the past tuples. This classification is inspired by text compression cases as defined by Kelesy~\cite{comp_stateful_text}. Typically, stateless stream compression relies only on the current tuple, while stateful stream compression also refers to the past tuples and maintains a \emph{state} (e.g., such as an incremental dictionary~\cite{comp_lzFamily}) to record them.
 Such different policies lead to different procedures, compressibilities and complexities, and we discuss the stateless and stateful stream compression as follows.
 
 \textbf{Stateless stream compression} consists of a set of operations that are repeated for every ``current'' input tuple, and have nothing to do with others.
Therefore, they can be summarized as  a three-step procedure: read, transform, and output, as summarized in Algorithm~\ref{alg:stateless}. First, the tuples are buffered into micro batches~\cite{storm} before they can be handled in the following steps. This step is mostly about memory copy, and therefore memory-bound. Second, the $s1$ finds compressible parts for each tuple in the micro batch, such as zero redundancy in different levels~\cite{comp_tersecades}. Arithmetic and logical operations are typically involved in this step, making it have higher operational intensity~\cite{roofline_toolkit} (or more instruction-bound) than $s0$. Third and finally, the $s2$ outputs the compressed data to the output stream according to the inner redundancy of tuples we have found. This step involves both integer/float operation and memory access, and typically has a middle level of  operational intensity compared with $s0$ and $s1$.
As the compressibility is mostly achieved in the transformation of single tuple in $s1$, stateless compression is considered as ``light-weight''~\cite{comp_tersecades}.
However, it can only achieve relatively low compressibility as the context relationship (i.e., in symbolic~\cite{comp_huffman} or transform domain~\cite{dct_comp} patterns, etc) between current tuple and past tuples is totally ignored.
 \begin{algorithm}
\caption{Stateless stream compression}
\label{alg:stateless}
\LinesNumbered 
\KwIn{input stream $inData$}
\KwOut{output stream $outData$}
\While{$inData$ is not stopped}
{
    (s0) buffer the tuples from $inData$ \label{algo:stateless_S0} \;
    (s1) transform and find the \emph{compressible} parts\label{algo:stateless_S0}\;
    (s2) output compressed data to $outData$ \label{algo:stateless_S0}\;
}
\end{algorithm}
 
 \textbf{Stateful stream compression} maintains a state for compressing, and a more complicated 5-step procedure is followed as shown in Algorithm~\ref{alg:stateful}. Except the micro batching (i.e., $s0$) and outputting (i.e., $s4$) similar to stateless compression case, it conducts the compression based on state-access. First, $s1$ preprocesses some value before
 accessing state (such as an index of a dictionary. Second, $s2$ updates the state in-cache (or in-memory) with 1) the current tuple and 2) $s1$-produced value.
 Third, the encoding is achieved by $s3$. Due to the state write or read, $s2$ and $s3$ introduces more memory operations than $s1$. Compared with stateless stream compression, the stateful compression is more complicated due to the mountainous of state. On the other hand, context relationship can be utilized in stateful compression, which may increase the compressibility.
 \begin{algorithm}
\caption{Stateful stream compression}
\label{alg:stateful}
\LinesNumbered 
\KwIn{input stream $inData$}
\KwOut{output stream $outData$}
\While{$inData$ is not stopped}
{
    (s0) buffer the tuples from $inData$ \label{algo:stateful_S0} \;
    (s1) pre-process \label{algo:stateful_S1} \;
    (s2) state update  \label{algo:stateful_S2} \;
    (s3) sate-based encoding\label{algo:stateful_S3}\;
    (s4) output compressed data to $outData$ \label{algo:stateful_S3}\;
}
\end{algorithm}
 %
 
 It is worth noting that concurrent writing may occur in the state update (i.e., $s2$ in Algorithm~\ref{alg:stateful}) if parallelized~\cite{comp_para_lzss}. Specifically, two or more parallel execution units (i.e., CPU/GPU cores, FPGA logic arrays, etc) may try to update the same part of the global state with different values. In this case, we can either use concurrency control like locks to avoid the conflicts, or just allow them to maintain their own state and disable the sharing. The sharing-or-not towards state increases the design space of stateful stream compression.

 \subsubsection{Parallelization granularity}
 \label{subsec:intro_grandularity}
 To reduce the latency overhead of compressing, many recent works~\cite{comp_paralz_2013,comp_para_hsi,comp_fp_2010,comp_gpu_lossy,comp_lz4_fpga} target compressing static datasets in parallel. 
%For example, Burtscher et al. compress the float-point data~\cite{comp_para_pfc} and to drill the inner parallelism (in a SIMD-like manner) of LZ77~\cite{comp_paralz_2013} on multicores.
%Recently, Knorr et al.~\cite{comp_ndzip} achieved high-throughput compressing of large volumes of scientific data scaling up to 24 threads, and Dua et al.~\cite{comp_para_hsi} compressed the hyperspectral images on supercomputer with a hyper-cube structure. Researcher have also utilized hardware accelerators like FPGA and GPU for parallelzing data compressing~\cite{comp_2004_tpds,comp_fp_2010,comp_waveSz,comp_lz4_fpga,comp_lzFamily,comp_lzss_cuda,comp_mpc_2015,comp_gpu_lossy}. 
Their parallelization is conducted in different granularity, due to the diversity of targeted devices and desired performance. In this work, we focus on revisiting parallel stream compression on edge devices and further take energy consumption into consideration.
The  pros and cons of different granularity are discussed as follows.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/parallel_dd.pdf}
    \caption{The coarse grained parallelization DD}
    \label{fig:parallel_dd}
\end{figure}

\textbf{A coarse grained compression} on data stream conducts simple data dividing (DD) for the entire compression procedure, as depicted in Figure~\ref{fig:parallel_dd}. Here, each execution unit is distributed with a partition of workload as assigned by a \emph{distribution ratio}. Specifically, we let $distribution\ ratio = \frac{\text{assigned workload size}}{\text{total workload size}}$ for each kind of execution unit(s).
Such a ratio
is shared by all compression steps (e.g, $s0$ $\sim$ $s2$ for stateless compression in Algorithm~\ref{alg:stateless}). The shared ratio simplifies the parallelization design, and achieves low communication overhead as each execution unit only needs to fetch data from its own \emph{local-coupled} memory (e.g. the L1D cache). 

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/parallel_pl.pdf}
    \caption{The fine grained parallelization PL}
    \label{fig:parallel_pl}
\end{figure}
\textbf{A more fine grained pipelined parallelization} (PL) is shown in Figure~\ref{fig:parallel_pl}. On the contrary to DD, each step can have its own work distribution ratio on execution units. Theoretically, the PL approach can provide better exploitation of different compression behaviors in different steps. For instance, to improve the energy efficiency, the memory-bounded $s0$ in Algorithm~\ref{alg:stateless} should be distributed less to the higher performance hardware compared with $s1$. However, more complicated communication is introduced to PL than DD, as one execution unit may fetch data from another due to the ratio divergence in different steps.
 \subsubsection{Tunable batch size}
 The micro batching processing utilizes cache and memory to accumulate and buffer tuples~\cite{sp_spark,sp_intra_exp}. 
 In most modern computational devices, the cache and memory
 are layered and have different speed grades and capacities.
 Therefore, a nature question arises as ``how many tuples should be batched in stream compression''. On the one hand, batching a too small number of tuples leads to frequent flush and reload. On the other hand, a larger number means we have to store tuples in slower memory storage. Therefore, it's necessary to determine a suitable size.
 %We explore such dilemma through experiments in section~\ref{}.
 \subsection{Edge Computing Hardware}
 Placed near the data source and faced with so-called \emph{13 V's challenges~\cite{IoT_survey2019}} of IoT, the edge computing hardware features different strategies compared with a high-performance data centers~\cite{nebulastream}. In particular, these devices adapt various designs in balancing the low latency demand and the low energy consumption constraint. We summarize three common utilization variants of them as follows.
 \subsubsection{Architecture Awareness}
 \label{subsec:intro_arch}
 \shuhao{Always add some sentences after the section title.}
 
 \textbf{Symmetric Architecture.} The idea of symmetric multicore processor (SMP) is not only widely used in center servers, but also applicable at edge devices. For instance, the raspberry pi 4 platform~\cite{amp_rasp4} adopts the 4-core SMP bcm2711. The major difference between SMP at the edge and SMP at the center is that each core of edge SMP is generally more energy-efficient and less powerful than that at the center.
 
 \textbf{Asymmetric Architecture.}
 Simply replacing cores can not thoroughly achieve a good trade-off between latency and energy consumption, as this strategy is still too fixed under the IoT environment. For instance, an overprovisioned processor
core will waste area and energy, whereas an underprovisioned core will fail to provide high performance~\cite{amp_survey_2016}.
 To be more flexible and more energy-efficient, the asymmetric architecture has been proposed in 2000s~\cite{amp_2003}, and is gaining increasing popularity nowadays~\cite{amp_arm,edge_survey}. The key of asymmetric architecture is to feature different types of execution units (e.g. cores) on the same processor, which opens up new optimization opportunities for stream compression. Yet the general, this study limit the scoop to the asymmetric architecture within single instruction set architecture (ISA), known as \emph{asymmetric multicore processors (AMPs)}~\cite{amp_survey_2016}, and leave the consideration of other asymmetric architectures such as the coupled edge CPU+GPU~\cite{edge_cpu_gpu,edge_cpu_gpu_2}, CPU+DSP~\cite{couple_cpu_dsp} and CPU+FPGA~\cite{yang2015adaptive}, etc. for future work.
 \begin{figure}[t]
    \centering
    \includegraphics*[width=0.32\textwidth]{figures/AMP.pdf}
    \caption{The 6-core AMP rk3399.}
    %\shuhao{(Mark ``big'' and ``little'' cores in figure)}}  
    \label{fig:rk3399}   
\end{figure}
\begin{table}[t]
\centering
\caption{Hardware Specifications. The unit of latency is ``ns per 32-bit access''.}
\vspace{+3pt}
\label{tab:asymmetry}
\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{|L{2cm}|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Asymmetric\\  cores\end{tabular}}        & \textbf{Type} & \textbf{L1 cache size}   & \textbf{Pipeline} \\ \cline{2-4} 
 & A72 & 48K I+ 32 K D                 & out-of-order     \\ \cline{2-4} 
 & A53 & 32K I+ 32K D                  & in-order \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Asymetric\\  communication\end{tabular}} & \textbf{Path} & \textbf{Description} & \textbf{Latency}  \\ \cline{2-4} 
 & c0  & intra-cluser                  & 4.4          \\ \cline{2-4} 
 & c1  & inter-cluster, cluster 1 to 0 & 8.9          \\ \cline{2-4} 
 & c2  & inter-cluster, cluster 0 to 1 & 26.3         \\ \hline
\end{tabular}%
}
\end{table}

 

Figure~\ref{fig:rk3399} shows the architecture of a recent AMP, rk3399~\cite{amp_rk3399}. 
The detailed hardware specifications are summarized in Table~\ref{tab:asymmetry}. 
In the following, we summarize two important asymmetry properties of AMPs, including both computation and communications.
% , and then review the existing approaches in exploiting such asymmetries.

\emph{Asymmetric computation.}
AMPs maintain a cluster-like structures to organize cores~\cite{amp_survey_2016}.  
Cores within the same cluster follow identical micro-architecture and share the equivalent clock frequency setting.
Despite the sharing of ARM V8 ISA~\cite{amp_armv8}, the rk3399 involves different types of cores on the same processor: the relatively batter-saving and slower A53 cores (also called ``little core'')~\cite{amp_A53ug} at cluster 0 and more powerful and power-hungry A72 cores (also called ``big core'')~\cite{amp_A72ug} at cluster 1. 

\emph{Asymmetric computation.}
There are two kinds of core communication in AMPs~\cite{amp_cluster_2021, amp_partition_2019}, i.e., \emph{intra-cluster} and \emph{inter-cluster} communication. The \emph{intra-cluster} communication (denoted as \emph{c0} in Figure~\ref{fig:rk3399}) is the direct sharing of L2 cache for cores within the same cluster, while \emph{inter-cluster} communication (denoted as \emph{c1} and \emph{c2}, respectively) represents that communication between cores went through a much slower interconnection link (i.e., CCI500). 
Such a hardware architecture is conceptually similar to NUMA~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
% This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
Different from NUMA, \emph{inter-cluster} communication on AMPs further involves additional \emph{polarity} effects. 
\xianzhi{Specifically, transferring data from little cores to big cores is more costly than the reverse process.
This is because big cores are typically faster than little cores and should wait for the little cores, which increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.}

As revealed in prior work~\cite{amp_impacts_2005, amp_modeling, amp_scheduling_2021, amp_pie_2011}, software with different operational intensity~\cite{roofline_boat} (i.e., instruction amount per unit memory access) have different preference on big cores and little cores in saving energy or time.
Therefore, by utilizing the asymmetric computation, i.e., distributing the stream compression software to the \emph{right} cores, we can gain a satisfying trade-off between latency and energy consumption. However, the latency penalty of asymmetric communication effects is also unignorable and requires careful design.
 
 \subsubsection{Frequency Regulation}
 \label{subsec:freq_regu}
 Tuning the frequency on edge computing hardware leads to different latency and power consumption, which is a physical kind of trade-off. In this study, we explore how this trade-off act in stream compression. Specifically, the energy consumption of stream compression is the product of power and time, which have different changing patterns with the frequency. Moreover, the frequency can not only be determined statically, but also be regulated dynamically by the DVFS technology~\cite{amp_DVFS1,amp_DVFS2,amp_DVFS3}. As DVFS tries to provide the \emph{minimal but necessary} frequency on the fly, it can theoretically make stream compression more energy efficient. However, the frequency switches during DVFS introduces extra overhead, and we are especially interested in whether the benefits of DVFS can outperform its overhead in stream compression.   
 \subsubsection{Number of Cores}
  \label{subsec:number_of_cores}
 Cloud-based stream processing~\cite{sp_briskstream,sp_coprocessing} always assumes to use all available computational resources due to the high-performance-first requirement. However, due the strict energy constraint at the edge, this assumption can not usually function. Specifically, some processor cores can be turned off or sleep in edge-based stream compression, in order to further save energy. In this study, we explore whether such regulation on numbers of enabled cores is \emph{fair} for energy cost and time cost. 
 \subsection{Impacts of the Workload}
 \label{subsec:intro_workload}
 The mobility and universality of IoT makes data property different from that in traditional
big data applications~\cite{IoT_survey2019,nebulastream}. Specifically, the IoT data stream has huge dynamics in both arrival pattern and statistic properties.
 
 \subsubsection{Arrival Pattern}
 \label{subsec:arrival}
 There are two facts of IoT which contribute to different arrival patterns of the data stream. First, there are wave crests and troughs in real world events. For instance, the visitor tracking system placed at a mall may generate more data within unit time when there is a promotion, as more people enters such place. Second, massive data are generated by mobile devices under complex network environment, which can also influence the data transmission. In the following, we consider the following arrival patterns caused by them:
 \begin{itemize}
     \item \textbf{Arrival rate}, which refers to how much data arrives during a time period.
     \item \textbf{Arrival skewness}, which means that during a certain studying time period, more data may arrive more intensively sometimes.
 \end{itemize}
 \subsubsection{Statistics Properties}
 \label{subsec:bg_statistics}
% \xianzhi{need polish after reading more...}
IoT data streams also have changeable statistics properties, as they are the reflection of real world. Specifically, they have different \emph{dynamic range} and \emph{tuple duplication}.
A stateless stream compression may be sensitive to dynamic range, as it compresses on the value of each single tuple. A stateful compression, on the other hand, may be more sensitive to tuple duplication as it explores the content relationship of stream for conducting compression. Such different interaction between workload and algorithm leads to different cost of compression in both latency and energy consumption.
%, as we evaluated in Section~\ref{}.


 

\begin{comment}


\subsection{The AMP Architecture}
\label{subsec:amp_intro}

The AMPs are designed to improve energy efficiency~\cite{amp_2003, amp_2004, amp_impacts_2005}, and they can trade off performance with power to different degrees. 
Figure~\ref{fig:rk3399} shows the architecture of a recent AMP, rk3399~\cite{amp_rk3399}. 
The detailed hardware specifications are summarized in Table~\ref{tab:asymmetry}. 
In the following, we summarize two important asymmetry properties of AMPs, including both cores and communications.
% , and then review the existing approaches in exploiting such asymmetries.

\textbf{Big and Little Cores.}
AMPs maintain a cluster-like structures to organize cores~\cite{amp_survey_2016}.  
Cores within the same cluster follow identical micro-architecture and share the equivalent clock frequency setting. For instance, the rk3399 consists both the relatively batter-saving and slower A53 cores (also called ``little core'')~\cite{amp_A53ug} at cluster 0 and more powerful and power-hungry A72 cores (also called ``big core'')~\cite{amp_A72ug} at cluster 1. All cores share the same ISA (i.e., the ARM v8 ISA~\cite{amp_armv8} for rk3399) despite the asymmetry.

\textbf{Intra- and Inter-Cluster Communication.}
There are two kinds of core communication in AMPs~\cite{amp_cluster_2021, amp_partition_2019}, i.e., \emph{intra-cluster} and \emph{inter-cluster} communication. The \emph{intra-cluster} communication (denoted as \emph{c0} in Figure~\ref{fig:rk3399}) is the direct sharing of L2 cache for cores within the same cluster, while \emph{inter-cluster} communication (denoted as \emph{c1} and \emph{c2}, respectively) represents that communication between cores went through a much slower interconnection link (i.e., CCI500). 
Such a hardware architecture is conceptually similar to NUMA~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
% This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
Different from NUMA, \emph{inter-cluster} communication on AMPs further involves additional \emph{polarity} effects. 
%Specifically, the communication cost from poorer performance source to higher performance sink (i.e., \emph{c2}) is always larger than its reverse process (i.e., \emph{c1}). 
\xianzhi{Specifically, transferring data from little cores to big cores is more costly than the reverse process.
This is because big cores are typically faster than little cores and should extra wait for them, which increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.}


%as extra waiting of big cores for its little cores increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.
%\shuhao{This is due to the extra waiting of a higher performance sink for its source increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.} 

\subsection{Parallel Data Compression}
\label{subsec:bg_comp}
To improve the compressing throughput, many recent works target compressing static datasets in parallel. 
For example, Burtscher et al. compress the float-point data~\cite{comp_para_pfc} and to drill the inner parallelism (in a SIMD-like manner) of LZ77~\cite{comp_paralz_2013} on multicores.
Recently, Knorr et al.~\cite{comp_ndzip} achieved high-throughput compressing of large volumes of scientific data scaling up to 24 threads, and Dua et al.~\cite{comp_para_hsi} compressed the hyperspectral images on supercomputer with a hyper-cube structure. Researcher have also utilized hardware accelerators like FPGA and GPU for parallelzing data compressing~\cite{comp_2004_tpds,comp_fp_2010,comp_waveSz,comp_lz4_fpga,comp_lzFamily,comp_lzss_cuda,comp_mpc_2015,comp_gpu_lossy}.

Different from compressing over static datasets, stream compressing~\cite{comp_tersecades,Scabbard} contains three additional constraints.
% When considering compression on continues streams~\cite{comp_tersecades,Scabbard}, three additional constraints are enforced as
First and foremost, the compression should be incremental so that processing of the current incoming tuple need not be dependent on the other tuples coming in the future. 
Second, the latency of conducting compression should be as low as possible to avoid the input stream be blocked due to compression and fail to be processed timely. 
Third, memory footprint of compression shall be constant and can not grow rapidly along with the ever-increasing amount of data.
Recent studies have proposed low-latency parallel stream compression algorithms on multicores and GPUs~\cite{comp_tersecades,Scabbard}. 
% However, it is unclear how can those works be applied for parallel stream compression on AMPs.
In this work, we focus on revisiting parallel stream compression on AMPs and further take energy consumption into consideration.
%\xianzhi{stateless/stateful here???}
\end{comment}
% The specific algorithm of lz4, tcomp32 and tdic32 are presented in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of \emph{a segment of code lines} (or \emph{code segment} for short), and the {//} for \emph{a certain line of code} . 
%  the Symmetric Multicore Processors (SMPs) for parallel compression:
% Our experiments have shown that SMPs-aware parallelization results in poor performance on AMPs.

\begin{comment}
\textbf{Choices of Compression Schemes}. Since the 1950s~\cite{comp_huffman}, a lot of methods have been proposed for improving the theoretical compressibility~\cite{comp_7z}, 
reducing compressing complexity on single core~\cite{comp_survey_2017, comp_survey_huffman}, 
accelerating compression~\cite{comp_acc}, and reducing the energy dissipation~\cite{comp_energy_2006} . However, not all of them are applicable for the compression on streaming data, and some of them lack the generality and can only be narrowly applied to specific occasions. For instance, lossy compression methods such as transform coding~\cite{comp_trans} are widely used in multimedia streams (e.g., video frames~\cite{comp_video}), but they will cause unacceptable corruption to the streams of faint yet vital data (e.g., those produced by body area networks~\cite{body_survey}). 

The dictionary compression strategies, 
which operate by searching for
matches between the data to be compressed and a set of strings (also called the vocabularies)
contained in a dictionary, have high level of adaptivity and universality. The well-known examples of them are LZ77~\cite{comp_ziv_lz78}, LZ78~\cite{comp_ziv_lz78} and their extensions such as 7z~\cite{comp_7z}, and lz4~\cite{comp_lz4}. A recent evaluation on stream of Dynamic Vision Sensor (DVS) data~\cite{comp_dvs} proved that dictionary compression, thought as a general way, can even outperform most scenario-specific compression. 

Entropy encoding strategies are also versatile. Unlike the dictionary compression which reorganize vocabularies and take advantage of their duplication patterns, entropy coding tries to make the average code length of symbols as close as possible to the Shannon's entropy, and a symbol can be one single byte (8-bit), word (32-bit), etc. in practice.
While the classic ways like huffman encoding~\cite{comp_survey_huffman} and Arithmetic encoding~\cite{comp_arithmatic} may be costly sometimes in building their code books or calculation, recent approaches such as Finite State
Entropy (FSE)~\cite{comp_fse} can achieve a trade-off between compression ratio and
speed. Besides stand-alone deployment, entropy coding can also be chained after a dictionary compression to achieve better compression ratio. This idea has achieved great success in the well-known Zlib~\cite{comp_zlib} and Zstd~\cite{comp_zstd}.

This paper revisits the dictionary compression and entropy encoding due to their versatility. Moreover, we exploit the fine-grained parallelization to meet stricter latency constraints, and use the AMP-aware core mapping of tasks to be energy efficient. 


\end{comment}


==> Sections/backup/2_Aspects_OLD.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\begin{comment}


\subsection{The AMP Architecture}
\label{subsec:amp_intro}

The AMPs are designed to improve energy efficiency~\cite{amp_2003, amp_2004, amp_impacts_2005}, and they can trade off performance with power to different degrees. 
Figure~\ref{fig:rk3399} shows the architecture of a recent AMP, rk3399~\cite{amp_rk3399}. 
The detailed hardware specifications are summarized in Table~\ref{tab:asymmetry}. 
In the following, we summarize two important asymmetry properties of AMPs, including both cores and communications.
% , and then review the existing approaches in exploiting such asymmetries.

\textbf{Big and Little Cores.}
AMPs maintain a cluster-like structures to organize cores~\cite{amp_survey_2016}.  
Cores within the same cluster follow identical micro-architecture and share the equivalent clock frequency setting. For instance, the rk3399 consists both the relatively batter-saving and slower A53 cores (also called ``little core'')~\cite{amp_A53ug} at cluster 0 and more powerful and power-hungry A72 cores (also called ``big core'')~\cite{amp_A72ug} at cluster 1. All cores share the same ISA (i.e., the ARM v8 ISA~\cite{amp_armv8} for rk3399) despite the asymmetry.

\textbf{Intra- and Inter-Cluster Communication.}
There are two kinds of core communication in AMPs~\cite{amp_cluster_2021, amp_partition_2019}, i.e., \emph{intra-cluster} and \emph{inter-cluster} communication. The \emph{intra-cluster} communication (denoted as \emph{c0} in Figure~\ref{fig:rk3399}) is the direct sharing of L2 cache for cores within the same cluster, while \emph{inter-cluster} communication (denoted as \emph{c1} and \emph{c2}, respectively) represents that communication between cores went through a much slower interconnection link (i.e., CCI500). 
Such a hardware architecture is conceptually similar to NUMA~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
% This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
Different from NUMA, \emph{inter-cluster} communication on AMPs further involves additional \emph{polarity} effects. 
%Specifically, the communication cost from poorer performance source to higher performance sink (i.e., \emph{c2}) is always larger than its reverse process (i.e., \emph{c1}). 
\xianzhi{Specifically, transferring data from little cores to big cores is more costly than the reverse process.
This is because big cores are typically faster than little cores and should extra wait for them, which increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.}


%as extra waiting of big cores for its little cores increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.
%\shuhao{This is due to the extra waiting of a higher performance sink for its source increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.} 

\subsection{Parallel Data Compression}
\label{subsec:bg_comp}
To improve the compressing throughput, many recent works target compressing static datasets in parallel. 
For example, Burtscher et al. compress the float-point data~\cite{comp_para_pfc} and to drill the inner parallelism (in a SIMD-like manner) of LZ77~\cite{comp_paralz_2013} on multicores.
Recently, Knorr et al.~\cite{comp_ndzip} achieved high-throughput compressing of large volumes of scientific data scaling up to 24 threads, and Dua et al.~\cite{comp_para_hsi} compressed the hyperspectral images on supercomputer with a hyper-cube structure. Researcher have also utilized hardware accelerators like FPGA and GPU for parallelzing data compressing~\cite{comp_2004_tpds,comp_fp_2010,comp_waveSz,comp_lz4_fpga,comp_lzFamily,comp_lzss_cuda,comp_mpc_2015,comp_gpu_lossy}.

Different from compressing over static datasets, stream compressing~\cite{comp_tersecades,Scabbard} contains three additional constraints.
% When considering compression on continues streams~\cite{comp_tersecades,Scabbard}, three additional constraints are enforced as
First and foremost, the compression should be incremental so that processing of the current incoming tuple need not be dependent on the other tuples coming in the future. 
Second, the latency of conducting compression should be as low as possible to avoid the input stream be blocked due to compression and fail to be processed timely. 
Third, memory footprint of compression shall be constant and can not grow rapidly along with the ever-increasing amount of data.
Recent studies have proposed low-latency parallel stream compression algorithms on multicores and GPUs~\cite{comp_tersecades,Scabbard}. 
% However, it is unclear how can those works be applied for parallel stream compression on AMPs.
In this work, we focus on revisiting parallel stream compression on AMPs and further take energy consumption into consideration.
%\xianzhi{stateless/stateful here???}
\end{comment}
% The specific algorithm of lz4, tcomp32 and tdic32 are presented in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of \emph{a segment of code lines} (or \emph{code segment} for short), and the {//} for \emph{a certain line of code} . 
%  the Symmetric Multicore Processors (SMPs) for parallel compression:
% Our experiments have shown that SMPs-aware parallelization results in poor performance on AMPs.

\begin{comment}
\textbf{Choices of Compression Schemes}. Since the 1950s~\cite{comp_huffman}, a lot of methods have been proposed for improving the theoretical compressibility~\cite{comp_7z}, 
reducing compressing complexity on single core~\cite{comp_survey_2017, comp_survey_huffman}, 
accelerating compression~\cite{comp_acc}, and reducing the energy dissipation~\cite{comp_energy_2006} . However, not all of them are applicable for the compression on streaming data, and some of them lack the generality and can only be narrowly applied to specific occasions. For instance, lossy compression methods such as transform coding~\cite{comp_trans} are widely used in multimedia streams (e.g., video frames~\cite{comp_video}), but they will cause unacceptable corruption to the streams of faint yet vital data (e.g., those produced by body area networks~\cite{body_survey}). 

The dictionary compression strategies, 
which operate by searching for
matches between the data to be compressed and a set of strings (also called the vocabularies)
contained in a dictionary, have high level of adaptivity and universality. The well-known examples of them are LZ77~\cite{comp_ziv_lz78}, LZ78~\cite{comp_ziv_lz78} and their extensions such as 7z~\cite{comp_7z}, and lz4~\cite{comp_lz4}. A recent evaluation on stream of Dynamic Vision Sensor (DVS) data~\cite{comp_dvs} proved that dictionary compression, thought as a general way, can even outperform most scenario-specific compression. 

Entropy encoding strategies are also versatile. Unlike the dictionary compression which reorganize vocabularies and take advantage of their duplication patterns, entropy coding tries to make the average code length of symbols as close as possible to the Shannon's entropy, and a symbol can be one single byte (8-bit), word (32-bit), etc. in practice.
While the classic ways like huffman encoding~\cite{comp_survey_huffman} and Arithmetic encoding~\cite{comp_arithmatic} may be costly sometimes in building their code books or calculation, recent approaches such as Finite State
Entropy (FSE)~\cite{comp_fse} can achieve a trade-off between compression ratio and
speed. Besides stand-alone deployment, entropy coding can also be chained after a dictionary compression to achieve better compression ratio. This idea has achieved great success in the well-known Zlib~\cite{comp_zlib} and Zstd~\cite{comp_zstd}.

This paper revisits the dictionary compression and entropy encoding due to their versatility. Moreover, we exploit the fine-grained parallelization to meet stricter latency constraints, and use the AMP-aware core mapping of tasks to be energy efficient. 


\end{comment}


==> Sections/backup/2_Background.tex <==

\section{Background
%\shuhao{why no discussion about the asymmetric communication cost??}
}
\label{sec:background}
%In this section, we introduce modern AMP (especially its asymmetric core communication) and provide an overview of the \compress.



\subsection{Modern AMP}
\label{subsec:amp_intro}
%\textbf{Purposes and Properties}.
%Initially, AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
%AMP was intended to improve energy efficiency and provide higher performance (i.e., by increased area efficiency) from the first beginning~\cite{amp_2003,amp_2004,amp_impacts_2005}.
 %To achieve these goals, AMP has two key characteristics. First, it involves different types of cores~\cite{amp_survey_2016}, which trade off performance with power to different degrees. 
 %Second, the different types of cores are formed within the same instruction set architectures (ISA).
% To reach the goals, there are two key factors of the AMP. First, it involves cores of different types~\cite{amp_survey_2016}, which trade off performance with power to different degrees. Next, the different types of cores are formed within the same instruction set architectures (ISA).
%Therefore, AMP embraces heterogeneity as a first principle, but still have convenient management methods and unified programming models by virtue of identical ISA.

% In this work, we limit our scope to lossless data stream compression. To further extending our work to lossy data stream compression is important but left as a future work.
% \textbf{Principles of \compress}. 
%according existing work in stream~\cite{comp_tersecades} and in-memory database compression~\cite{db_comp0,db_comp1}. 
% \textbf{Algorithms used in this paper}. 
% Data compression is the art of science of representing information in a compact form~\cite{comp_intro_book}, and various compression algorithms have been introduced with diverse trade-offs. 
% Due to the space-saving effect and great compressible space for data at the edge (e.g., the large space and time correlation of sensor data~\cite{comp_wsn}), 

We use the rk3399 processor~\cite{amp_rk3399} as an example to show the architecture characteristics of AMP,
as shown in Figure~\ref{fig:rk3399},
which has three key properties.

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/AMP.pdf}
    \caption{The 6-core AMP rk3399.}  \label{fig:rk3399}   
\end{figure}
%\textbf{Overview}.
%\label{subsec:amp}
%The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}. 

%Figure \ref{fig:rk3399} shows a concrete example of AMP, the rk3399 processor~\cite{amp_rk3399}. Three key properties of AMP can be observed in this processor as listed below. 

\begin{myitemize}
    \item \textbf{Asymmetric cores}. AMP couples different kinds of cores. This design can trade off performance with power to different degrees on the same processor under the same instruction set architectures (ISA). For rk3399, it couples both the in-order A53~\cite{amp_A53ug} cores and out-of-order A72~\cite{amp_A72ug} cores.
    
    \item \textbf{Asymmetric cache-memory structure}. The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the equivalent clock frequency setting.
    In contrast, the micro-architecture and frequency for cores from different \emph{clusters} are not identical.
    For instance, the A53 and A72 cores are placed at \emph{cluster0} and \emph{cluster1}, respectively in rk3399.
    
    \item \textbf{On-chip peripherals}. AMP for embedded systems has many peripherals to complete their embedded tasks (e.g., the I2C and the USB protocols~\cite{amp_i2c}). 
    The peripherals are arranged in unified addressing ways in RISC architectures like ARM~\cite{amp_arm}.
    In rk3399, I2C and other peripherals share the inter connection hardware CCI500~\cite{amp_CCI500} with cores, caches, and memory.
\end{myitemize}

In this paper, we focus on two major AMP effects according to the above properties.

\textbf{Energy reduction and performance improvement}.
The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
Specifically, the core asymmetry of AMP can exploit the fact that applications’ resource
requirements are different. The reason is that both high energy-efficient cores and high-performance cores are integrated on the same processor, and by the same contract between hardware and software. Accordingly, by deciding ``the right kind of core''~\cite{amp_scheduling_2021} to satisfy the application requirements, we can achieve either saving in energy or boosting in speed, and even both of them.
%AMP couples relatively battery-saving and slower cores with relatively more powerful and power-hungry cores within the ISA, which offers a large space for optimization.
%AMP integrates both high energy efficiency cores and high performance cores on the same processor and by the same contract between hardware and software, which offers a large space for optimization.
%The AMP is designed to improve energy efficiency and to provide higher performance (i.e., by increasing area efficiency)~\cite{amp_2003,amp_2004,amp_impacts_2005}.
%Specifically, it exploits the fact that applications’ resource
%requirements are different~\cite{amp_latency_2015} by coupling different kinds of cores which trade off performance with power to different degrees on the same processor\ under the same instruction set architectures (ISA).
%software-hardware contract (e.g., the ARMv8 ISA).
%Thus, by deciding 'the right kind of core'~\cite{amp_scheduling_2021} to satisfy the requirements, we can achieve either saving in energy or boost in speed, and even both of them.
%This is totally different from symmetric multicore processors (SMPs), which must do the trade-off between performance and energy within the same type of cores.
\begin{comment}
\textbf{Applications}. AMP has been gaining much popularity these years~\cite{amp_iot}. Nowadays, top processor vendors like to apply the idea of AMP to build their flag-ship processors for edge and mobile computing: the rk3399(2016)~\cite{amp_rk3399} by Rockchip, the kirin 9000(2020)~\cite{amp_kirin9000} by Hisilicon and the snapdragon 8 Gen 1(2021)~\cite{amp_sd8g1} by Qualcomm; as they can enhance battery life, reduce the cost of cooling and overall improve system’s scalability and reliability in these scenarios specifically. Moreover, the application filed of AMP  will extend to personal computers and even data center, according to Intel's recent release of 12th generation \emph{Core} Processor~\cite{amp_i9_12} and AMD's new plans~\cite{amp_amd}.
\end{comment}

\textbf{Asymmetric core communication}.
%The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. 
The asymmetric   cache-memory   structure of AMP leads to asymmetric core communication.
%Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the same clock frequency setting, while these for cores from different \emph{clusters} are different. 
Following existing work~\cite{amp_partition_2019}, we define 
the communication between cores in the same cluster as \emph{intra-cluster} communication (red lines in Figure \ref{fig:rk3399}), and between cores in different clusters as \emph{inter-cluster} communication~\cite{amp_partition_2019} (blue lines). 
%This kind of organization forms the asymmetry in core communication.
The \emph{intra-cluster} communication can be achieved directly by cache sharing (e.g., L2 cache for rk3399), and it is bidirectional symmetric for the simple bridging of identical cores. The \emph{inter-cluster} communication on the other hand, is much more complicated for two reasons: First, it leads to more overhead, as it is achieved by special inter connection hardware like the CCI500~\cite{amp_CCI500}, which is often much lower than direct cache sharing. Second, it is \textbf{polar}, as data sink core resides at higher performance \emph{cluster} (e.g., core4) has to \emph{wait for} the data source if the source core belongs to a poorer performance \emph{cluster} (e.g., core0). This can increase the total communication overhead in hardware level of \emph{hand-shaking}, \emph{acknowledgement}, and \emph{synchronization}. However, the reverse process, i.e., from core in higher performance \emph{cluster} to core in poorer performance \emph{cluster}, suffers less
in waiting and synchronization, and leads to less overhead. Even worse, frequently addressing the on-chip peripherals can add more uncertainties and overhead to the \emph{inter-cluster} communication. 

%Besides, as the on-chip peripherals or protocols with relative low speed also share the hardware interconnection with the cores, frequently addressing them can add more uncertainties and overhead to the \emph{inter-cluster} communication. 



%The AMP have \emph{clusters} or \emph{cluster-like structures} to organize cores. 


\begin{comment}
\xianzhi{The AMP maintains \emph{clusters} or \emph{cluster-like structures} to organize cores. }
\shuhao{maintains a cluster-like structure?}
%Typically, the same \emph{cluster} have cores under identical micro-architecture and within the same frequency domain, 
\xianzhi{Typically, cores within the same \emph{cluster} follow identical micro-architecture and share the same clock frequency setting, while cores from different \emph{clusters} typically follow different micro-architectures, clock frequency settings or even both.}
\shuhao{Typically, cores within the same follow identical micro-architecture and share the same clock frequency setting?}
%while different \emph{clusters} contain cores different in micro-architecture, frequency domain or even both. 
\shuhao{Typically, cores within the same cluster follow an identical micro-architecture and share the same clock frequency setting, while cores from different clusters typically follow different micro-architectures, clock frequency settings or even both. Nevertheless, those cores share memory subsystem and adopt the same ISA.}
%Therefore \shuhao{Nevertheless?}, 
\xianzhi{Nevertheless,}
the two kinds of asymmetry in core and cache-memory structure are formed within the same ISA. 


\shuhao{those cores share memory subsystem and adopt the same ISA?}
The rk3399 processor~\cite{amp_rk3399} shown in Figure \ref{fig:rk3399} is a concrete example for AMP.

 This processor has two kinds of cores under ARMV8 64-bit ISA: the in-order A53~\cite{amp_A53ug} running under maximum frequency 1.416GHz (core0 to core3)  and the out-of-order (OoO) A72~\cite{amp_A72ug} running under maximum frequency 1.8GHz (core4 to core5), and they are placed in \emph{cluster0} and \emph{cluster1} respectively. The communication between cores in the same cluster (e.g., core0 and core1) is \emph{intra-cluster}, and between cores in different clusters (e.g., core0 and core4) is \emph{inter-cluster}. While the \emph{intra-cluster} communication is carried on directly by shared L2 cache of the \emph{cluster}, the \emph{inter-cluster} communication requires data transferring through the CCI500~\cite{amp_CCI500}, which is a cross-bar inter connection hardware with snoop filter entries for the coherent between \emph{clusters}. 
\shuhao{shows a the rk3399 processor which is a concrete example of AMP. This processor has two kinds of cores under ARMV8 64-bit ISA: the in-order A53 with a maximum frequency of 1.416GHz (core0~core3) and the out-of-order (OoO) A72 with a maximum frequency of 1.8GHz (core4~core5), and they are placed in cluster0 and cluster1 respectively. The  intra-cluster communication is carried on directly by shared L2 cache of the cluster, while the inter-cluster communication requires data transferring through the CCI500, which is a cross-bar inter connection hardware with snoop filter entries for the coherent between clusters.}


The L2-based  \emph{intra-cluster} and the CCI500-based \emph{inter-cluster}  data sharing form the asymmetry of core communication, and they are drawn as red lines and blue lines respectively in Figure \ref{fig:rk3399}.
For the \emph{intra-cluster} communication, it does not need to go through the slower CCI500 so has less overhead, and it is also  without polarity due to its simple bridging of the symmetric cores within the same \emph{cluster}.  The \emph{inter-cluster} communication is on the contrary, with both more overhead and the communication polarity.
 To illustrate the \emph{inter-cluster} communication further, let's now consider an data transferring from core0 (A53) to core4 (A72), and allow both of them to run at maximum
frequency (1.416GHz and 1.8GHz respectively). In this case, core4 will always have to \emph{wait for} core0 due to 1) its higher frequency and 2) its OoO nature with more greedy cache line fetching, which increase the total communication overhead in hardware level of \emph{hand-shaking}, \emph{acknowledgement} and \emph{synchronization}, etc. So this communication process has to \emph{go through the narrow and slower path} in Figure \ref{fig:rk3399}. However, the reverse process, i.e., from core4 to core0, is faster, as slower and less greedy core0 for data sink will lead to less suffering in waiting and synchronization.
\end{comment}

\begin{comment}
The formulation of The asymmetric core communication is demonstrated in subsection \ref{subsec:latency}, and experiments in subsection \ref{sucsec:confirmation} will do the confirmation.


In addition to the cache and memory, AMP for embedded systems have many peripherals to finish their embedded tasks (e.g., the I2C and the USB protocols~\cite{amp_i2c}), and they are arranged in unified addressing ways in some RISC architectures like ARM~\cite{amp_arm}. As these peripherals or protocols with relative low speed also share the hardware interconnection with cores, frequently addressing them can add more uncertainties and overhead to the \emph{inter-cluster} communication. 

\end{comment}


\subsection{Streaming Lossless Compression}
% In this work, we limit our scope to lossless data stream compression. To further extending our work to lossy data stream compression is important but left as a future work.
\textbf{Principles of \compress}. By analyzing existing works, we observe that lossless data stream compression can be achieved  by 1) using \emph{dictionary} to represent the repeated sequence~\cite{comp_lzFamily},   2) cutting off unnecessary bits ~\cite{comp_elias,comp_baseDelta}, and 3) variable length coding approaching the entropy~\cite{comp_huffman}. 
Moreover, the complexity of lossless data stream compression must be \emph{relatively low} within an acceptable time overhead. 
Complicated algorithms like the original huffman encoding or the original LZ77 cannot be applicable,
as discussed in ~\cite{comp_tersecades,db_comp0,db_comp1}.


%according existing work in stream~\cite{comp_tersecades} and in-memory database compression~\cite{db_comp0,db_comp1}. 

\textbf{Algorithms used in this paper}. 
We introduce and adopt three compression algorithms for \compress in this paper as follows. All of them are with relatively low overhead.
We use these algorithms because they are representative and can cover all of the three common approaches for \compress. Furthermore, 
the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.

\begin{myitemize}
    \item \textbf{lz4}~\cite{comp_lz4} is a widely-used  LZ77-based~\cite{comp_lzFamily} compression. It uses a hash table to replace the traditional \emph{dictionary} of LZ77, so it is much faster than LZ77.
    \item \textbf{tcomp32} is a simplification of elias encoding~\cite{comp_elias}, which is already claimed as 'light-weight' in cutting off bits by existing works~\cite{db_comp0}. We change its encoding methods with a fixed length-indicator, so it is more stable in dealing with stream data with more variety.  
    
    \item \textbf{tdic32} is a simplified variable length coding by the hybridization of two above, as it borrows the hash table from lz4 and uses a memory I/O pattern similar to tcomp32 (i.e., per 32-bit single symbol). The frequently-showed symbols are encoded with their hash index (which is always shorter). Those not found in hash table are  encoded by their original values together a one-bit indicator (which means longer encoding).  
\end{myitemize}

%The specific algorithm of lz4, tcomp32 and tdic32 are presented in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of \emph{a segment of code lines} (or \emph{code segment} for short), and the {//} for \emph{a certain line of code}. These algorithms are representative enough for this work, as they cover all of the three common approaches for \compress. Therefore, the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.

\textbf{AMP-aware opportunity}.
 None of existing work has parallelized \compress on AMP, though this combination is feasible and can achieve significant reduction in time and energy overhead. 
 %\xianzhi{extend this part?}
 On the one hand, \compress involves varying data transformation (e.g., replace a data sequence by its \emph{lz4 token}) and memory addressing (i.e., read and write data by aligned or unaligned memory I/O), which leads to diverse ILP and MLP among different algorithms, and even within the same one.
 According to existing work in parallelization~\cite{comp_paralz_2013,comp_lzss_cuda}, it can be further accelerated by TLP (i.e., by running multiple threads which only handle a part of the whole data). On the other hand, the \textbf{a}symmetric cores in AMP provide flexible support to optimize the execution for different ILP and MLP, and the  
  \textbf{m}ulticores in AMP can directly support the TLP. The rest part of this paper can illustrate how to achieve the combination and optimization.


\begin{comment}
\subsection{Data Compression}
\label{subsec:dc_intro}
% In this work, we limit our scope to lossless data stream compression. To further extending our work to lossy data stream compression is important but left as a future work.
% \textbf{Principles of \compress}. 
%according existing work in stream~\cite{comp_tersecades} and in-memory database compression~\cite{db_comp0,db_comp1}. 
% \textbf{Algorithms used in this paper}. 
Data compression is the art of science of representing information in a compact form~\cite{comp_intro_book}, and various compression algorithms have been introduced with diverse trade-offs. Due to the space-saving effect and great compressible space for data at the edge (e.g., the large space and time correlation of sensor data~\cite{comp_wsn}), compression is popular in edge computing applications like cloud offloading~\cite{comp_mobile_vm}, vehicle trajectory~\cite{comp_vechiel}, wireless sensor networks~\cite{comp_wsn,comp_wsn2}, etc. 
Nevertheless, the costly nature of data compressing is not ignorable, especially in edge computing. and significant interest have been created in accelerating it.

Significant interest have been created in accelerating compression, and 
parallelization is an effective way for the acceleration. Parallel data compression has been widely deployed at earlier VLSI~\cite{comp_1985}, FPGA~\cite{comp_lz4_fpga}, symmetric multicore processor (SMP)~\cite{comp_para_bzip2} and GPU~\cite{comp_pipeline_gpu,comp_lzss_cuda}. However, none has ever considered the special asymmetry and energy-efficiency nature of AMP.

The \emph{streaming lossless compression (\compress)} has been widely adopted in modern stream applications~\cite{comp_tersecades}. 
\compress reduces computational workloads and memory footprints without affecting the accuracy of results. 
Different from traditional batch-based compression algorithms, \compress needs to compress data as soon as they arrive. 
The costly nature of data compressing and the stringent response time requirements have created significant interest in accelerating \compress and reducing its energy dissipation.


We select three %representative
compression algorithms to parallelize on AMP in our work, and they are of relatively low overhead for edge computing.
% We use these algorithms because they are representative and can cover all of the three common approaches for \compress. Furthermore, 
Nevertheless, our framework can be easily extended to support other compression algorithms.
% the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.

\begin{myitemize}
    \item \textbf{lz4}~\cite{comp_lz4} is a widely-used  LZ77-based~\cite{comp_lzFamily} compression. It uses a hash table to replace the traditional \emph{dictionary} of LZ77, so it is much faster than LZ77.
    \item \textbf{tcomp32} is a simplification of elias encoding~\cite{comp_elias}, which is already claimed as 'light-weight' in cutting off bits by existing works~\cite{db_comp0}. We change its encoding methods with a fixed length-indicator, so it is more stable in dealing with stream data with more variety.  
    \item \textbf{tdic32} is a simplified variable length coding by the hybridization of two above, as it borrows the hash table from lz4 and uses a memory I/O pattern similar to tcomp32 (i.e., per 32-bit single symbol). The frequently-showed symbols are encoded with their hash index (which is always shorter). Those not found in hash table are  encoded by their original values together a one-bit indicator (which means longer encoding).  
\end{myitemize}

\begin{comment}
    for two reasons: First, it leads to more overhead, as it is achieved by special inter connection hardware like the CCI500~\cite{amp_CCI500}, which is often much lower than direct cache sharing. Second, it is \textbf{polar}, as data sink core resides at higher performance \emph{cluster} (e.g., core4) has to \emph{wait for} the data source if the source core belongs to a poorer performance \emph{cluster} (e.g., core0). This can increase the total communication overhead in hardware level of \emph{hand-shaking}, \emph{acknowledgement}, and \emph{synchronization}. However, the reverse process, i.e., from core in higher performance \emph{cluster} to core in poorer performance \emph{cluster}, suffers less
    in waiting and synchronization, and leads to less overhead. Even worse, frequently addressing the on-chip peripherals can add more uncertainties and overhead to the \emph{inter-cluster} communication.
\end{comment}

We present the specific algorithm of lz4, tcomp32 and tdic32 in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of an algorithm \emph{component} which has several lines of code, and the {//} for \emph{a certain line of code}.
%The specific algorithm of lz4, tcomp32 and tdic32 are presented in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of \emph{a segment of code lines} (or \emph{code segment} for short), and the {//} for \emph{a certain line of code}. These algorithms are representative enough for this work, as they cover all of the three common approaches for \compress. Therefore, the methods to parallelize them with energy efficiency in this paper can be easily extended to other \compress algorithms.
\end{comment}

==> Sections/backup/2___20220108.tex <==
\section{Background and Motivation}
\label{sec:background}
%\shuhao{In this section, xxx}
% we first introduce the \shuhao{basic notations and assumptions} of data compression, followed by the discussion of characteristics of modern AMPs.
In this section, we first introduce the characteristics of modern AMPs, followed by 
basic notations and assumptions of parallel data compression on AMP.


\subsection{Asymmetric Multicore Processors}
\label{subsec:amp_intro}
The AMPs are designed to improve energy efficiency or increase area efficiency~\cite{amp_2003,amp_2004,amp_impacts_2005}, and they can trade off performance with power to different degrees. Figure~\ref{fig:rk3399} shows the architecture of a recent AMP processor ,rk3399~\cite{amp_rk3399}.
In the following, we summarize two important asymmetry properties of AMPs, including both cores and communications. We also present the corresponding specific indicators in Table~\ref{tab:asymmetry}. 

\textbf{Asymmetric Cores.} 
To organize cores, the AMPs maintain a cluster-like structures s~\cite{amp_survey_2016}.  
Cores within the same \emph{cluster} follow identical micro-architecture and share the equivalent clock frequency setting.
For instance, the rk3399 consists both the relatively batter-saving and slower A53 cores (also called ''little core'')~\cite{amp_A53ug} at cluster 0 and more powerful and power-hungry A72 cores (also called ''big core'')~\cite{amp_A72ug}  at cluster 1. 
According to existing researches on modeling and utilizing AMP~\cite{amp_impacts_2005,amp_modeling,amp_scheduling_2021,amp_pie_2011}, %\xianzhi{software with high ILP and high MLP favor more of the big cores in different degrees}, 
big cores are suitable to support software with high ILP and high MLP,
while the little cores often provides more thread parallelism. Besides, the cores share the same ISA (i.e., the ARM v8 ISA~\cite{amp_armv8} for rk3399) despite the asymmetry.
%高ILP和MLP都更加喜欢大核，但程度不同 （如果不强调程度不同就会被reviewer怼：为什么ILP和MLP不统统丢给大核？）
%先用software这个笼统的词，因为task在2.2才定义
\begin{figure}
    \centering
    \includegraphics*[width=0.35\textwidth]{figures/AMP.pdf}
    \caption{The 6-core AMP rk3399.}  \label{fig:rk3399}   
\end{figure}

\textbf{Asymmetric Communication.}
%just follow existing work and use the inter/intra cluster
%\xianzhi{
There are two kinds of core communication in AMP~\cite{amp_cluster_2021,amp_partition_2019}, i.e.,  \textbf{intra-cluster} and \textbf{inter-cluster} communication.
The \textbf{intra-cluster} communication is the direct sharing of L2 cache for cores within the same cluster, while \textbf{inter-cluster} communication represents that cores from different clusters go through a much slower interconnection link.
%}
%Cores within the same cluster share L2 caches, while the communication between cores from different clusters go through a much slower inter connection link. 
Therefore, access latency varies depending on whether a
core is accessing a ``local'' or ``remote'' cache. Specifically, we use different lengths of \emph{c0}, \emph{c1} and \emph{c2} to indicate the different latency in Figure~\ref{fig:rk3399}.
This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
%\xianzhi{
However, the \emph{inter-cluster} communication is more complicated than the socket link in NUMA, because it bridges asymmetric cores instead of symmetric cores. On the one hand, it leads to \emph{more communication overhead}, as the inter connection hardware is slower than L2 sharing. On the other hand, it is \emph{of polarity}.
%从高端到低端的过程比其逆过程的代价要大
Specifically, the communication cost 
%in
''from poorer performance source to higher performance sink ''(i.e., c2) is always larger than its reverse process (i.e., c1) . This is because the extra waiting of a higher performance sink for its source increases the \textbf{synchronization} and \textbf{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.  
%}
\begin{table}[]
\centering
\caption{Specific indicators of the asymmetry, the unit of latency is ''ns per 32-bit access''}
\label{tab:asymmetry}
\resizebox{.85\columnwidth}{!}{%
\begin{tabular}{|L{2cm}|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Asymmetric\\  cores\end{tabular}}        & \textbf{Type} & \textbf{L1 cache size}   & \textbf{Pipeline} \\ \cline{2-4} 
 & A72 & 48K I+ 32 K D                 & in-order     \\ \cline{2-4} 
 & A53 & 32K I+ 32K D                  & out-of-order \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Asymetric\\  communication\end{tabular}} & \textbf{Path} & \textbf{Description} & \textbf{Latency}  \\ \cline{2-4} 
 & c0  & intra-cluser                  & 4.4          \\ \cline{2-4} 
 & c1  & inter-cluster, cluster 1 to 0 & 8.9          \\ \cline{2-4} 
 & c2  & inter-cluster, cluster 0 to 1 & 26.3         \\ \hline
\end{tabular}%
}
\end{table}

\subsection{Parallel Data Compression on AMPs}
\label{subsec:dc_intro}
Compression reduces computational workloads and memory footprints, and is particularly important in edge computing applications like cloud offloading~\cite{comp_mobile_vm}, vehicle trajectory~\cite{comp_vechiel}, wireless sensor networks~\cite{comp_wsn,comp_wsn2}, etc. 
However, parallelizing data compression on edge devices with AMPs is non-trivial due to the aforementioned asymmetry properties.
 
\begin{comment} 
\shuhao{
First, the various ILP and MLP contribute to different task-core affinities. Instead of performing the entire compression on the same type of core(s), 
we execute different \emph{components} on different types of cores for both energy and performance concerns.
Therefore, an equal and black-box view of compression   such as~\cite{comp_para_bzip2,comp_lzss_cuda} is inappropriate.
We should consider it in a more fine-grained manner.
} 
\end{comment}

%\xianzhi{
First, the asymmetric cores make the equal and black-box view of compression in existing works (such as~\cite{comp_para_bzip2,comp_lzss_cuda}) insufficient on AMP. Specifically, even different parts of the same compression algorithm consist of different ILP and MLP,
which leads to varying software-hardware affinities, as discussed in Section~\ref{subsec:amp_intro}. 
Failing to place the compression at the right cores can incur both performance degradation and energy dissipation.
%Failing to place the compression at right cores, both performance lose and energy dissipation will incur.
%}

%\xianzhi{
Second, the asymmetric communication increases the difficulty of meeting the latency constraint. Parallel compression requires multiple cores, 
which requires both {inter-cluster} and {intra-cluster} communication. 
 Despite the ease of intra-cluster communication (which is nearly identical to core communication on SMPs), inter-cluster communication is complex, as discussed in Section~\ref{subsec:amp_intro}. 
%高端核的额外等待会增加硬件上的同步与握手开销
If we are unable to modelize and estimate the asymmetric communication well for fine-grained scheduling, especially {inter-cluster} communication, there can be frequent time-outs. Unfortunately, existing works~\cite{amp_partition_2019,amp_cluster_2021} only investigate inter-cluster communication for task switching in toperating systems, with no modeling of its polarity in parallel structures.
%只管了任务调度时的额外开销，没管并行结构中的极性
%}


\begin{comment}
\shuhao{
Second, as data sink core that resides at higher performance \emph{cluster} (e.g., core4) has to \emph{wait for} the data source if the source core belongs to a poorer-performance \emph{cluster} (e.g., core0). This can increase the total communication overhead in hardware level (e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}) of \emph{hand-shaking}, \emph{acknowledgement}, and \emph{synchronization}. However, the reverse process, i.e., from core in higher-performance \emph{cluster} to core in poorer-performance \emph{cluster}, suffers less in waiting and synchronization, and leads to less overhead.
}
\end{comment}
\subsection{\design Overview}
\label{subsec:overview}
We propose a novel framework to parallelize data compression algorithms, called \design, which is specifically designed for AMPs at the edges. The key of \design is to empower parallel compression with asymmetry awareness and address the two challenges discussed in Section~\ref{subsec:dc_intro}.  In \design, the following concepts are introduced for parallel compression on AMP:
1)
\textbf{job}
, which is to compress a specific
piece of data (batched or continuous tuples) under specific
algorithm within a given cutting-off latency.
2) \textbf{task}, which is a fine-grained execution unit of the {job} on a specific AMP core. A task conducts a \emph{true subset} (i.e., only partial) of the job's whole function, and processes a \emph{subset} (i.e., either full or partial) of the whole input data. 3) \textbf{scheduling plan}
is
a list of
tasks
, that covers all the algorithms and all the data of a
job.
Specifically, \design parallelizes compression jobs and determines the optimal scheduling plan, with the goal of minimizing energy consumption while satisfying the latency constraint. It works under the flow depicted in Figure~\ref{fig:wf}.
\begin{comment}
For illustration, we use \emph{tcomp32} as a running example throughout the paper, which is a simplification of elias encoding~\cite{comp_elias}, and we change its encoding methods with a fixed length-indicator for more stability in dealing with data with more variety. 
Algorithm~\ref{alg:tcomp32} illustrates the implementation of this algorithm. 
\shuhao{Note that, we can abstract the algorithm into three steps: xxx.}
\xianzhi{
Note that, three major steps are involved in the tcomp32 algorithm: read symbol (Line~\ref{algo:tcomp32_read}), encoding function (Line~\ref{algo:tcomp32_encode} to~\ref{algo:tcomp32_encodeEnd}), and write encoded (~\ref{algo:tcomp32_write} to~\ref{algo:tcomp32_writeEnd}), as ''/**/'' style of comments indicate.
These steps are also typical patterns of other compression algorithms like the lz4~\cite{comp_lz4}.
}
\end{comment}

\begin{figure}[t]
    \centering
    \includegraphics*[width=0.75\columnwidth]{figures/system.pdf}
    \caption{The \design system.}  \label{fig:sys}   
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics*[width=0.75\columnwidth]{figures/workFlow.pdf}
    \caption{The workflow of \design. 
    %\shuhao{Make this figure more specific to tcomp32. See my following descriptions accordingly.}
    }  
    \label{fig:wf}   
\end{figure}
%Figure~\ref{fig:wf} shows an example workflow of \design to parallelize a compression job, i.e., compressing a batch of data using \emph{tcomp32}. A user-specified processing latency of 3 seconds is given as the constraint. Subsequently, \design tries to parallelize this compression job minimizing energy consumption while satisfying the latency constraint.
%tcomp32 (Algorithm~\ref{alg:tcomp32})   &  Line~\ref{algo:tcomp32_read}   &  Line~\ref{algo:tcomp32_encode} to~\ref{algo:tcomp32_encodeEnd}  & Line~\ref{algo:tcomp32_write} to~\ref{algo:tcomp32_writeEnd}  \\ \hline

%\xianzhi{
First, 
we apply fine-grained job decomposition to exploit both task pipeline and data parallelism during compression.
%fine-grained job decomposition is applied to exploit both task pipeline and data parallelism during compression.
Specifically, the algorithm and data of jobs can be decomposed into tasks running simultaneously. The tasks under series connection form a pipeline with stages, while those under parallel connection achieve data parallelism by acting as replicas in a stage. Considering various core mapping strategies, we have multiple possible {scheduling plans}, i.e., the lists of tasks, with latency and energy remaining to be estimated.
%}


\begin{comment}
\begin{table}[t]
\centering
\caption{A template \emph{scheduling plan} of parallel tcomp32}
\label{tab:tcomp32_plan}
\resizebox{.5\columnwidth}{!}{%
\begin{tabular}{|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
 \emph{Task} & <\emph{stage},\emph{replica}> & Core \\ \hline
0 & <0,0> & 0    \\ \hline
1 & <0,1> & 1    \\ \hline
2 & <1,0> & 4   \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}
%Specifically, the whole compression decomposed into three independent \emph{stages} namely $s0$, $s1$ and $s2$, and each \emph{stage} contains one and only one step. A pipeline is formed by $s0$ to $s2$ therefore. The costly \emph{stage}, i.e., $s1$ for encoding function, is further replicated into multiple \emph{replicas}, processing subsets of inputs concurrently. We further define a \emph{task} as "\emph{mapping} a certain \emph{replica} of a certain \emph{stage} to a certain AMP core", and multiple lists of \emph{tasks} are created for the whole decomposition due to varying core-mapping ways. Each list here is a possible \emph{scheduling plan}, with latency and energy remain to be estimated. 

\begin{comment}
\shuhao{
First, 
fine-grained job decomposition is applied to exploit both task pipeline and data parallelism during compression. 
Specifically, the compressing steps of read symbol (Line xxx), encoding function (Line xxx), and write encoded (Line xxx) are decomposed into three independent tasks forming as a pipeline. The read symbol task is heavy and is further replicated into multiple replicas, processing subsets of inputs concurrently.
}

\shuhao{
Second, 
we determine the optimal way of scheduling each replica to AMPs, by the guidance of an asymmetry-aware cost model. Specifically, this scheduling procedure evaluates energy consumption and execution latency for each plan and takes the latency constrain 3s into consideration.
----
@xianzhi: Merge the following paragraphs and tables into "Second, we xxx".
----
Because of its \textbf{a}symmetry,
the AMP can provide flexible support for data compression with different ILP and MLP,
and it can also extend the TLP via \textbf{m}ulticores. 
Fine-grained adaptation to different ILP and MLP (i.e., multiple \emph{stages} in parallel compression) requires the synthetic use of both big cores and little cores, which means that \emph{inter-cluster} communication is unavoidable. 
As a result,
accurate modeling and prediction of the \emph{inter-cluster} communication are needed, especially when the trade-off between energy and latency is present. 
To the best of knowledge, 
existing works~\cite{amp_partition_2019,amp_cluster_2021} study the \emph{inter-cluster} communication only for task switching in OS, and lack modeling of its polarity in pipeline structures.
On the contrary, we address this polarity in our cost model in Section~\ref{subsec:elc}. For the confirmation, we also present the latency overhead of \emph{inter-cluster} communication from core0 to core4 of rk3399 and its reverse process in  Appendix~\ref{appendix:polar}
}
\end{comment}

%\xianzhi{
Second, 
we determine the \emph{optimal} {scheduling plan} with the guidance of an asymmetry-aware cost model. Specifically, this scheduling procedure evaluates energy consumption and execution latency for each plan and takes the latency constraint into consideration. 
The basis of the cost model is the ILP and MLP of {tasks}, which determine the affinity of {tasks} on asymmetric cores in both execution latency and energy consumption. Due to the varying ILP/MLP of {tasks} , synthetic use of both big cores and little cores is 
common
%frequent
for the best core mapping of {tasks}.
%经常出现综合利用大小核的情况
This phenomenon means that {inter-cluster} communication is unavoidable, especially when the trade-off between energy and latency is present. To address the complex latency pattern ( as introduced in~\ref{subsec:amp_intro}) of doing so, we model {inter-cluster} communication, especially with polarity, in Section~\ref{subsec:elc}.
%A little unwell, modify sec 3 and pictures tomorrow morning
%}

==> Sections/backup/3-20220108.tex <==
\section{Fine-Grained Parallel Compression} % of Compression Job
In this section, we illustrate the principles of job decomposition, and then demonstrate the practice through a running example.
\label{sec:decompos}
\subsection{Principles of Decomposition}
The purpose of decomposition is to create opportunities for the best task-core affinity and make the most of multiple cores on AMPs. Specifically, we consider both pipelining and data parallelism as follows.
\label{subsec:decomp_principle}

\textbf{Pipeling Parallelism.} 
Data compression is \emph{the art of science of representing information in a compact form}~\cite{comp_intro_book}, and it typically consists of three stages as 1) read input data (i.e., in so-called \emph{symbol(s)}), 2) encode data to the specific \emph{compact form} and 3) write output data. These stages usually contain different functions to conduct, and consist of different ILP and MLP. For instance, arithmetic computation for encoding data contains more ILP than a simple and byte-aligned data reading. 
Hence, they should be independently placed at asymmetric cores for performance boosts or energy reduction, as we discussed in Section~\ref{subsec:amp_intro}. If the individually mapped stages were also executed in parallel, we would have a speed-up pipeline along with more \emph{fine-grained} exposure of task-core affinity.
There is an insightful idea to further divide each stage and form a deeper pipeline, which can theoretically increase the speed-up further. However, this is not suitable for the compression algorithms that are \emph{simple} or \emph{light-weight} themselves, as extra communication overhead between \emph{too many} fine-grained stages can even eliminate the acceleration and increase energy dissipation.

%Besides, a too much deep pipeline is also unfit for the edge devices, which have only limited amount of cores. 
%In a word, there are two major aspects for pipelining compression on AMP: 1) to sufficiently expose ILP and MLP and 2) to limit the communication overhead.

\textbf{Data parallelism.}
A perfectly balanced pipeline is hard to achieve, and there are usually bottleneck stages that limit the whole speed-up. To alleviate this problem, we can duplicate partial {stages} into multiple {replicas}, and each replica will only process a subset of input data. 
 The \textbf{\emph{RLAS optimization}} in existing work~\cite{sp_briskstream} is an effective and automatic method for generating {replicas} in NUMA machines~\cite{numa_2000}, and
it is also applicable to AMP, as there are also multiple single-ISA cores in AMP. 
\subsection{Practice of Decomposing}
\label{subsec:decom_practice}
\begin{algorithm}[t]
\caption{tcomp32 algorithm}
\label{alg:tcomp32}
\scriptsize
\LinesNumbered 
\KwIn{input array $inData$}
\KwOut{output array $outData$}
\While{not reach the end of $inData$} {
\tcc{(s0) read input data}
  $number \leftarrow read \ next \ 32-bit from \ inData$ \label{algo:tcomp32_read}\;
\tcc{(s1) encode data to the tcomp32-specific \emph{compact form} }

\eIf{ $number$ = 0 {\label{algo:tcomp32_encode}}}  
{
   $n\leftarrow 1$ \;
}
{
   $n \leftarrow$ ceil(log2($number$+1)) \label{algo:tcomp32_encodeEnd}\;
    \tcp{e.g., $n$=2 for $number$=3} 
}
 \tcc{(s2) write output data}
    write 5-bit $n-1$ to $outData$ \label{algo:tcomp32_write}\;
    write $n$-bit $number$ to $outData$ \label{algo:tcomp32_writeEnd}\;  
}
\end{algorithm}
We use \emph{tcomp32} as a running example to show the practice of decomposing. 
 The tcomp32 is a simplified version of the elias encoding~\cite{comp_elias}, and we have changed its encoding methods to use a fixed length-indicator for greater stability when dealing with more diverse data.
 %The tcomp32 is a simplification of elias encoding~\cite{comp_elias}, and we change its encoding methods with a fixed length-indicator for more stability in dealing with data with more variety. 
Algorithm~\ref{alg:tcomp32} illustrates the implementation of this algorithm.  
%Note that, we divide tcomp32 into three major stages (namely $s0$, $s1$ and $s2$) as discussed in Section~\ref{subsec:decomp_principle}, and they are indicated in ''/**/'' style of comments. Specifically, the $s0$ to $s2$ of tcomp32 have varying ILP/MLP characteristics, and we use the ARM v8 ISA for the instruction level illustration as follows.
%就是从CPU指令的角度分析一下

%tcomp32
Line~\ref{algo:tcomp32_read} is the first stage $s0$,
and it is just about loading 32-bit aligned data, which involves a relatively small number of instructions. Most of the instructions are for memory addressing (i.e., the {LDR} instruction). Therefore, most processor cycles in $s0$ are spent waiting for long-latency memory operations to complete instead of running computational work. By the definition of~\cite{amp_pie_2011,amp_ILP2}, this is a typical MLP-leading {stage}.


Line~\ref{algo:tcomp32_encode} to~\ref{algo:tcomp32_encodeEnd} is the next stage $s1$. It computes the integer $log2$, which involves a larger number of instructions since the $log2$ should be conducted during several loops of computation. At this {stage}, there are nearly no memory addressing instructions as the input data and middle value have been loaded to registers, which means much lower MLP compared with $s0$. However, because many arithmetic and shift instructions, such as ADD or LSR, are involved in operating registers, ILP takes the lead in this stage.
%However, many arithmetic and shift instructions like {ADD} or {LSR} are involved to operate registers, which make this {stage} leading by ILP.

Line~\ref{algo:tcomp32_write} to~\ref{algo:tcomp32_writeEnd} is the last stage $s2$, which
is an unaligned I/O with medium amount of instructions compared with $s0$ and $s1$. For each byte-unaligned data to write, it involves 1) logical and shift operations in register(s), such as {AND, OR, LSR} and {LSL}. 2)update the memory content with register data, by  {LDR} and {STR} operation. 3) update the memory pointer by {ADD} or {SUB} operation. These three parts have nearly the same density of instructions. Two of them, i.e., 1) and 3), is only about arithmetic/logical operation, while the 2) involves memory addressing. Taking all of them into account, the $s2$ is still ILP-leading, though not such significant as $s1$.

 These three {stages} with different ILP/MLP can be executed in parallel smoothly,
 as there is no variable written by multiple stages at the same time (i.e., which leads to
 cross \textbf{data dependency}~\cite{comp_para_lz77_gpu} ). However, the communication overhead between $s0$ and $s1$ is nearly the same as the stand-alone running overhead of $s0$, so we need to emerge $s0$ and $s1$ as Section~\ref{subsec:decomp_principle} stressed, and then construct the tcomp32 pipeline as Figure~\ref{fig:tcomp32_stage} depicts. It is worth noting that the new 'stage 0' is still ILP-leading as the previous $s1$ is more decisive than $s0$, and the new 'stage 1' is just the same as the former $s2$. Further, due to the high instruction density of new 'stage 0', which is the bottleneck, we can duplicate it as demonstrated in Figure~\ref{fig:tcomp32_replica}.


\begin{figure}[h]\shuhao{1. Never use [h]. 2. Remove this figure and the corresponding texts as you are running out of space. 3. If you can shorten 3.2, you may merge 3.1 and 3.2, and use 3.2 as just short paragram of an example. Learn from https://www.comp.nus.edu.sg/~hebs/pub/icde20-tstream.pdf Section II-A.}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/tcomp32_pipe.pdf}
    \caption{The tcomp32 pipeline.}  \label{fig:tcomp32_stage}   
\end{figure}

\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/tcomp32_replica.pdf}
    \caption{The final decomposition of tcomp32.}  \label{fig:tcomp32_replica}
\end{figure}

 %Returning to the concrete cases,
 %we show the relationship between \emph{stages} and algorithm lines for lz4, tcomp32, and tdic32 in Table~\ref{tab:lc_steps}.
 

In this way, we can provide flexible support for different ILP and MLP within the same compression algorithm,
and extend the parallelism by executing {repicas} on multiple cores in parallel. 
However, the question of how to appropriately arrange {tasks} (i.e., map the stages and replicas to AMP cores) and form the optimal {scheduling plan} is still to be answered. And we continue to solve it with our asymmetry-aware scheduling in Section~\ref{sec:costmodel}.

\begin{comment}
\begin{table}[h]
\caption{Fine-grained stages of concrete \compress algorithms}
\label{tab:lc_steps}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
        & $s0$ & $s1$ & $s2$ \\ \hline
lz4 (Algorithm~\ref{alg:lz4})           &  Line~\ref{algo:lz4_read}  & Line~\ref{algo:lz4_encode} to~\ref{algo:lz4_encodeEnd}   & Line~\ref{algo:lz4_write}   \\ \hline
tcomp32 (Algorithm~\ref{alg:tcomp32})   &  Line~\ref{algo:tcomp32_read}   &  Line~\ref{algo:tcomp32_encode} to~\ref{algo:tcomp32_encodeEnd}  & Line~\ref{algo:tcomp32_write} to~\ref{algo:tcomp32_writeEnd}  \\ \hline
tdic32  (Algorithm~\ref{alg:tdic32})    &  Line~\ref{algo:tdic32_read}  & Line~\ref{algo:tdic32_encode} to~\ref{algo:tdic32_encodeEnd}   &  Line~\ref{algo:tdic32_write}   \\ \hline
\end{tabular}%
}
\end{table}
\begin{table}[h]
\caption{Leading factors of different algorithm components.}
\label{tab:lc_factors}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
 \diagbox{Algorithm}{Leading Factor}{Component}        & read symbol(s) & encoding function & write encoded \\ \hline
lz4 & MLP & MLP & MLP   \\ \hline
tcomp32 & MLP & ILP & ILP   \\ \hline
tdic32 & MLP & MLP & ILP   \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}

==> Sections/backup/3_Decom.tex <==

\section{The Fine-grained Decomposition}
\label{sec:problem}
\label{sec:lib}
 %In this section, we first introduce the fine-grained steps of parallel \compress. Then, we discuss the parallelization of these steps as \emph{tasks}. Next, we illustrate the implementation of the library. 
 %Finally, we give a formal definition of our research problem. 
%\subsection{Fine-grained Stages in Lossless Data Stream Compression}
In this section, we introduce our motivation, terminologies and library design for the fine-grained decomposition of compression algorithms.
\label{subsec:PLSC}
\subsection{Motivation}
We present the specific algorithm of lz4, tcomp32 and tdic32 in Algorithm \ref{alg:lz4}, \ref{alg:tcomp32},\ref{alg:tdic32} respectively. Noting that we use the {/* */} style of comments to identify the purpose of an algorithm \emph{component} which has several code lines, and the {//} for \emph{a certain line of code}.
By analysing the algorithm details of them, we can find these three algorithms have differences in following two aspects.
\begin{myitemize}
    \item \textbf{The instruction density} (or ILP). The tcomp32 is most instruction-bound among the three, as it requires both arithemetic calculation and the \emph{AND/OR} operation\mynote{ Which is caused by unaligned I/O}. The tdic32 is less as it doesn't require too much math calculation, while lz4 is the least as it requires neither compound math calculation nor unaligned I/O.
    \item \textbf{The memory access density} (or MLP). The lz4 is most memory-bound due to its hash tabling and \emph{looking-back} search, tdic32 is less as it doesn't have to back search the memory, and tcomp32 is the least as it has neither.
\end{myitemize}

Moreover, even different \emph{components} within the same algorithm can have different leading factor in terms of ILP or MLP (i.e., have different density in instruction and memory access), as we listed in Table \ref{tab:lc_factors}. Taken the tcomp32 in Algorithm \ref{alg:tcomp32} for instance. It's \emph{encoding function} (Line \ref{algo:tcomp32_encode} to \ref{algo:tdic32_encodeEnd} )  is more ILP-leading and less MLP-leading than the \emph{write encoded}  (Line \ref{algo:tcomp32_write} to \ref{algo:tcomp32_writeEnd} ), due to the $log2$ computing in \emph{encoding function}.


\begin{table}[h]
\caption{Leading Factors of Algorithm Componets}
\label{tab:lc_factors}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
 \diagbox{Algorithm}{Leading Factor}{Component}        & read symbol(s) & encoding function & write encoded \\ \hline
lz4 & MLP & MLP & MLP   \\ \hline
tcomp32 & MLP & ILP & ILP   \\ \hline
tdic32 & MLP & MLP & ILP   \\ \hline
\end{tabular}%
}
\end{table}
%Taken the tcomp32 in Algorithm \ref{alg:tcomp32} for instance. It's \textbf{\emph{encodingFunction}} (Line \ref{algo:tcomp32_encode} to \ref{algo:tdic32_encodeEnd} ) segment is more instruction-bound and less memory-access-bound than the \emph{write encoded data} segment (Line \ref{algo:tcomp32_write} to \ref{algo:tcomp32_writeEnd} ).

\begin{comment}
According to subsection \ref{subsec:LC_algo}, a more exhaustive decomposition of \compress algorithm lead to higher level of task-core affinity awareness, and then result in better parallel execution.
\end{comment}

The different ILP and MLP contribute to different task-core affinities. According to the existing works on AMP~\cite{amp_impacts_2005,amp_modeling,amp_scheduling_2021}, high ILP will generally benefit more from the OoO big cores than high MLP, vice versa. Instead of running the whole  on the same type of core(s), it may be much better to execute different \emph{code segment} at different types of cores for both energy and performance concern.
%\shuhao{how?},\
Therefore, a black-box view of compression in OS as \emph{threads} is inappropriate, and we should have a \emph{per-component} view of it. 
\subsection{Terminologies}

\begin{algorithm}[h]
\caption{Abstract compression algorithm with stages}
\label{alg:LC}
\LinesNumbered 
\KwIn{input array $inData$}
\KwOut{output array $outData$}
$toEncode \leftarrow initial \ value$ \;
\While{not reach the end of $inData$}
{
    (s0) read symbol or symbols \label{algo:lcA_S0} \;
    (s1)\emph{encoding function} \label{algo:lcA_S1}\;
    (s2) write encoded \label{algo:lcA_S2}\;
}

%\newpage
\end{algorithm}
\textbf{Job}. We define the users' requirement of \emph{'compress specified data under specified algorithm within specified latency'} as a compression \emph{job}. 

\textbf{Stage}. We summarize the common component of the lz4, tcomp32 and tdic32 as Algorithm \ref{alg:LC} \mynote{Noting if there are extra data structure like hash table, code-book or state machine, etc., we assume they are initialized before compression and will be updated during the \emph{encoding function}}. In this abstraction, compression can be viewed as multiple series of
data-parallel \emph{stages} written as $s0$, $s1$ and $s2$, and each \emph{stage} contains one and only one algorithm component. The \emph{stages} form a pipeline as Figure \ref{fig:chain} depicts.
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/fstages.pdf}
    \caption{The pipeline of $s0$, $s1$ and $s2$ .}  \label{fig:chain}   
\end{figure}

\textbf{Replica}. To speed-up the pipeline of \emph{stages}, some bottleneck \emph{stage} can be duplicated into several \emph{replicas}, and each one only handles a subset on input data.

\textbf{Task}. A \emph{task} is to map a certain \emph{replica} of a certain \emph{stage} at a certain AMP core, for the real execution.

\textbf{Scheduling Plan}. We define one \emph{scheduling plan} as the list of \emph{tasks}, which covers all \emph{stages} and all \emph{replicas} of the decomposition. Due to the various core mapping ways, there are more than one possible \emph{scheduling plans} in one decomposition.

\subsection{Library Design}
We design the fine-grained decomposition of lz4, tcomp32, and tdic32 as a C++-20 style library, which enables following features.
\begin{myitemize}
    \item \textbf{Stage Emerging}. There may be some cross-reference between \emph{stages}, like the {$bytePoninter$} variable in $s0$ and $s1$ of lz4. To overcome the complexity of addressing it, we can simply emerge the \emph{stages} with cross-reference as one \emph{stage}.
    \item \textbf{Sleep-awake mechanism}.  All \emph{stages} will only be \emph{awake} when \emph{there is} data to handle, otherwise, they will \emph{sleep} to reduce energy dissipation.
    \item \textbf{Automatic Generation of Replicas}.
    We adopt the RLAS algorithm from existing work~\cite{sp_briskstream}. The RLAS can analyse
    the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} without 
    manual intervention.  
    \item \textbf{Extensibility}. We make the most of the \emph{C++ Class}, and the library can be easily extend to support other compression algorithms through inheritance and derivation.
\end{myitemize}



==> Sections/backup/4-20220108.tex <==
\section{Compression Task Scheduling on AMPs}
\label{sec:costmodel}
\xianzhi{Grammar here}
%without formulation
%In this section, we introduce our asymmetry-aware cost model, including the model design and model instantiation.
%with formulation
In this section, we introduce our asymmetry-aware cost model, which guides the scheduling in our  approach, including its optimization problem, model design, and model instantiation.

%exist if the formulation is here
\subsection{Problem Formulation}
\label{subsec:problem}
%It's crucial for \design to find the optimal \emph{scheduling plan}, which is guided by the cost model. 


\begin{table}[!h] \centering
  \caption{Symbols and meanings}
  \label{reftab:symbols}
  \resizebox{.85\columnwidth}{!}{%
  %\begin{tabular}{|l|l|ll}
  \begin{tabular}{|L{1cm}|L{5cm}|L{0cm}L{0cm}}
\cline{1-2}
Variable           & \multicolumn{1}{c|}{Description}                          &  &  \\ \cline{1-2}
$t_{i}$      & Task $i$                 &  &  \\ \cline{1-2}
%$S_n$              & The stage $n$ of the whole compression                    &  &  \\ \cline{1-2}
%$R_{n,i}$          & The replica $i$ of $S_n$                              &  &  \\ \cline{1-2}
$m_{i}$          & The number of memory access times under the worst case of $t_{i}$                       &  &  \\ \cline{1-2}
$f_{i}$      & The relative weight factor of $t_{i}$, among all tasks in the same stage  &  &  \\ \cline{1-2}
$i_{i}$           & Input data size of $t_{i}$                           &  &  \\ \cline{1-2}
$L_{set}$          & User assigned cutting-off latency       &  &  \\ \cline{1-2}
%$c_j$              & The $j$ th core of the AMP                                &  &  \\ \cline{1-2}
$C_j$              & Maximum executable instructions within unit time of core $j$  &  &  \\ \cline{1-2}
$I_{job}$          & Total input size of a job                       &  &  \\ \cline{1-2}
$E_{job}$          & Total energy consumption of a compression job            &  &  \\ \cline{1-2}
$L_{job}$          & Total latency of a job                       &  &  \\ \cline{1-2}
$W_j$              & Total instructions per unit time by all workload on core $j$ &  &  \\ \cline{1-2}

$e_{i}$ & Energy consumption of $t_{i}$                      &  &  \\ \cline{1-2}
$l_{i}$     & Latency of $t_{i}$                               &  &  \\ \cline{1-2}
$\iota_{i}$      & Instructions of $t_{i}$                             &  &  \\ \cline{1-2}
$\eta_{i}$     & Instructions per unit time of $t_{i}$        &  &  \\ \cline{1-2}
$\zeta_{i}$     & Instructions per unit energy of $t_{i}$          &  &  \\ \cline{1-2}
$\kappa_{i}$     & Instructions per unit memory access of $t_{i}$, also {\emph{quantified ratio between ILP and MLP}}&  &  \\ \cline{1-2}
%$E_{i}^{j}$
\end{tabular}%
    
}
\end{table}
%the equations for the goal and s.t.













 We list the main terminologies  in Table~\ref{reftab:symbols},
and define the optimal {scheduling plan} as ``\emph{the most energy saving one that is within user set latency}''. Equations~\ref{eqn:ejob} to~\ref{eqn:amountC} express this meaning in a formal way.
The optimization goal of minimizing the energy
%\mynote{Noting the term of \emph{power} is inappropriate against the term \emph{energy}, as it is not straightly bound to the users' ending experience in terms of energy billings.} 
cost (in the unit of Joule) is motivated by the worldly concern of energy consumption and carbon emissions~\cite{carbon_china,carnon_eu,carbon_2}. Besides, energy reduction is one of the major reasons for adopting AMP in edge computing. 
Because each {task} consumes the energy and adds it to the total, we use the \emph{sum} operator in Equation~\ref{eqn:ejob} (i.e., $E_{job}=\sum_{i}e_{i}$).
In addition to the energy, there is another insight from the users' aspect, i.e., the total latency of finishing the whole compression job, as there are often strict real-time restrictions in edge-based applications like stream analysis~\cite{nebulastream}. 
Though we do not intend to minimize the latency,
%\mynote{Which will usually conflict with the goal of minimizing energy due to the energy-delay trade-off~\cite{amp_webbrowser}}, 
we make it the primary constraint as Equation~\ref{eqn:toatlLat}, meaning not to exceed the threshold. 
Unlike the energy cost, latency in a chained or pipelined structure is frequently determined by the bottleneck, so we have a \emph{max} operator in Equation~\ref{eqn:toatlLat} (i.e., $L_{job}=\max(l_{i})$). 
%To cover the tolerance ranging from ms to s, we use the unit us for recognizing the latency.
Task oversubscription has been studied in previous work~\cite{algo_oversub}. However, it is not the focus of this paper, so we  disable it in Equation~\ref{eqn:amountC}.
%In addition to the users' aspect, we should also keep the hardware under suitable condition for the stability concern (e.g., the incident long latency should be as less as possible~\cite{amp_fairness_2020,amp_scheduling_2018}). And therefore Equation~\ref{eqn:amountC} is aimed to prevent overload of each core. 


\begin{align}
   &minimize   \sum_{i}e_{i} \label{eqn:ejob}\\
     & \text{s.t.,}  \text{$\forall i \in {0,..,task_n}$,} \text{$\forall j \in {0,..,cores-1}$,} \nonumber \\
     &    \max(l_{i})  \leq L_{set}, \label{eqn:toatlLat},\\
     &    \sum_{\text{task at core j}} \eta_{i} \leq {C_j}, \label{eqn:amountC}
\end{align}

%the equations for the goal and s.t.
% \begin{align}
%   minimize  & \ E_{job} \label{eqn:goal} \\
%     where \ E_{job} &=\sum_{n,i,j}\epsilon_{n,i,j} \label{eqn:ejob}\\
%     \text{s.t.,}  & \ T_{job}  \leq T_{set}, \text{$\forall j \in {0,..,cores-1}$,}\label{eqn:toatlLat} \\
%      &\text{$\forall j \in {0,..,cores-1}$,} \nonumber\\
%     &{W_j}  \leq {C_j}, \label{eqn:amountC}  \\
%             T_{job} &=\max(\tau_{n,i,j}) \label{eqn:tjob} 
%             \\
%             W_j     &=\sum_{n,i} \eta_{n,i,j},  \label{eqn:wjob}
%             &\text{$\forall j \in {0,..,cores-1}$,} \nonumber
% \end{align}

To achieve the goal and perform the necessary evaluations, 
we should pay close attention to the {$e_{i}$} and {$l_{i}$}, 
which are the partial effects in energy and latency of each task (i.e., the $t_{i}$) and contribute to the overall compression job. 
To bridge the gap between software and hardware, we consider the intrinsic property of \emph{tasks} as {$\kappa_{i}$}, which involves the level of both ILP and MLP.
%eqn of energy


\subsection{Asymmetry-aware Model Design}
\label{subsec:elc}
% We show our detailed cost model in this section, which guides to achieve the goal mentioned in Section~\ref{subsec:problem}.
%To address the evaluation objects (i.e., the goal and restrictions) in Section~\ref{subsec:problem}, we present the detailed \model model in this section.
% \textbf{ Energy evaluation ({$e_{i}$})}.
Our goal and primary concern is to reduce energy consumption.
Accordingly, we must precisely evaluate the energy effects of each task (i.e., the $e_i$). 
Instead of direct modeling, we adopt an indirect method that is more feasible and stable, as shown by Equation~\ref{eqn:epsilon}. 
In this equation, both {$\zeta_{i}$} and  {$\eta_{i}$} are intrinsic, hardly changing hardware attributes in response to software property {$\kappa_{i}$}, and they can be acquired by the AMP-adapted \emph{roofline model}, for both performance and energy, respectively. 
Then, the latency 
{$l_{i}$} is used for the transformation in both units and physical quantity.


\iffalse

\textbf{Evaluate the Energy ({$e_{i}$})}.
Minimizing energy consumption is the goal and first concern, so we should evaluate the energy effects of each \myeu (i.e., the $e_{i}$ ) precisely. Instead of direct modeling, we choose a indirect way which is more feasible and stable, and Equation~\ref{eqn:epsilon} depicts the method. In this equation, both {$\zeta_{i}$} and  {$\eta_{i}$} are the intrinsic, hardly changing attributes of the hardware in response to software property {$\kappa_{i}$}, and they can be acquired by the AMP-adapted \emph{roof line model} (for performance and energy respectively). Then, the latency 
{$l_{i}$} is used for the transformation in both unit and physical quantity\mynote{Just according to their definitions}.
%The expansion of these variables are introduced in following subsections.
\fi

\begin{align}
e_{i} &=\frac{\eta_{i} \times l_{i}}{\zeta_{i}} \label{eqn:epsilon} 
\end{align}


\textbf{Modeling for  {$\zeta_{i}$} and {$\eta_{i}$.} 
%and {$C_j$}
}.
%To address the challenge of ILP, MLP, TLP....xxx
Roofline models,
including performance roofline model~\cite{roofline_1st} and energy roofline model~\cite{roofline_energy},
are critical tools for evaluating a hardware's computation power and energy efficiency. 
%\xianzhi{
We use them specifically to predict the outcome of \emph{unit} performance (i.e., {$\eta_{i}$}) and energy (i.e., {$\zeta_{i}$}) of how a given program runs on \textbf{\emph{asymmetric cores}}, which is inspired by the boat-hull adoption~\cite{roofline_boat}. 
%}
Literally, we can use $\iota_{i}$, $l_{i}$ and $e_{i}$ to define and calibrate {$\eta_{i}$} and {$\zeta_{i}$} as shown in Equations~\ref{eqn:def_eta} and~\ref{eqn:def_zeta}.
Previous studies only drew the roofline graph because it is sufficient for hardware evaluation.
However, we extend it to formulas and apply it to AMP for the formulaic estimation of hardware-software co-relationships.




\iffalse

\textbf{Formulaic Roof Lines for  {$\zeta_{i}$}, {$\eta_{i}$} 
%and {$C_j$}
}.
The roof lines, including performance roof line~\cite{roofline_1st} and energy roof line~\cite{roofline_energy}, are essential tools to evaluate the computation power and energy efficiency of a hardware. 
Inspired by the boat-hull adoption~\cite{roofline_boat}, we can also use them to predict the outcome of \emph{unit} performance (i.e.,{$\eta_{i}$}) and energy(i.e.,{$\zeta_{i}$}) of how a given software runs on AMP. By literal meaning, we can use $\iota_{i}$, $l_{i}$ and $e_{i}$ to define and calibrate {$\eta_{i}$} and {$\zeta_{i}$} as Equation~\ref{eqn:def_eta} and~\ref{eqn:def_zeta}.
Although existing studies only draw the roof line graph as it is enough for hardware evaluation, we expand it further to formulas and adopt it to AMP, for the formulaic estimation of hardware-software co-relationship. 
\fi

\begin{align}
    \eta_{i} &=\frac{\iota_{i}}{l_{i}} \label{eqn:def_eta}\\
    \zeta_{i}&= \frac{\iota_{i}}{e_{i}}  \label{eqn:def_zeta}\\
    \eta_{i} &=
    \begin{cases}
      \kappa_{i}*k_{L1}&,  \kappa_{i}<=\kappa_{i}^{L1}  \\
       \kappa_{i}*k_{L2}+b_{L2}&, \kappa_{i}^{L1}<\kappa_{i}<=\kappa_{i}^{L2} \\
       \kappa_{i}*k_{Exceed L2}+b_{Exceed L2}&, \kappa_{i}^{L2}<\kappa_{i}<=\kappa_{i}^{roof} \\
      \eta_{i}^{max}&, \kappa_{i}>\kappa_{i}^{roof} \label{eqn:roofline2} \\
    \end{cases}
\end{align}

%\begin{align}
%C_{j} &=\eta_{i}^{max} \label{eqn:cj} 
%\end{align}

%We use the proportion of instruction density to memory-access density (i.e., IPM in their graphs and $\kappa_{i}$ in our case) as the independent variable, as in previous works. 


In our model, the independent variable of roofline models is $\kappa_{i}$ (aslo denoted as \emph{IPM} in existing works) ,
which represents the quantified ratio between ILP and MLP.
$\kappa_{i}$ is a vital bond for the awareness of asymmetric cores, as different types of cores can lead to diverse {$\zeta_{i}$} and {$\eta_{i}$} for the same given $\kappa_{i}$.
Moreover, due to the similarity of performance and energy roofline models,
we can consider the {$\kappa_{i}-to-\zeta_{i}$} and {$\kappa_{i}-to-\eta_{i}$} relationships in a unified and similar manner.
%
%\xianzhi{The independent variable of roof line models is $\kappa_{i}$ in our model (or the $IPM$ used by state-of-art graphs), which just represents the quantified ratio between ILP and MLP. The $\kappa_{i}$ is a vital bond for the awareness of asymmetric cores, as different types of cores lead to various {$\zeta_{i}$} and {$\eta_{i}$} for the same given $\kappa_{i}$. Moreover, due to the similarity of performance and energy roofline models, we can consider the {$\kappa_{i}-to-\zeta_{i}$} and {$\kappa_{i}-to-\eta_{i}$} relationships in a unified and similar manner.}
%
We use {$\eta_{i}$} in  Equation~\ref{eqn:roofline2} for illustration.
It is worth noting that we use the cache-aware roofline model~\cite{roofline_cache} instead of the original one because the asymmetric cache-memory structure cannot be overlooked.


\iffalse
Following prior works, we let the proportion between instruction density and memory-access density (i.e., IPM in their graphs and $\kappa_{i}$ in our case) as the independent variable. Due to the similarity of performance and energy roof line, we can consider their outputs, the {$\zeta_{i}$} and {$\eta_{i}$} in an unified and similar way, and let's modeling {$\eta_{i}$} in  Equation~\ref{eqn:roofline2} for example.  Noting we adapt the cache-aware roof line~\cite{roofline_cache} to AMP instead of the original one, as the asymmetric cache-memory structure can not be neglected. 
\fi

Because there are four segments in reality,
this equation has a piecewise linear form with coefficients $k$ and $b$. 
First, if {$\kappa_{i}$} does not put significant pressure on L1D, 
$\eta_{i}$ will grow along with {$k_{L1}$}. 
Then, {$\kappa_{i}$} with different pressures on L1D and L2 causes $\eta_{i}$ to grow in different patterns until it reaches the maximum value ($\eta_{i}^{max}$).
Note that the concrete position of the segments, the growth rate, and the intercept can differ for {$\eta_{i}$} and {$\zeta_{i}$}, 
as the core micro-architecture (OoO and In-Order) has a different influence on performance and energy.





\iffalse
This equation has a piecewise linear form with coefficient $k$ and $b$, as there are four segments in reality. First, when {$\kappa_{i}$} do not put too much pressure on L1D, the $\eta_{i}$ will just grow with {$k_{L1}$}. Then, {$\kappa_{i}$} with different pressure on L1D and L2 makes $\eta_{i}$ grow in different patterns, and it will finally reach the maximum value ($\eta_{i}^{max}$). Noting that the concrete position of segments, the growth rate and the intercept may be different for
{$\eta_{i}$} and {$\zeta_{i}$}, as the core micro-architecture (OoO and In-Order) have different influence in terms of performance and energy.
%In addition, the {$\eta_{i}^{max}$}  is exactly the maximum computation power according to state-of-art, so we also have Equation~\ref{eqn:cj} to decide the {$C_j$}.
\fi


We next show the procedure for obtaining {$\kappa_{i}$}, which bridges the ILP/MLP of software and the AMP hardware.
By definition, we have Equation~\ref{eqn:kapa} to obtain {$\kappa_{i}$}. 
The {$\iota_{i}$} can be read directly from perf events~\cite{amp_perf} of instructions, and it is only relevant to {$j$} when there is an excessive amount of {sleep-notify} between {stages}. 
The value of {$m_{i}$} is relative fixed, 
and we can apply an algorithm analysis of {$t_{i}$} to determine it. 
Furthermore, because {$\kappa_{i}$} is the intrinsic of {$t_{i}$} and has nothing to do with data size ({$i_{i}$}),
we can profile it once rather than calculating every time.
A well-balanced pipeline is created by a suitable construction of \emph{replicas} by \emph{RLAS}, which can prevent such a case. 
Even when an unbalance is unavoidable, we can profile  $\delta$  and use the Equation~\ref{eqn:kapap}. 
Moreover, if $i_{i}$ is not available in the algorithm analysis, we can estimate it by using Equation~\ref{eqn:sizeESti} and profiling the coefficient $\beta$.









\iffalse
The way to acquire {$\kappa_{i}$} is simple, and by definition, we have Equation~\ref{eqn:kapa} to get {$\kappa_{i}$}. The {$\iota_{i}$} can be directly read from perf events~\cite{amp_perf} of instructions, and it is only relevant to {$j$} when there is too much \emph{sleep-notify} between \emph{stages}. The {$m_{i}$} is relative fixed, and an algorithm analysis of {$R_{n,i}$} can decide it. More importantly, since {$\kappa_{i}$} is the intrinsic of {$t_{i}$} and have no thing to do with data size({$i_{i}$}), we can profile it only once instead of calculating every time.A suitable construction of \emph{replicas} by \emph{RLAS} makes a well-balanced pipeline, which can prevent such case. Even when the unbalance is inevitable, we can additionally profile $\delta$ and use the Equation~\ref{eqn:kapap}. Even worse, when $i_{i}$ is not available in algorithm analysis, we can alternatively use Equation~\ref{eqn:sizeESti} and profile the coefficient $\beta$ to estimate it.
\fi


\begin{align}
\kappa_{i} &= \frac{\iota_{i}}{m_{i}}  \label{eqn:kapa}  \\
\kappa'_{i} &= \kappa_{i} + \delta*i_{i}  \label{eqn:kapap} \\
  i_{i}&=\beta\times\frac{f_{i}\times I_{job}}{\sum_{\text{all $i'$ in the same stage of $t_{i}$}  }f_{i'}}, \label{eqn:sizeESti} 
\end{align}

\textbf{Modelling for Latency($l_{i}$).}
\label{subsec:latency}
%corresponding to 3.2.
In Equation~\ref{eqn:latency},
 {$l_{i}$} is divided into two parts. 
  The {$l_{i}^{fetch}$} is the time spent fetching data from the previous stage of {$t_{i}$}.
 In contrast,  {$l_{i}^{run}$} represents the \emph{real running time}, i.e., 
 the time {$t_{i}$} spent on processing data.

\iffalse
\textbf{Evaluate the Latency($l_{i}$) under \emph{asymmetric communication}}.
\label{subsec:latency}
The {$l_{i}$} is consisted of two parts in Equation~\ref{eqn:latency}. The {$l_{i}^{run}$} is the \emph{real running time}, i.e., processing the {$t_{i}$} on core {$j$}, while the {$l_{i}^{fetch}$} is the time used for fetching data from the prior stage of {$t_{i}$}.
\fi

\iffalse
With a given data set, the {$l_{i}^{run}$} can be uniquely determined by the input size of {$t_{i}$}(i.e., {$i_{i}$}), and the core {$j$} to run it. Therefore, Equation~\ref{eqn:tau_run} illustrates the simple linear relationship to estimate it, with a constant system overhead {$\omega_{j}$}. 
%When {$I_{n,i}$} is hard to get before execution (e.g., for the stages in the middle of the whole PLSC), we can use 1) the input size of the whole job (denoted as {$I_{-1,-1}$}) and 2) the {$F_{n,i}$} among all replications of {$S_{n}$} to represent it in Equation~\ref{eqn:sizeESti}, where the value {$\beta$} can be also fixed to the certain data set and {$S_{n}$} like {$\lambda$}.
\fi
Inspired by prior~\cite{sp_briskstream,sp_distance}, we evaluate {$l_{i}^{fetch}$} by taking into account the data size to be fetched as well as the \emph{distance} of core {$j$} (which conducts $t_i$) and the core {$j'$} (which conducts $t_{i'}$, i.e., data source of $t_i$).
%\xianzhi{
However, the \emph{distance} here is under the \textbf{\emph{asymmetric communication}} rather than a flat and symmetric path.
%}
Equation~\ref{eqn:tau_fetch} adapts their methods with the \emph{asymmetric communication awareness} to fit into an AMP with cache-memory structure similar to Figure~\ref{fig:rk3399}. 
 When running on the same core (i.e., $j=j'$), there is no additional cost in fetching. 
 Otherwise, 
 we have the worst-case memory-access latency between core {$j$} and {$j'$}, denoted as {$M_{(j,j')}$}, for the common reference.
%Depending on whether core $j$ and $j′$ are %in the same cluster, latency can vary:
Depending on whether core $j$ and $j'$ are in the same cluster, $l^{fetch}$ can vary:
If they are the in same cluster, the L1 of them will act as the first point of data exchange, so the denominator is the minimum L1 cache line size of core {$j$} and {$j'$}, i.e., the {$L1_{j,j'}$}.
If not, the first exchange location will be the cluster L2 cache of cores {$j$} and {$j'$}, and core communication will have to go through the CCI500. 
As a result, we convert {$L1_{j,j'}$} to {$L2_{j,j'}$}, which represents the minimum L2 cache line size of cores {$j$} and {$j'$}, and there is an extra polarity of communication, i.e., 
 {$\rho_{j,j'}$}. 
  It is worth noting that {$\rho_{0,4}$} differs from  {$\rho_{4,0}$}, as discussed previously in Section~\ref{subsec:amp_intro}. Despite the fact that this equation appears to be complicated, it is still in linear form.


The {$l_{i}^{run}$} is less complicated than {$l_{i}^{fetch}$}. With a given data set, it can be uniquely determined by the input size of {$t_{i}$} (i.e., {$i_{i}$}), and the related core {$j$}. 
As a result, 
Equation~\ref{eqn:tau_run} depicts the simple linear relationship used to estimate it, 
with a system overhead {$\omega_{j}$} that is constant. 




\iffalse

Inspired by prior work~\cite{sp_briskstream,sp_distance}, we evaluate the {$l_{i}^{fetch}$} by considering the data size to be fetched and the \emph{distance} of core {$j$} and the source core {$j'$}, however, the \emph{distance} here is under the \emph{asymmetric model} instead of a flat path. Equation~\ref{eqn:tau_fetch} adapts their methods with the \emph{asymmetric core communication} to fit into the AMP with cache-memory structure similar to Figure~\ref{fig:rk3399}\mynote{For AMP devices with other and more complicated cache-memory layout, the Equation~\ref{eqn:tau_fetch} can be expanded by analogy to these steps.}. When running on the same core (i.e., $j=j'$), there is no additional cost in fetching. Otherwise, we have the worst case memory access latency between core {$j$} and {$j'$} (denoted as {$M_{(j,j')}$}) for the common reference, and things can vary according to whether core {$j$} and {$j'$} belong to the same cluster\mynote{In the rk3399 platform and other platform alike to it, cores in the same cluster shares the L2 cache.} or not. If the same, the L1 of them will act as the first place for data exchange, so the minimum L1 cache line size of core {$j$} and {$j'$}, i.e., the {$L1_{j,j'}$}, is the 
denominator. If not, the first exchange place will be the cluster L2 cache of core {$j$} and {$j'$} respectively, and the core communication have to go through the CCI500 . Therefore, we changed the {$L1_{j,j'}$} into {$L2_{j,j'}$}, which represent the minimum L2 cache line size of core {$j$} and {$j'$}, and there is an extra polarity of the communication, i.e., the {$\rho_{j,j'}$}. Noting that the {$\rho_{0,4}$} is different from {$\rho_{4,0}$}, according to our former discussion in Section~\ref{subsec:amp_intro}. Although this equation looks a little complex, it is still under a linear former in fact. 
\fi

%eqn for latency
%\begin{align}
%\end{align}
%illustrate the latency eqn further
\begin{align}
        % assuming & \ \text{$t_{i}$ is mapped to core $j$} \nonumber \\
         assuming &\ \text{$t_{i}$ is mapped to core $j$,}  \nonumber \\
         &\text{$t_{i'}$ is the data source of $t_{i}$, mapped to core $j'$} \nonumber \\
      l_{i} &= l_{i}^{fetch} + l_{i}^{run} \label{eqn:latency}\\
   % I_{n}&=\beta\times\frac{f_{i}\times I_{-1,-1}}{\sum_{all\ i' \ in \ S_n}F_{n,i'}}, \label{eqn:sizeESti}  \\
 l_{i}^{fetch}&=
     \begin{cases}
       0,   \text{if j=j'}&  \\
       \lceil i_{i}/L1_{j,j'}\rceil\times M_{(j,j')}+\omega_{same},
      % if \ c_j \ and \ c_j' \ shares \ L2\ cache &  \nonumber \\
      for \ the \ same  \ cluster \nonumber \\
       \lceil i_{i}/L2_{j,j'}\rceil\times M_{(j,j')}\times \rho_{j,j'}+\omega_{different}, otherwise &  \\ 
      \end{cases} \\
   \label{eqn:tau_fetch} \\
     l_{i}^{run}&=\lambda_{j} \times i_{i}+\omega_{j}, \label{eqn:tau_run} 
\end{align}
\compact
%roof line

\subsection{Model Instantiation}



To demonstrate the model instantiation, we use a simple parallel compression with two tasks (namely $t_{0}$ and $t_{1}$) in series connection, and we assume the target AMP is the rk3399 introduced in Section\ref{subsec:amp_intro}. \shuhao{always add a ``~'' before $\ref$, $\cite$, etc.}




%We use a simple parallel compression with two tasks (namely $t_{0}$ and $t_{1}$)  as an example to illustrate the model instantiation, and we assume the target AMP is the rk3399 introduced in Section~\ref{subsec:amp_intro}. 



%Noting that only $t_{0}$ and $t_{1}$ respectively belonging to two \emph{stages} are used in the calibration phase, as the \emph{replicas} of a \emph{stage} are not needed there.
%Taking the pipelined lz4 with \emph{stages} and \emph{replicas} in subsection~\ref{subsec:PLSC} as the example, and the 6-core rk3399 as the targeted AMP. 
%Here, we have the {$t_{0}$}, {$t_{1}$} and {$t_{2}}$} to determine. 


First and foremost, we calibrate the performance and energy roof lines on both the big core and the little core. 
To \emph{scan} $\kappa$,
We use a benchmark program similar to \cite{roofline_cache},
 which has a fixed $m$ and can change its $iota$ by adjusting the loop times.
 We read the real result value of $\iota$ by perf events, $l$ by OS API, and $e$ by the energy meter for each setting of loop time, then calculate the value of $\kappa$, $\eta$, and $\zeta$ by Equations~\ref{eqn:kapa},~\ref{eqn:def_eta},~\ref{eqn:def_zeta}, and finally fit Equation~\ref{eqn:roofline2}.





%First of all, we calibrate the performance and energy roof lines on both big core and little core. We use a benchmark program similar to \cite{roofline_cache} to do the \emph{scanning} of $\kappa$, which has fixed $M$ and can change its $iota$ by adjustable times of loops. For each setting of loop time, we read the real result value of $\iota$ by perf events, $l$ by OS API, and $e$ by energy meter, then calculate the value of $\kappa$, $\eta$, and $\zeta$ by Equation~\ref{eqn:kapa},~\ref{eqn:def_eta},~\ref{eqn:def_zeta} respectively, and finally fit Equation~\ref{eqn:roofline2}.


Then, by scanning the $I_{job}$ from high to low,
we calibrate the $l^{run}$ and $l^{fetch}$ of $t_{0}$ and $t_{1}$ for all possible combinations of their core mapping,
and the records are used to fit Equations~\ref{eqn:tau_run} and~\ref{eqn:tau_fetch}. 
While $l^{run}$ can be obtained directly from the OS API, $l^{fetch}$ is the subtraction of the latency of the whole job (i.e., $L_{job}$)  and that of the bottleneck stage (i.e., $\max(l^{run}_{i})$). 




%Then, we calibrate the $l^{run}$ and $l^{fetch}$ of $t_{0}$ and $t_{1}$ for all possible combination of their core mapping, by scanning the $I_{job}$ from high to low, and the records are used to fit Equation~\ref{eqn:tau_run} and~\ref{eqn:tau_fetch}. While $l^{run}$ can be directly acquired from OS API, $l^{fetch}$ is the subtraction of the latency of the whole job (i.e., $L_{job}$)  and that of the bottleneck stage (i.e., $\max(l^{run}_{i})$). 


Finally, we profile $\kappa$ of $t_{0}$ and $t_{1}$ using similar $\iota$ acquisition  methods to the first step.
However, we test $t_{0}$ and $t_{1}$ instead of the benchmark program, 
and the $m$ here is statically analysed by the stage-specific algorithm analysis (for instance, refer to $s0$ and $s1$ in Algorithm~\ref{alg:tcomp32}), according to its worst case of memory access. 




%Finally, we profile $\kappa$ of $t_{0}$ and $t_{1}$, with similar $\iota$ acquiring methods to the first step but test the $t_{0}$ and $t_{1}$ instead of the benchmark program, and the $m$ here is statically analysed by the stage-specific algorithm analyse in Algorithm~\ref{alg:lz4}, according to its worst case of memory access. 

After we have completed these calibrations,
 we can evaluate a \emph{scheduling plan} on a given dataset in terms of energy and latency by simply inputting its $I_{job}$. 
 Specifically, we use Equations~\ref{eqn:epsilon}  and~\ref{eqn:latency}  to estimate the energy and latency of each \emph{task}, and then predict the behavior of the whole plan.




%Upon these calibrations are done, we can evaluate a \emph{scheduling plan} on given data set in terms of energy and latency by just inputting its $I_{job}$. During the dynamic-programming-based enumeration of \emph{scheduling plans} in Algorithm~\ref{alg:scheduler}, we use Equation~\ref{eqn:epsilon}  and~\ref{eqn:latency}  to estimate energy and latency of each \emph{task}, and then predict the corresponding behavior of the whole plan.




==> Sections/backup/4_System.tex <==
\section{The \design System} % of the Embedded Sys
\label{sec:sys}
We propose a framework, called \design, for energy efficient parallelization of \compress on AMP.
%with formulation
%In this section, we first present an overview of the \design's structure and working procedure, and then give the formal definition to its optimization problem.
%without formulation
In this section, We present the structure of \design and illustrate its working procedures, and then demonstrate its implementation details.
%We summarize the common component of the lz4, tcomp32 and tdic32 as Algorithm \ref{alg:LC} \mynote{Noting if there are extra data structure like hash table, code-book or state machine, etc., we assume they are initialized before compression and will be updated during the \emph{encoding function}}. In this abstraction, compression can be viewed as multiple series of
%data-parallel \emph{stages} written as $s0$, $s1$ and $s2$, and each \emph{stage} contains one and only one algorithm component. The \emph{stages} form a pipeline as Figure \ref{fig:chain} depicts.



%comment if only overview
%\subsection{System Overview}


\subsection{System Overview}
\label{sec:overview}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.95\columnwidth]{figures/system.pdf}
    \caption{The \design system}  \label{fig:sys}   
\end{figure}
%We propose a framework, called \design, for energy efficient parallelization of \compress on AMP. 
\textbf{What is \design}.
The structure
of \design is shown in Figure \ref{fig:sys}. \design consists of
three major components, including the decomposer, the scheduler, and the executor. 
%
The decomposer accepts the users' input of data, algorithm choice and latency requirements as a \emph{job}, then conduct a sufficient exposing of the \emph{job}'s ILP and MLP, and also further extends the TLP. In this way, it generates multiple possible \emph{scheduling plans}. The scheduler will choose the optimal \emph{scheduling plans} from all by the guidance of AMP-aware cost model
during the enumerating in dynamic programming~\cite{algo_dp_1954}. Specifically, the
model receives the quantified ratio between ILP and MLP as its judgement basis for evaluating energy and latency of each \emph{scheduling plan}. The executor will finally conduct the selected optimal \emph{scheduling plan} on the tailored software with energy measurement functions provided by the meter.

\textbf{How \design works}. 
We present the system workflow in Figure \ref{fig:wf}. In Figure \ref{fig:wf}, the compression \emph{job} is to \emph{'compress 10M byte of XML text data under lz4 algorithm within 3s'}. The detailed workflow is as follows.
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/workFlow.pdf}
    \caption{The \design workflow}  \label{fig:wf}   
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/lz4_pipe.pdf}
    \caption{The lz4 pipeline.}  \label{fig:lz4_lo}   
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/lz4_replica.pdf}
    \caption{lz4 \emph{stages} with \emph{replicas}}  \label{fig:lz4replica}   
\end{figure}
\begin{table}[h]
\centering
\caption{A template \emph{scheduling plan} of lz4}
\label{tab:lz4_plan}
\resizebox{.5\columnwidth}{!}{%
\begin{tabular}{|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
 \emph{Task} & <\emph{stage},\emph{replica}> & Core \\ \hline
0 & <0,0> & 0    \\ \hline
1 & <0,1> & 1    \\ \hline
2 & <1,0> & 4   \\ \hline
\end{tabular}%
}
\end{table}
    First, when \design accepts such \emph{job}, lz4 algorithm will be decomposed to several \emph{stages} and form a task-pipeline shown in Figure \ref{fig:lz4_lo}, noting that the stage-emerging is used here according to section \ref{subsec:PLSC}.
    %, where each \emph{stage} undertake a subset of the lz4's whole function (e.g., write the \emph{lz4-token}~\cite{comp_lz4}).
    Then, \design tries to increase the data parallelism and automatically duplicates the bottleneck \emph{stages} into \emph{replicas} by using the RLAS optimization~\cite{sp_briskstream}. Specifically, the 'load\&find match' (\emph{stage} 0) is slower, so it will have 2 replications as Figure \ref{fig:lz4replica} depicts.
    After this step, the lists of parallel lz4 \emph{tasks} (namely \emph{scheduling plans}) are created, and each \emph{task} is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. We present a template \emph{scheduling plan} with 3 \emph{tasks} in Table \ref{tab:lz4_plan}. Third, \design determine the optimal \emph{scheduling plan} from all that possible according to the AMP-aware cost model, which evaluate energy consumption and execution latency for each plan and take the latency constrain 3s into consideration. Fourth, after having the optimal plan, \design executes it in the tailored run time while measuring its energy consumption by the meter. Finally, we can acquire the compressed data as well as the system log in terms of execution latency, energy cost, etc..
%Assuming that we have a \emph{job} of \emph{' compressing 10M byte of XML text data under lz4 algorithm within 3s '}, and await for the  compressed data. To begin with, the decomposer divide the lz4 algorithm  into several fine-grained \emph{stages}, which one undertake a subset of the lz4's whole function. Then, still in the decomposer, the bottleneck \emph{stages} will be automatically duplicatated into several \emph{replicas} and each one handles a subset of this \emph{stage's} input data. Therefore, the list of parallel lz4 \emph{tasks}, namely \emph{scheduling plan}, are created. For each \emph{task}, it is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. Although there are more than one \emph{scheduling plans} feasible with varying core-mapping, the scheduler will only pick the optimal one by the cost model, which leads to synthetically run \emph{tasks} at both big cores and little cores at the executor. After running such plan, we eventually get the compressed data and can keep an execution log of energy, latency, etc..

\begin{comment}

decompose it into fine-grained \emph{stages}, which one undertake a subset of the \emph{job}'s whole function in order to expose ILP and MLP of compression sufficiently. To further increase TLP and relive bottleneck, it also adapts existing RLAS optimization~\cite{sp_briskstream} to 
duplicate \emph{stage} into several \emph{replicas} and each one handles a subset of this \emph{stage's} input data. Therefore, the compression \emph{tasks} are created, and a \emph{task} is to map a certain \emph{replica} of a certain \emph{stage} at a certain AMP core.

is used to analyze input batches and queries for useful information,
which is then fed into the performance model. The
performance model module uses the collected data to build
models for queries with both CPUs and GPUs to assist operator
dispatching. The dispatcher module assigns stream data
to operators with proper processors according to the performance
model on the fly
Specifically, \design compresses the user specified data under given algorithm and latency restriction (i.e., a compression \emph{job}) by the following steps.

\textbf{Fine-grained decomposing} by the decomposer.
 The purpose of this step is to   expose ILP and MLP of compression, and take the advantage of TLP sufficiently.
The decomposer exploits both task-pipeling and data parallelism. Specifically, it first divide the \emph{job} into fine-grained \emph{stages} which one undertake a subset of the \emph{job}'s 
whole function. Then, \emph{stage} can be duplicated into several \emph{replicas} and each one handles a subset of this \emph{stage's} input data. 

The detailed decomposing is presented in section \ref{sec:lib}.
%We firstly develop a library to divide the whole \emph{job} into several \emph{stages} to expose ILP and MLP sufficiently, and each \emph{stage} only undertake a subset of the job's  whole whole function. Then use the RLAS optimization~\cite{sp_briskstream} to extend TLP and relieve bottleneck by automatic duplication of \emph{stages}. The detailed decomposing is presented in section \ref{sec:lib}.

\textbf{Determine the scheduling plan} by the scheduler. 
After the decomposing, we have the list of \emph{tasks} as the \emph{scheduling plan}, which covers all \emph{stages} and all \emph{replicas} to finish a \emph{job}. Due to the various core mapping ways, there are more than one possible \emph{scheduling plans} existing,
and we have to decide the optimal one by the guidance of cost model in dynamic programming~\cite{algo_dp_1954}'s enumerating. We illustrate this cost model in section \ref{sec:costmodel}.

\textbf{Executing on AMP} by the support of the executor. Once the optimal \emph{scheduling plan} is selected, it will run in the tailored runtime of the executor, where the software interference is minimized. Besides, the executor also provides low-overhead energy measurement by its meter. We present the software configuration and hardware design of the executor in section \ref{sec:implementation}. 

\subsection{Terminologies}
\textbf{Job}. We define the users' requirement of \emph{'compress specified data under specified algorithm within specified latency'} as a compression \emph{job}. 

\textbf{Stage}. 
The whole job of compression can be divided into multiple series of
data-parallel \emph{stages}, and each \emph{stage} only undertake a subset of the \emph{job}'s  whole whole function.
If these \emph{stages} can run simultaneously, they naturally form a pipeline~\cite{comp_pipeline_gpu}.

\textbf{Replica}. To further increase parallelism, the \emph{stage} can be duplicated into several \emph{replicas}, and each one only handles a subset of this \emph{stage's} input data.

\textbf{Task}. A \emph{task} is to map a certain \emph{replica} of a certain \emph{stage} at a certain AMP core, for the real execution.

\textbf{Scheduling Plan}. We define one \emph{scheduling plan} as the list of \emph{tasks}, which covers all \emph{stages} and all \emph{replicas} to finish a \emph{job}. Due to the various core mapping ways, there are more than one possible \emph{scheduling plans} existing.
\end{comment}



\subsection{Implementation Details}
%In this section, we demonstrate how we implement each component of \design.
\label{sec:imple}

\textbf{The Decomposer}
 generates both \emph{stages} and \emph{replicas} of the \emph{job}, and form all possible \emph{scheduling plans} of \emph{tasks}. 
To construct the fine-frained \emph{stages}, We develop the fine-grained decomposition of lz4, tcomp32, and tdic32 as a C++-20 style library, which enables following features.
\begin{myitemize}
    \item \textbf{Sleep-awake mechanism}.  All \emph{stages} will only be \emph{awake} when \emph{there is} data to handle, otherwise, they will \emph{sleep} to reduce energy dissipation.
    %\item \textbf{Automatic Generation of Replicas}.We adopt the RLAS algorithm from existing work~\cite{sp_briskstream}. The RLAS can analyse the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} without  manual intervention.  
    \item \textbf{Extensibility}. We make the most of the \emph{C++ Class}, and the library can be easily extend to support other compression algorithms through inheritance and derivation.
\end{myitemize}
Then, we adopt the RLAS algorithm, which analyses
    the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} in the runtime without
    manual intervention.  
    

\begin{algorithm}[h]
\caption{The working procedure of the scheduler}
\label{alg:scheduler}
\LinesNumbered 
\KwIn{ Array of all possible \emph{scheduling plan} $allPlan$}
\KwIn{Cutting-off latency $L_{set}$}
\KwOut{The optimal \emph{scheduling plan} $oPlan$ }
$oPlan$ $\leftarrow$ the first one in $allPlan$ \;
$e \leftarrow infinity$ \;
\ForEach {\emph{scheduling plan} $tPlan$ enumerated from $allPlan$ by dynamic programming\label{algo:dp0} } 
{
$t$ $\leftarrow$ estimated $L_{job}$ of $tPlan$ \label{algo:estiL} \;
\If{$t <L_{set}$ \label{algo:compareL}}
{
  $e0$ $\leftarrow$ estimated $E_{job}$ of $tPlan$ \label{algo:estiE}\;
  \If{$e0 < e$ \label{algo:compareE}}
  {
    $oPlan$ $\leftarrow$ $tPlan$ \label{algo:oPlan0}\;
    $e$ $\leftarrow$ $e0$ \label{algo:oPlan1}\;
  }
}

}

%\newpage
\end{algorithm}
\textbf{The scheduler} is to determine optimal \emph{scheduling plan}, and its pseudocode is demonstrated as Algorithm \ref{alg:scheduler}. As multiple formation of \emph{task} leads to a large space of \emph{scheduling plans}, we adopt the dynamic programming to reduce the complexity (Line \ref{algo:dp0}). For each \emph{scheduling plan} enumerated, the scheduler will first predict its $L_{job}$ by the cost model (Line \ref{algo:estiL}) and compare with the $L_{set}$ (Line \ref{algo:compareL}). If not exceed, the corresponding $E_{job}$  (Line \ref{algo:estiE}) will also be estimated and compared with the current least predicted energy (Line \ref{algo:compareE}); otherwise, we simply discard such \emph{scheduling plan}. After the dynamic programming is done, we will find the optimal \emph{scheduling plan} with both satisfying $L_{job}$ and least $E_{job}$, according to the Line \ref{algo:oPlan0} and \ref{algo:oPlan1}.  


\textbf{The executor} provides a clean environment to conduct the selected optimal \emph{scheduling plan}, as well as accurate low overhead energy measurement for the calibration of cost model and the evaluation or monitoring by the users. Specifically, it consists the co-design as follows:
\begin{myitemize}
    \item \textbf{The Tailored Software Environment.}
Instead of direct implementation the common release of software environment like the ubuntu by prior work~\cite{amp_DVFS2}, {\design} has a customized and tailored manner as the redundant software in common releases which has nothing to do with parallel {\compress} may have interference to it (i.e., in terms of core occupation and energy consumption), and may also challenge the real-time properties of the whole system.  To minimize the such kind of interference and uncertainty by other software, we customized the software system by the \emph{buildroot}~\cite{amp_buildroot} 2021-08-rc1, so the unnecessary software can be directly discard or disabled by explicit scripts and configurations.
%\mynote{our configuration file is avaliable %at xxxx}. 
Besides, the \emph{buildroot} can also provide C++20 support for both cross-compilers and libraries conveniently, which is the standard of {\design}'s implementation. 
For the kernel of the operating system, we choose the mainline linux 5.10~\cite{amp_linux}, which has already supported the 64-bit AMP stably, and has the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime,amp_linux_eas}.
  
  \item \textbf{The Energy Meter}.
%To provide energy measurement in {\design}, it is not a good idea to let the AMP platform directly sample its energy consumption like existing studies~\cite{amp_scheduling_2021,amp_webbrowser} do. As we noted in section \ref{subsec:amp_intro}, frequently addressing the low-speed peripherals can make the asymmetric core communication more complicated. Besides, using wireless-connected meter~\cite{amp_game} is also inappropriate in our case, due to the additional latency and power consumption caused by it. Therefore, {\design} has its own design of the energy meter and its supplementary (i.e., the MCU software and Linux driver of it).
The key aspects of this meter are 1) to relieve the AMP platform from continuously sampling, which leads to less interference of the \emph{inter-cluster} communication, and 2) to achieve low-latency data reporting by wired communication. It is designed as Figure \ref{fig:meter} depicts.
The Texas Instrument's INA226~\cite{amp_ina226} current/voltage sensor chip in this meter is a precise one of wide use, and it provides the raw measurement. The Espressif's ESP32S2~\cite{amp_esp32s2} micro control unit (MCU) is applied for periodic sampling and calculation of the energy in Joule, and it can report data to the AMP platform via USB2.0. Hence, the energy measurement process in {\design} is quite simple, which follows the flow chart in Figure \ref{fig:flow_meter} and is without any additional overhead in running the \emph{scheduling plans}.
The meter is assembled by trust-worth manufacturer under Surface-Mounted-Technology (SMT) , and its final specifications are listed in Table \ref{tab:meter}. For more details, we present its hardware schematics in Appendix \ref{appendix:sch}.

\end{myitemize}


\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter.pdf}
    \caption{The design of energy meter}  \label{fig:meter}   
\end{figure}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter_flow.pdf}
    \caption{The control flow for AMP to access the meter }  \label{fig:flow_meter}   
\end{figure}


%discard if move to sec 5

%Next in section \ref{subsec:elc}, we present the details to study them.
%\label{sec:models}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%many plan to xxx, in stage, replication. Different scheduling 
%The \model  predicts energy, latency and core load of each \emph{stage} and its all \emph{replicas} in \compress for the optimization. In this section, we give the formal definition



==> Sections/backup/4_System1225.tex <==
\section{The \design System} % of the Embedded Sys
\label{sec:sys}
We propose a framework, called \design, for energy efficient parallelization of \compress on AMP.
%with formulation
%In this section, we first present an overview of the \design's structure and working procedure, and then give the formal definition to its optimization problem.
%without formulation
In this section, we firstly present an overview  of \design, and then demonstrate its implementation details.
%We summarize the common component of the lz4, tcomp32 and tdic32 as Algorithm \ref{alg:LC} \mynote{Noting if there are extra data structure like hash table, code-book or state machine, etc., we assume they are initialized before compression and will be updated during the \emph{encoding function}}. In this abstraction, compression can be viewed as multiple series of
%data-parallel \emph{stages} written as $s0$, $s1$ and $s2$, and each \emph{stage} contains one and only one algorithm component. The \emph{stages} form a pipeline as Figure \ref{fig:chain} depicts.



%comment if only overview
%\subsection{System Overview}


\subsection{System Overview}
\label{sec:overview}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.95\columnwidth]{figures/system.pdf}
    \caption{The \design system}  \label{fig:sys}   
\end{figure}
%We propose a framework, called \design, for energy efficient parallelization of \compress on AMP. 
\textbf{What is \design}.
The structure
of \design is shown in Figure \ref{fig:sys}. \design consists of
three major components, including the decomposer, the scheduler, and the executor. 
%
The decomposer accepts the users' input of data, algorithm choice and latency requirements as a \emph{job}, then conduct a sufficient exposing of the \emph{job}'s ILP and MLP, and also further extends the TLP. In this way, it generates multiple possible \emph{scheduling plans}. The scheduler will choose the optimal \emph{scheduling plans} from all by the guidance of AMP-aware cost model
during the enumerating in dynamic programming~\cite{algo_dp_1954}. Specifically, the
model receives the quantified ratio between ILP and MLP as its basis for judgement in evaluating the energy and latency of each \emph{scheduling plan}. The executor finally conduct the selected optimal \emph{scheduling plan} on the tailored software with energy measurement functions provided by the meter.

\textbf{How \design works}. 
We present the system workflow in Figure \ref{fig:wf}. In Figure \ref{fig:wf}, the compression \emph{job} is to \emph{'compress 10M byte of XML text data under lz4 algorithm within 3s'}. The detailed workflow is as follows.
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/workFlow.pdf}
    \caption{The \design workflow}  \label{fig:wf}   
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/lz4_pipe.pdf}
    \caption{The lz4 pipeline.}  \label{fig:lz4_lo}   
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/lz4_replica.pdf}
    \caption{lz4 \emph{stages} with \emph{replicas}}  \label{fig:lz4replica}   
\end{figure}
\begin{table}[h]
\centering
\caption{A template \emph{scheduling plan} of lz4}
\label{tab:lz4_plan}
\resizebox{.5\columnwidth}{!}{%
\begin{tabular}{|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
 \emph{Task} & <\emph{stage},\emph{replica}> & Core \\ \hline
0 & <0,0> & 0    \\ \hline
1 & <0,1> & 1    \\ \hline
2 & <1,0> & 4   \\ \hline
\end{tabular}%
}
\end{table}
    First, when \design accepts such \emph{job}, lz4 algorithm will be decomposed to several \emph{stages} and form a task-pipeline shown in Figure \ref{fig:lz4_lo}, noting that the stage-emerging is used here according to Section \ref{subsec:PLSC}.
    %, where each \emph{stage} undertake a subset of the lz4's whole function (e.g., write the \emph{lz4-token}~\cite{comp_lz4}).
    Then, \design tries to increase the data parallelism and automatically duplicates the bottleneck \emph{stages} into \emph{replicas} by using the RLAS optimization~\cite{sp_briskstream}. Specifically, the 'load\&find match' (\emph{stage} 0) is slower, so it will have 2 replications as Figure \ref{fig:lz4replica} depicts.
    After this step, the lists of parallel lz4 \emph{tasks} (namely \emph{scheduling plans}) are created, and each \emph{task} is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. We present a template \emph{scheduling plan} with 3 \emph{tasks} in Table \ref{tab:lz4_plan}. Third, \design determine the optimal \emph{scheduling plan} from all that possible according to the AMP-aware cost model, which evaluates energy consumption and execution latency for each plan and take the latency constrain 3s into consideration. Fourth, after having the optimal plan, \design executes it in the tailored run time while measuring its energy consumption by the meter. Finally, we can acquire the compressed data as well as the system log including execution latency, energy cost, etc.
%Assuming that we have a \emph{job} of \emph{' compressing 10M byte of XML text data under lz4 algorithm within 3s '}, and await for the  compressed data. To begin with, the decomposer divide the lz4 algorithm  into several fine-grained \emph{stages}, which one undertake a subset of the lz4's whole function. Then, still in the decomposer, the bottleneck \emph{stages} will be automatically duplicatated into several \emph{replicas} and each one handles a subset of this \emph{stage's} input data. Therefore, the list of parallel lz4 \emph{tasks}, namely \emph{scheduling plan}, are created. For each \emph{task}, it is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. Although there are more than one \emph{scheduling plans} feasible with varying core-mapping, the scheduler will only pick the optimal one by the cost model, which leads to synthetically run \emph{tasks} at both big cores and little cores at the executor. After running such plan, we eventually get the compressed data and can keep an execution log of energy, latency, etc..




\subsection{Implementation Details}
%In this section, we demonstrate how we implement each component of \design.
\label{sec:imple}

\textbf{The Decomposer}
 generates both \emph{stages} and \emph{replicas} of the \emph{job}, and form all possible \emph{scheduling plans} of \emph{tasks}. 
To construct the fine-frained \emph{stages}, We develop the fine-grained decomposition of lz4, tcomp32, and tdic32 as a C++-20 style library, which enables following features.
\begin{myitemize}
    \item \textbf{Sleep-awake mechanism}.  All \emph{stages} will only be \emph{awake} when \emph{there is} data to handle, otherwise, they will \emph{sleep} to reduce energy dissipation.
    %\item \textbf{Automatic Generation of Replicas}.We adopt the RLAS algorithm from existing work~\cite{sp_briskstream}. The RLAS can analyse the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} without  manual intervention.  
    \item \textbf{Extensibility}. We make the most of the \emph{C++ Class}, and the library can be easily extend to support other compression algorithms through inheritance and derivation.
\end{myitemize}
Then, we adopt the RLAS algorithm, which analyses
    the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} in the runtime without
    manual intervention.  
    

\begin{algorithm}[h]
\caption{The working procedure of the scheduler}
\label{alg:scheduler}
\LinesNumbered 
\KwIn{ Array of all possible \emph{scheduling plan} $allPlan$}
\KwIn{Cutting-off latency $L_{set}$}
\KwOut{The optimal \emph{scheduling plan} $oPlan$ }
$oPlan$ $\leftarrow$ the first one in $allPlan$ \;
$e \leftarrow infinity$ \;
\ForEach {\emph{scheduling plan} $tPlan$ enumerated from $allPlan$ by dynamic programming\label{algo:dp0} } 
{
$t$ $\leftarrow$ estimated $L_{job}$ of $tPlan$ \label{algo:estiL} \;
\If{$t <L_{set}$ \label{algo:compareL}}
{
  $e0$ $\leftarrow$ estimated $E_{job}$ of $tPlan$ \label{algo:estiE}\;
  \If{$e0 < e$ \label{algo:compareE}}
  {
    $oPlan$ $\leftarrow$ $tPlan$ \label{algo:oPlan0}\;
    $e$ $\leftarrow$ $e0$ \label{algo:oPlan1}\;
  }
}

}

%\newpage
\end{algorithm}
\textbf{The scheduler} determines the optimal \emph{scheduling plan}, and its pseudocode is demonstrated in Algorithm \ref{alg:scheduler}. As multiple formation of \emph{task} leads to a large space of \emph{scheduling plans}, we adopt the dynamic programming to reduce the complexity (Line \ref{algo:dp0}). For each \emph{scheduling plan} enumerated, the scheduler will first predict its $L_{job}$ by the cost model (Line \ref{algo:estiL}) and compare with the $L_{set}$ (Line \ref{algo:compareL}). If not exceed, the corresponding $E_{job}$  (Line \ref{algo:estiE}) will also be estimated and compared with the current least predicted energy (Line \ref{algo:compareE}); otherwise, we simply discard such \emph{scheduling plan}. After the dynamic programming is done, we will find the optimal \emph{scheduling plan} with both satisfying $L_{job}$ and least $E_{job}$, according to the Line \ref{algo:oPlan0} and \ref{algo:oPlan1}.  


\textbf{The executor} provides a clean environment to conduct the selected optimal \emph{scheduling plan}, as well as accurate low overhead energy measurement for the calibration of cost model and the system monitoring by the users. Specifically, it consists the co-design as follows:
\begin{myitemize}
    \item \textbf{The Tailored Runtime.}
Instead of directly deploying the common release of software environment like the ubuntu by prior work~\cite{amp_DVFS2}, {\design} has a customized and tailored manner as the redundant software in common releases which has nothing to do with parallel {\compress} may have interference to parallel compression (i.e., in terms of core occupation and energy consumption), and may also challenge the real-time properties of the whole system.  To minimize the such kind of interference and uncertainty by other software, we customized the software system by the \emph{buildroot}~\cite{amp_buildroot} 2021-08-rc1, so the unnecessary software can be directly discard or disabled by explicit scripts and configurations.
%\mynote{our configuration file is avaliable %at xxxx}. 
Besides, the \emph{buildroot} can also provide convenient C++20 support with both cross-compilers and libraries, which is the standard of {\design}'s implementation. 
For the kernel of the operating system, we choose the mainline linux 5.10~\cite{amp_linux}, which has already supported the 64-bit AMP stably, and has the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime,amp_linux_eas}.
  
  \item \textbf{The Energy Meter}.
%To provide energy measurement in {\design}, it is not a good idea to let the AMP platform directly sample its energy consumption like existing studies~\cite{amp_scheduling_2021,amp_webbrowser} do. As we noted in Section \ref{subsec:amp_intro}, frequently addressing the low-speed peripherals can make the asymmetric core communication more complicated. Besides, using wireless-connected meter~\cite{amp_game} is also inappropriate in our case, due to the additional latency and power consumption caused by it. Therefore, {\design} has its own design of the energy meter and its supplementary (i.e., the MCU software and Linux driver of it).
The key aspects of this meter are 1) to relieve the AMP platform from continuously sampling and frequent peripheral addressing (so there is less interference of to \emph{inter-cluster} communication according to Section~\ref{sucbsec:sideEffects}), and 2) to achieve low-latency data reporting by wired communication. It is designed as Figure \ref{fig:meter} depicts.
The Texas Instrument's INA226~\cite{amp_ina226} current/voltage sensor chip in this meter is a precise one of wide use, and it provides the raw measurement. The Espressif's ESP32S2~\cite{amp_esp32s2} micro control unit (MCU) is applied for periodic sampling and calculation of the energy in Joule, and it can report data to the AMP platform via USB2.0. Hence, the energy measurement process in {\design} is quite simple, which follows the flow chart in Figure \ref{fig:flow_meter} and there is no additional overhead in running the \emph{scheduling plans}.
The meter is assembled by trust-worth manufacturer under Surface-Mounted-Technology (SMT) , and its final specifications are listed in Table \ref{tab:meter}. For more details, we present its hardware schematics in Appendix \ref{appendix:sch}.

\end{myitemize}


\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter.pdf}
    \caption{The design of energy meter}  \label{fig:meter}   
\end{figure}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter_flow.pdf}
    \caption{The control flow for AMP to access the meter }  \label{fig:flow_meter}   
\end{figure}


%discard if move to sec 5

%Next in Section \ref{subsec:elc}, we present the details to study them.
%\label{sec:models}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%many plan to xxx, in stage, replication. Different scheduling 
%The \model  predicts energy, latency and core load of each \emph{stage} and its all \emph{replicas} in \compress for the optimization. In this section, we give the formal definition



==> Sections/backup/4_System_short.tex <==
\section{The \design System} % of the Embedded Sys
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.95\columnwidth]{figures/system.pdf}
    \caption{The \design system}  \label{fig:sys}   
\end{figure}
\label{sec:sys}
We propose a framework, called \design, for energy efficient parallelization of \compress on AMP,
which is shown in Figure \ref{fig:sys}. \design consists of
three major components, including the decomposer, the scheduler, and the executor. 
%
First, the decomposer accepts the users' input of data, algorithm choice and latency requirements as a \emph{job}, then conduct a sufficient exposing of the \emph{job}'s ILP and MLP, and also further extends the TLP according to \ref{subsec:pros}. In this way, it generates multiple possible lists of parallel compression \emph{tasks}, and each list is a \emph{scheduling plan}. Next, the scheduler will choose the optimal \emph{scheduling plan} from all by the guidance of asymmetry-aware cost model
during the enumerating in dynamic programming~\cite{algo_dp_1954}. Specifically, the
model receives the quantified ratio between ILP and MLP as its basis for judgement in evaluating the energy and latency of each \emph{scheduling plan}. Third, the executor conduct the selected optimal \emph{scheduling plan} on the tailored software with energy measurement functions provided by the meter.

%with formulation
%In this section, we first present an overview of the \design's structure and working procedure, and then give the formal definition to its optimization problem.
%without formulation
%In this section, we firstly present an overview  of \design, and then demonstrate its implementation details.
%We summarize the common component of the lz4, tcomp32 and tdic32 as Algorithm \ref{alg:LC} \mynote{Noting if there are extra data structure like hash table, code-book or state machine, etc., we assume they are initialized before compression and will be updated during the \emph{encoding function}}. In this abstraction, compression can be viewed as multiple series of
%data-parallel \emph{stages} written as $s0$, $s1$ and $s2$, and each \emph{stage} contains one and only one algorithm component. The \emph{stages} form a pipeline as Figure \ref{fig:chain} depicts.



%comment if only overview
%\subsection{System Overview}


%\subsection{System Overview}
\label{sec:overview}

%We propose a framework, called \design, for energy efficient parallelization of \compress on AMP. 


%discard if move to sec 5

%Next in Section \ref{subsec:elc}, we present the details to study them.
%\label{sec:models}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%many plan to xxx, in stage, replication. Different scheduling 
%The \model  predicts energy, latency and core load of each \emph{stage} and its all \emph{replicas} in \compress for the optimization. In this section, we give the formal definition



==> Sections/backup/5_Imple.tex <==
\section{Implementation Details}
\label{sec:imple}
In this section, we demonstrate how we implement each component of \design.

\subsection{The Decomposer}
The decomposer generates both \emph{stages} and \emph{replicas} of the \emph{job}, and form all possible \emph{scheduling plans} of \emph{tasks}. 
To construct the fine-frained \emph{stages}, We develop the fine-grained decomposition of lz4, tcomp32, and tdic32 as a C++-20 style library, which enables following features.
\begin{myitemize}
    \item \textbf{Sleep-awake mechanism}.  All \emph{stages} will only be \emph{awake} when \emph{there is} data to handle, otherwise, they will \emph{sleep} to reduce energy dissipation.
    %\item \textbf{Automatic Generation of Replicas}.We adopt the RLAS algorithm from existing work~\cite{sp_briskstream}. The RLAS can analyse the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} without  manual intervention.  
    \item \textbf{Extensibility}. We make the most of the \emph{C++ Class}, and the library can be easily extend to support other compression algorithms through inheritance and derivation.
\end{myitemize}
Then, we adopt the RLAS algorithm, which analyses
    the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} in the runtime without
    manual intervention.  
    
\subsection{The scheduler}
\begin{algorithm}[h]
\caption{The working procedure of the scheduler}
\label{alg:scheduler}
\LinesNumbered 
\KwIn{ Array of all possible \emph{scheduling plan} $allPlan$}
\KwIn{Cutting-off latency $L_{set}$}
\KwOut{The optimal \emph{scheduling plan} $oPlan$ }
$oPlan$ $\leftarrow$ the first one in $allPlan$ \;
$e \leftarrow infinity$ \;
\ForEach {\emph{scheduling plan} $tPlan$ enumerated from $allPlan$ by dynamic programming\label{algo:dp0} } 
{
$t$ $\leftarrow$ estimated $L_{job}$ of $tPlan$ \label{algo:estiL} \;
\If{$t <L_{set}$ \label{algo:compareL}}
{
  $e0$ $\leftarrow$ estimated $E_{job}$ of $tPlan$ \label{algo:estiE}\;
  \If{$e0 < e$ \label{algo:compareE}}
  {
    $oPlan$ $\leftarrow$ $tPlan$ \label{algo:oPlan0}\;
    $e$ $\leftarrow$ $e0$ \label{algo:oPlan1}\;
  }
}

}

%\newpage
\end{algorithm}
The scheduler is to determine optimal \emph{scheduling plan}, and its pseudocode is demonstrated as Algorithm \ref{alg:scheduler}. As multiple formation of \emph{task} leads to a large space of \emph{scheduling plans}, we adopt the dynamic programming to reduce the complexity (Line \ref{algo:dp0}). For each \emph{scheduling plan} enumerated, the scheduler will first predict its $L_{job}$ by the cost model (Line \ref{algo:estiL}) and compare with the $L_{set}$ (Line \ref{algo:compareL}). If not exceed, the corresponding $E_{job}$  (Line \ref{algo:estiE}) will also be estimated and compared with the current least predicted energy (Line \ref{algo:compareE}); otherwise, we simply discard such \emph{scheduling plan}. After the dynamic programming is done, we will find the optimal \emph{scheduling plan} with both satisfying $L_{job}$ and least $E_{job}$, according to the Line \ref{algo:oPlan0} and \ref{algo:oPlan1}.  
\subsection{The executor}
The executor consists several anti-interference strategies in both software and hardware, which provides a clean environment to conduct the selected optimal \emph{scheduling plan}, as well as accurate low overhead energy measurement for the calibration of cost model and the evaluation or monitoring by the users.

\textbf{The Tailored Software Environment}
Instead of direct implementation the common release of software environment like the ubuntu by prior work~\cite{amp_DVFS2}, {\design} has a customized and tailored manner as the redundant software in common releases which has nothing to do with parallel {\compress} may have interference to it (i.e., in terms of core occupation and energy consumption), and may also challenge the real-time properties of the whole system.  To minimize the such kind of interference and uncertainty by other software, we customized the software system by the \emph{buildroot}~\cite{amp_buildroot} 2021-08-rc1, so the unnecessary software can be directly discard or disabled by explicit scripts and configurations.
%\mynote{our configuration file is avaliable %at xxxx}. 
Besides, the \emph{buildroot} can also provide C++20 support for both cross-compilers and libraries conveniently, which is the standard of {\design}'s implementation. 

For the kernel of the operating system, we choose the mainline linux 5.10~\cite{amp_linux}, which has already supported the 64-bit AMP stably, and has the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime,amp_linux_eas}.

\textbf{The Energy Meter}
To provide energy measurement in {\design}, it is not a good idea to let the AMP platform directly sample its energy consumption like existing studies~\cite{amp_scheduling_2021,amp_webbrowser} do. As we noted in section \ref{subsec:amp_intro}, frequently addressing the low-speed peripherals can make the asymmetric core communication more complicated. Besides, using wireless-connected meter~\cite{amp_game} is also inappropriate in our case, due to the additional latency and power consumption caused by it. Therefore, {\design} has its own design of the energy meter and its supplementary (i.e., the MCU software and Linux driver of it).
The key aspects of this meter are 1) to relieve the AMP platform from continuously sampling and 2) to achieve low-latency data reporting by wired communication, so it is designed as Figure \ref{fig:meter}.

The Texas Instrument's INA226~\cite{amp_ina226} current/voltage sensor chip in this meter is a precise one of wide use, and it provides the raw measurement. The Espressif's ESP32S2~\cite{amp_esp32s2} micro control unit (MCU) is applied for periodic sampling and calculation of the energy in Joule, and it can report data to the AMP platform via USB2.0. Hence, the energy measurement process in {\design} is quite simple, which follows the flow chart in Figure \ref{fig:flow_meter} and is without any additional overhead in running the \emph{scheduling plans}.

The meter is assembled by trust-worth manufacturer under Surface-Mounted-Technology (SMT) , and its final specifications are listed in Table \ref{tab:meter}. For more details, we present its hardware schematics in Appendix \ref{appendix:sch}.

\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter.pdf}
    \caption{The design of energy meter}  \label{fig:meter}   
\end{figure}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/meter_flow.pdf}
    \caption{The control flow for AMP to access the meter }  \label{fig:flow_meter}   
\end{figure}

==> Sections/backup/5_System_20220108.tex <==
\section{Implementation Details}
\label{sec:imple}
\shuhao{Remove Section 5 as you are running out of space. Merge the ``necessary paragraph'' into previous sections. 
Backup the figures etc, you can reuse them in a journal version.
1) The system overview discussion may be merged to 2.3. Remember, only the critical and necessary discussions are needed.
2) The discussion of decomposer may be merged to Section 3.
3) The discussion of scheduler merged into section 4.
}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.75\columnwidth]{figures/system.pdf}
    \caption{The \design system.}  \label{fig:sys}   
\end{figure}

 We implement the \design system
in this section as Figure~\ref{fig:sys} demonstrates.
%Assuming that we have a \emph{job} of \emph{' compressing 10M byte of XML text data under lz4 algorithm within 3s '}, and await for the  compressed data. To begin with, the decomposer divide the lz4 algorithm  into several fine-grained \emph{stages}, which one undertake a subset of the lz4's whole function. Then, still in the decomposer, the bottleneck \emph{stages} will be automatically duplicatated into several \emph{replicas} and each one handles a subset of this \emph{stage's} input data. Therefore, the list of parallel lz4 \emph{tasks}, namely \emph{scheduling plan}, are created. For each \emph{task}, it is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. Although there are more than one \emph{scheduling plans} feasible with varying core-mapping, the scheduler will only pick the optimal one by the cost model, which leads to synthetically run \emph{tasks} at both big cores and little cores at the executor. After running such plan, we eventually get the compressed data and can keep an execution log of energy, latency, etc..
\design consists of
two major components, including a decomposer and a scheduler. 
%
First, the decomposer accepts the compression job and performs a sufficient exposing of its ILP and MLP, as well as further parallelism extension, as shown in Section~\ref{sec:decompos}. 
In this way, it generates multiple possible {scheduling plans} with parallel compression {tasks}.
Second, the scheduler selects the optimal {scheduling plan} using the guidance of our asymmetry-aware cost model
during the enumeration in dynamic programming~\cite{algo_dp_1954}. 
In particular, the
model uses the quantified ratio between ILP and MLP as its basis for judgement in assessing the energy and latency of each {scheduling plan} according to Section~\ref{sec:costmodel}. 
For the smooth execution of such an optimal {scheduling plan}, 
we also optimize  \design in its run time environment and energy measurement (more details can be found in our technical report~\cite{}).
%\xianzhi{For the smooth execution of such optimal {scheduling plan}, we also optimized the \design in its run time environment and energy measurement (details can be found at our technical report~\cite{}) }


%\subsection{Implementation Details}
%In this section, we demonstrate how we implement each component of \design.
\label{sec:imple}

\textbf{The Decomposer}
 generates fine-grained taks and forms all possible {scheduling plans}.
 Specifically, 
 we develop the pipeline stages of compression algorithms as a C++-20 style library, which enables the following features.
 \shuhao{shorten this part. No need to emphasize. No need to itemize.}
\begin{myitemize}
    \item \textbf{Sleep-awake mechanism}.  All tasks will  be \emph{awake} only when \emph{there is} data to process; otherwise, they will \emph{sleep} to reduce energy dissipation.
    %\item \textbf{Automatic Generation of Replicas}.We adopt the RLAS algorithm from existing work~\cite{sp_briskstream}. The RLAS can analyse the \emph{stages} and  generate \emph{replicas} to relieve the bottleneck \emph{stages} without  manual intervention.  
    
    \item \textbf{Extensibility}. We require that most of the \emph{C++ Classes}, and the library can be easily extended to support more compression algorithms through inheritance and derivation.
\end{myitemize}
Then, to suitably generate the {replicas}, we adopt the RLAS algorithm, which analyses
    the {stages} and  automatically replicates the bottleneck {stages} on the fly without
    manual intervention.  
%Specifically for this lz4 \emph{job}, it will be decomposed to several \emph{stages} and form a task-pipeline shown in Figure~\ref{fig:lz4_lo}, noting that the stage-emerging is used here according to Section~\ref{subsec:pros}. Then, the bottleneck \emph{stage} 'load\&find match' (\emph{stage} 0) will have 2 replications as Figure~\ref{fig:lz4replica} depicts.  After this step, the lists of parallel lz4 \emph{tasks} (namely \emph{scheduling plans}) are created, and each \emph{task} is a certain \emph{replica} of a certain \emph{stage} to be mapped at a certain AMP core. We present a template \emph{scheduling plan} with 3 \emph{tasks} in Table~\ref{tab:lz4_plan}.

\begin{algorithm}[h]
\caption{The working procedure of the scheduler}
\label{alg:scheduler}
\LinesNumbered 
\KwIn{ Array of all possible \emph{scheduling plan} $allPlan$}
\KwIn{Cutting-off latency $L_{set}$}
\KwOut{The optimal \emph{scheduling plan} $oPlan$ }
$oPlan$ $\leftarrow$ the first one in $allPlan$ \;
$e \leftarrow infinity$ \;
\ForEach {\emph{scheduling plan} $tPlan$ enumerated from $allPlan$ by dynamic programming\label{algo:dp0} } 
{
$t$ $\leftarrow$ estimated $L_{job}$ of $tPlan$ \label{algo:estiL} \;
\If{$t <L_{set}$ \label{algo:compareL}}
{
  $e0$ $\leftarrow$ estimated $E_{job}$ of $tPlan$ \label{algo:estiE}\;
  \If{$e0 < e$ \label{algo:compareE}}
  {
    $oPlan$ $\leftarrow$ $tPlan$ \label{algo:oPlan0}\;
    $e$ $\leftarrow$ $e0$ \label{algo:oPlan1}\;
  }
}

}

%\newpage
\end{algorithm}


\label{sec:sys} 
\shuhao{Merge this scheduler discussion into section 4. Make it Section 4.4}
\textbf{The scheduler} determines the optimal \emph{scheduling plan}, and its pseudocode is demonstrated in Algorithm~\ref{alg:scheduler}. As the formation of \emph{task} leads to a large space of \emph{scheduling plans}, we adopt dynamic programming~\cite{algo_dp_1954} to reduce the complexity of enumeration (Line~\ref{algo:dp0}). 
For each \emph{scheduling plan} enumerated, the scheduler first predicts its $L_{job}$ by the cost model (Line~\ref{algo:estiL}) and compares it with the $L_{set}$ (Line~\ref{algo:compareL}). If not exceeded, the corresponding $E_{job}$  (Line~\ref{algo:estiE}) will also be estimated and compared with the current least predicted energy (Line~\ref{algo:compareE}); otherwise, we simply discard this \emph{scheduling plan}. 
After the dynamic programming is done, we can find the optimal \emph{scheduling plan} with both $L_{job}<L_{set}$ and the least $E_{job}$, according to Lines~\ref{algo:oPlan0} and~\ref{algo:oPlan1}.  



==> Sections/backup/6_Evaluation.tex <==
\section{Evaluation }
\label{sec:evaluation}
In the following, we present our evaluation results. Each experiment is repeated 10 times and we report the average.
% In Section~\ref{subsec:e2e}, we compare \design against alternative solutions in handling different real-world workloads, and examine the model correctness of \design. Next, we evaluate the impacts of varying system setting (i.e., the $L_{set}$ and core frequencies) in Section~\ref{subsec:system_sens}, and effects of different workload configurations (i.e., input data size and statistics properties) in Section~\ref{subsec:workload_sens}, for \design and its competitors. We also show in Section~\ref{subsec:factor_ana} the relative importance of design factors of \design.

% of \design’s major techniques in the end.
% Hence, there is no extra preprocessing in loading data.
%The main object of our experiments is to comprehend the behavior of {\design} on AMP. Specifically, we seek answers to the following questions.
% The primary goal of our experiments is to explore the behavior of {\design} on AMP. 
% We firstly introduce our methodology in Section~\ref{subsec:exp_set_up}.
% Then,
\begin{table}[t]
\centering
\caption{Average prediction and real value of of $E$ for two-task tcomp32. The unit of energy is Joule.}
\vspace{+3pt}
\label{tab:correctness}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\diagbox{variable}{$(c, c') pair$}    & (0, 1) & (0, 4) & (4, 0) & (4, 5) \\ \hline
Estimated $E$ &4.7&4.0&4.2&5.8     \\ \hline
Measured $E$  &4.5&3.9&4.3&5.5       \\ \hline
Relative error &0.04&0.03&0.02&0.05\\ \hline
\end{tabular}%
}
\end{table}

\begin{table}[t]
\centering
\caption{Average prediction and real value of $E$ for optimal \emph{scheduling plans}. The unit of energy is Joule.}
\vspace{+3pt}
\label{tab:correctness2}
\resizebox{.75\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\diagbox{variable}{method}    & lz4 & tcomp32 & tdic32 \\ \hline
Estimated $E$ &4.4&4.0&4.1     \\ \hline
Measured $E$  &3.9&3.7&4.5    \\ \hline
Relative error &0.14&0.08&0.09\\ \hline

\end{tabular}%
}
\end{table}

\label{sucsec:confirmation}
We first evaluate the accuracy of the cost model of \design.
Specifically, we examine the correctness of the cost model in predicting the energy ($E$) for scheduling of parallelized tcomp32 as discussed previously in Section~\ref{sec:decompos} as an example.

Table~\ref{tab:correctness} shows the predicted and measured values of $E$ for four different pairs of $(c, c')$, which cover all scenarios if the same type of cores are treated equally.
%which are mapped to cores $j$ and $j′$, %respectively.
To validate the overall effectiveness of our cost model, we show the relative error rate associated with estimated energy consumption $E$ by our analytical model. 
Specifically, we define $relative\_error=\frac{|E^{mes}-E^{est} |}{E^{mes}}$, where {$E^{mes}$} represents the measured value and {$E^{est}$} represents the estimated value by the model. 

We show the model accuracy of all algorithms under the generated optimal {scheduling plan} in Table~\ref{tab:correctness2}. 
Overall, our estimation approximates the measurement well for the $E$ of all three algorithms. It is able to produce the optimal scheduling plan and predict the performance behavior quite accurately. 
The inaccuracy is mainly caused by the difficulty in accurately estimating the frequency ($m$) and latency of actual memory accessing ($M_{c, c'}$), as it is affected by multiple factors such as memory access patterns and hardware prefetcher units.
% Nevertheless, we plan to investigate in future work.
\subsection{Compression Abilities V.S. Overhead}
\label{subsec:e2e}
In this section, we show the end-to-end comparison between \design and four competing mechanisms.

\begin{figure}[!th]
    \centering
    \includegraphics*[width=0.98\columnwidth]{figures/e2e/total/energy.pdf}
     \caption{Energy consumption comparison.} 
    \label{fig:eng_total}  
\end{figure}
\begin{figure} [t]
    \centering
    \includegraphics*[width=0.98\columnwidth]{figures/e2e/total/violation.pdf}
    \caption{Latency constraint violation (LCV) comparison.}  \label{fig:vio_total}   
\end{figure}
\textbf{Energy Consumption Comparison}.
Figure~\ref{fig:eng_total} reports the energy consumption under relatively loose {$L_{set}$} for different mechanisms.
In general, we can see that \design always outperforms other mechanisms, by virtue of its least energy consumption and no latency constraint violation. 
For example, \design can save up to 53.23\% energy on the lz4-{Stock} workload compared with {BO}.
\design wisely utilizes all cores taking the costly inter-cluster communication overhead into consideration.
% The reason is that the optimal scheduling plan in reality is \emph{to synthetically use both big cores and little cores}, 
% and {\design} can always enjoy such optimization. 
In contrast, {LO} and {BO} avoid inter-cluster communication overhead but under-utilizes computational powers.
{R\&R} achieves load balancing among cores but overlook the communication overhead.
\design outperforms OS scheduler as the latter treats the compression algorithm as a black box, overlooking many optimization opportunities.


\textbf{Latency Constraint Violation Comparison}.
% latency constraint violation refers to the degree of dissatisfaction with the latency constraint, as discussed in  Section~\ref{subsec:performance_metrics}.
Figure~\ref{fig:vio_total} presents the ratio of latency constraint violation under different mechanisms.
We can see that both {\design} and {BO} successfully prevent any latency constraint violations for the evaluated workloads.
% can achieve \emph{zero} violation in this case.
LO and R\&R fails to preserve the latency constraints due to the low utilization of computational power of AMPs, especially the high performance big cores.
OS, although tries to have a sufficient utilization, still fails due to two reasons. 
First, 
its frequent migration of tasks leads to extra overhead. 
Our further investigation reveals that OS scheduler involves about 60,000 context switches while \design only involves about 10 context switches for processing every megabyte of input data.
Second, 
treating compression tasks as black box results in a relatively inaccurate estimating of latency and causes latency constraint violations.
%\shuhao{RR and OS fails because xxx.}
 \etoePic {lset} {Impacts of varying {$L_{set}$}.} {fig:rovio_lz4}
\subsection{System Configuration Analysis}
\label{subsec:system_sens}
In this section, we evaluate the system sensitivity to user-specified latency constraint and CPU core frequency.

\textbf{Varying Latency Constraint ({$L_{set}$}).}
Different use case scenarios may demand a trade-off between energy consumption and latency constraints. 
We study the impact of varying latency constraints by parallelizing tcomp32 with {Rovio} dataset.
The results are shown in Figure~\ref{fig:rovio_lz4}.
Unlike {OS}, {R\&R}, {BO}, and {LO}, which have relatively fixed energy consumption, {\design} is an \emph{adaptive} method to trade off latency and energy consumption. Specifically, \design can focus more on energy saving under a loose $L_{set}$, and output nearly the same high performance plan as BO under tight $L_{set}$.
 
\begin{figure}[t]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/freq/ene.pdf}
    \caption{Impacts of varying CPU Core frequency. ``B'' denotes the big cores while ``L'' denotes the little cores.}  \label{fig:eng_freq}   
\end{figure} 
\textbf{Varying CPU Core Frequency.}
Different CPU core frequencies of AMPs can lead to diverse computational power and energy consumption. 
We study the impact of varying CPU core frequency by parallelizing tcomp32 with {Rovio} dataset. %\shuhao{Why change dataset comapre to previous one??}
The results are shown in Figure~\ref{fig:eng_freq}. 
The \design outperforms other mechanisms with varying frequency settings. Although lower frequency result in low power (measured in Watts), their increased latency in compression causes higher energy consumption, especially when tasks running on little cores. This also reaffirms the insufficiency of applying DVFS~\cite{amp_DVFS1, amp_DVFS2, amp_DVFS3} in our context.

%  according to state-of-the-art~\cite{amp_DVFS1, amp_DVFS2, amp_DVFS3}
% 
% For each mechanism, 
%\cred{lower frequency is not equal to low energy consumption in Joule ?????}, and this is even on the total contrary for \textbf{LO}, \textbf{R\&R}, \textbf{NS} and \textbf{\design}. 
% \xianzhi{a lower frequency does not inevitably lead to lower energy consumption.}
%Although lower frequency can absolutely lead to low power (measured in Watt) according to state-of-art~\cite{amp_DVFS1, amp_DVFS2, amp_DVFS3}, their increased latency in \compress is even more significant and cause higher energy consumption sometimes (especially for {tasks} running at little cores). 
% This is why we should synthetically consider the roof lines and latency in Equation~\ref{eqn:epsilon}, and also confirms the failure of DVFS further.

\subsection{Workload Sensitivity Study}
\label{subsec:workload_sens}
In this section, we show the superiority of \design under varying workload characteristics, including input data size, vocabulary duplication,  symbol duplication, and dynamic range. 
As not all compression algorithms are sensitive to all statistical properties, we examine tcomp32 under varying input data size, the tdic32 under changing symbol duplication, the lz4 under varying vocabulary duplication, and the tcomp32 under different dynamic range, which are the most sensitive, respectively.

% Workload characteristics, including data size and statistical properties of data, vary significantly. 
% In this section, we first use real world dataset Rovio and tcomp32 algorithm to study the impacts of varying input data sizes. 
% % ?However, as statistical properties are hard to adjust in real world datasets, 
% Then, we use the synthetic dataset Micro to study the impact of varying three major statistical properties, including symbol duplication, vocabulary duplication, and dynamic range. 

\begin{figure}[t]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/batchSize/ene.pdf}
    \caption{Impacts of different input data size.}  \label{fig:eng_bsize}   
\end{figure}
\textbf{Input Data Size ($I$)}.
 %The input data size (i.e., $I$) can influence the baseline of energy consumption but has little effect on latency constraint violation.
 %The reason is that {$L_{set}$} is typically synchronously growing with input data size. 
 %and core overload is determined by intrinsic properties of the data and algorithm. 
We study the energy consumption with different input data size (i.e., $I$) by using tcomp32 with Rovio dataset as an example.
The results are shown in Figure~\ref{fig:eng_bsize}.
As expected according to Equations~\ref{eqn:epsilon}, ~\ref{eqn:tau_fetch} and ~\ref{eqn:tau_run}, the energy consumption is approximately linear to the data size. 
Different mechanisms result in different scheduling plans that have varying growth rates in terms of energy consumption per unit of input data, which is linearly proportional to {$\frac{\eta}{\zeta}$}.
% , as their resulting scheduling plans have different . 
As pointed out by Equation~\ref{eqn:roofline}, the {$\frac{\eta}{\zeta}$} is determined by both tasks (i.e., by the $\kappa$) and cores (i.e, by the different parameter $a$, $b$ for big core and little core).
\design guarantees minimum {$\frac{\eta}{\zeta}$} by suitable core-mapping for tasks with different $\kappa$.
In contrast, neither of LO, BO, R\&R and OS can  achieve such proper mapping, which leads to a high growth rate.
% In contrast, \design can  utilize both big cores and little cores
% and always consumes the least energy.
%The LO has a

\wsPic {v64} {Impacts of different vocabulary duplication.} {fig:v64}
\textbf{Vocabulary Duplication.}
In the following, we use the synthetic dataset Micro to study the impact of varying three major statistical properties.
We first parallelize lz4 to compress Micro with varying vocabulary duplication. 
$\kappa$ of lz4 decreases with increasing duplication in the dataset as it leads to more ``matches''. That is, a vocabulary is more likely to be found in previous records. 
Therefore, the total loops of sliding-window-based traversing is reduced (which leads to lower $\chi$), and the backward searching for expanding match is increased (which means higher $m$).
% of 64-bit vocabulary. 
Figure~\ref{fig:v64} shows that \design always achieve least energy consumption, as \design is able to accurately estimate $\eta$ and $\zeta$ under changing $\kappa$.
%先讲\kapp怎么变
% With the duplication growing from low to high, the $\kappa$ drops from high to low. 
% This is because lz4 has more ``matches'', that is a vocabulary is more likely to be found in previous records. 
All mechanisms has high energy consumption when duplication is moderate. This is because 
``mismatch'' (which slightly increases total instructions $\chi$ due to more loops) and ``match'' (which slightly increases memory access times $m$ due to more backward searching) are reconciled in lz4.

\begin{comment}
%具体代入big core 和little core 的roofline, 中间的\kappa 最耗能，搞定
% the resulting middle $\kappa$ under such case 
% makes ``mismatch'
% much energy dissipated in handling L1D miss
% because the ``mismatch'' (which slightly increases total instructions $\chi$ due to more loops) and ``match'' (which slightly increases memory access times $m$ due to more backward searching) are reconciled in lz4, 
% a middle vocabulary duplication consumes the most energy for all mechanisms. 
% when duplication is moderate, has high energy consumption. The reason is middle $\kappa$ in this case leads to highest {$\frac{\eta}{\zeta}$}.
\xianzhi{ 
Our further investigation on the substitution of $\kappa$ to the roofline (Equation~\ref{eqn:roofline}) of big cores and little cores reveals that a middle $\kappa$ in the studied range leads to highest {$\frac{\eta}{\zeta}$}, which why??
 %代入进roofline 就是这样，
 explains why middle vocabulary duplication leads to highest energy consumption for all mechanism.
 }
There are three key observations.
With the duplication grow from low to high,
the $\kappa$ drops from high to low. This is because lz4 has more ``matches'' in the increasing vocabulary duplication, that is a vocabulary is more likely to be found in previous records. Therefore, the total loops of lz4 is reduced (which leads to lower $\chi$), and the backward searching of expansion match is increased (which means high $m$).
Our further investigation on the substitution of $\kappa$ in the lz4's range to the roofline (Equation~\ref{eqn:roofline}) of big cores and little cores reveal that a middle $\kappa$
 leads highest {$\frac{\eta}{\zeta}$}
First, 
when duplication is low to moderate, all mechanisms has high energy consumption.
This is because lz4 algorithm encounters middle level of ``mismatch'' (which slightly increases total instructions $\chi$ due to more loops) and ``match'' (which slightly increases memory access times $m$ due to more backward searching) and consists middle $\kappa$.
when duplication is high, all mechanisms achieve lower energy. In such a case, lz4 has more ``matches'', that is a vocabulary is more likely to be found in previous records. Therefore, the total loops of lz4 is reduced (which leads to lower $\chi$), and the backward searching of expansion match is increased (which means high $m$). Therefore, a low $\kappa$ is generated, which leads to lowest {$\frac{\eta}{\zeta}$} according to our further investigation.
\end{comment}
% all mechanisms achieve lower energy consumption when duplication is high. 
% In such a case, lz4 has more ``matches and backward searching'', that is a vocabulary is more likely to be found in previous
% This increases memory access times $m$ due to more backward searching.

\begin{comment}
Second,  
moderate vocabulary duplication
leads to the highest energy consumption.
case means a middle $\kappa$ in the \emph{encoding} of lz4, according the system log of \design indicates. The substitution of such $\kappa$ to Equation~\ref{eqn:roofline} results in high {$\frac{\eta}{\zeta}$} for both big cores and little cores 
\shuhao{"give the reason why is that."}
\shuhao{because the ``mismatch'' (which slightly increases total instructions $\chi$ due to more loops) and ``match'' (which slightly increases memory access times $m$ due to more backward searching) are reconciled in lz4, 
a middle vocabulary duplication consumes the most energy for all mechanisms. 
Specifically, we have a moderate operational intensity ($\kappa$) which leads to high {$\frac{\eta}{\zeta}$} in Equation~\ref{eqn:epsilon} under this case.}
\end{comment}


% //
% We adjust the entropy of the 32-bit symbol,  leaving the other parameters unchanged in {Micro}. We show the results of the most entropy-sensitive algorithm tdic32 in Figure~\ref{fig:e32}.
% %In general, tdic32 consumes middle ILP space and middle MLP space.It employs a MLP-leading hash tabling, but does not necessitate backward searching. Moreover, it consists of ILP-leading unaligned I/O, which is not accompanied by a heavy computation as tcomp32 does. 
% We can see that little cores and big cores have different or even contradictory responses to increasing entropy under this algorithm with globally moderate ILP and MLP, which is caused by different task-core affinity.
% However, 
% due to their higher quantity, 
% the little cores appear to be more decisive in plans that use all the cores, 
% such as {R\&R}, {OS}, {NS}, and {\design}.
% Furthermore, it is self-evident that {\design} is always the best at changing symbol entropy.
% \wsPic {e32} {Impacts of different symbol entropy.} {fig:e32}
% //

\wsPic {e32} {Impacts of different symbol duplication.} {fig:e32}
\textbf{Symbol Duplication}.
We next vary the duplication of the 32-bit symbol, leaving the other parameters unchanged in {Micro}. 
The tdic32 is more sensitive to symbol duplication. Specifically, high duplication significantly reduces the \emph{update} frequency of its hash table (i.e., replace the table content with new value), and can also reduce the overhead of writing output data.
The results of parallelizing tdic32 are shown in Figure~\ref{fig:e32}.
We can see that LO has an increasing energy consumption with increasing symbol duplication. This is because the pipeline and cache of little cores is less efficient as it in-order executed. 
In contrast, BO becomes more energy efficient with increasing symbol duplication as big cores are out-of-order executed.
\design, {R\&R}, and {OS} utilize both big and little cores and are affected by little cores more as there are more little cores.
Nevertheless, \design is always able to achieve least energy consumption at changing symbol duplication, which reaffirms its superiority compared to competing mechanisms.

% little cores and big cores have different or even contradictory responses to increasing symbol duplication.
% under this algorithm
%with globally moderate operational intensity ($\kappa$), 
% which is caused by different task-core affinity.
% However, due to their higher quantity, the little cores appear to be more decisive in plans that use all the cores, such as {R\&R}, {OS}, and {\design}.
% \xianzhi{Furthermore,
% the superiority of \design is confirmed again in 
% encountering varying symbol duplication.}
% it is \shuhao{self-evident???? that {\design} is always the best at changing symbol duplication.} \shuhao{reaffirms that} \shuhao{Be more specific.}

\wsPic {r32} {Impacts of different dynamic range.} {fig:r32}
\textbf{Dynamic Range}.
Finally, the results of parallelizing tcomp32 under varying the dynamic range of the 32-bit symbol, are shown in Figure~\ref{fig:r32}.
% we evaluate the impact of varying the dynamic range of the 32-bit symbol.
%  are shown in Figure~\ref{fig:r32}.
%In general, tdic32 consumes middle ILP space and middle MLP space.It employs a MLP-leading hash tabling, but does not necessitate backward searching. Moreover, it consists of ILP-leading unaligned I/O, which is not accompanied by a heavy computation as tcomp32 does. 
We can see that the energy consumption grows with increasing dynamic range for all mechanisms. In particular, tcomp32 spends even more in the $log2$ computation ( Line~\ref{algo:tcomp32_encodeEnd} of Algorithm~\ref{alg:tcomp32}), which increases both operational intensity ($\kappa$) and latency ($l$). This results a higher energy consumption according to Equations~\ref{eqn:epsilon} and~\ref{eqn:roofline}.
% According to Equations~\ref{eqn:epsilon} and~\ref{eqn:roofline}, higher energy consumption
% is naturally caused.
\design always outperforms others, but its energy saving becomes less significant when the dynamic range is high, as there is less room for optimization.
%little cores and big cores have different or even contradictory responses to increasing duplication under this algorithm with globally moderate operational intensity ($\kappa$), which is caused by different task-core affinity.

\begin{comment}
\shuhao{Follow my style in previous part to revise this part.
We evaluate the scheduling of tcomp32 tasks by scanning the dynamic range of a 32-bit symbol from low to high and fixing other parameters of Micro.
The performance results is demonstrated in Figure~\ref{fig:r32}.
With the growing range,  tcomp32 spends even more in the $log2$ computation, which  increases both operational intensity ($\kappa$) and latency ($l$). According to Equations~\ref{eqn:epsilon} and~\ref{eqn:roofline2}, higher $\kappa$ and $l$ lead to more energy consumption.
Although {\design} still outperforms the others, its energy saving becomes less significant when the dynamic range is high, as there is less room for optimization.}
\end{comment}
\subsection{Factor analysis}
\label{subsec:factor_ana}
To better comprehend the overheads and benefits of various design aspects of \design, we show a factor analysis in Figure~\ref{fig:factor_ene} that highlights energy dissipation and latency constraint violation. 
% tested under loose $L_{set}$, and 
The \emph{energy dissipation} is calculated by $\frac{E^{actual} - E^{min}}{E^{min}}$, where $E^{actual}$ is the actual energy consumption, and $E^{min}$ is the theoretical minimum energy consumption according to our cost model. 
We use tcomp32 and Rovio dataset as an example. The results are shown in Figure~\ref{fig:factor_ene}. 
\emph{simple} refers to a SMP-aware parallel data compression~\cite{cpmp_bzip2}, which only exploits the data parallelism. %pbzip2~\cite{cpmp_bzip2}-like
\emph{+decom.} adds the fine-grained decomposition and enables the pipeling parallelism, as described in Section~\ref{sec:decompos}.
\emph{+asy-core.} adds the asymmetric-core-awareness, including all modeling in Section~\ref{subsec:elc} but ignoring the $\rho$ in Equation~\ref{eqn:tau_fetch}. 
Specifically, this method uses a NUMA-aware~\cite{sp_briskstream} way to evaluate core communication in AMPs.
Finally, \emph{+asy-comm.} adds the consideration of $\rho$ in Equation~\ref{eqn:tau_fetch}, and is the fully functional \design as introduced in Section~\ref{sec:overview}.

\begin{figure}[t]
    \centering
    \includegraphics*[width=0.98\columnwidth]{figures/factor_ene.pdf}
    \caption{Factor analysis. LCV means latency constraint violation.}  
    \label{fig:factor_ene}   
\end{figure}

We have the following observations.
First, 
compared to \emph{simple}, \emph{+decom.} provides opportunities for better utilization of both big cores and little cores, which can reduce energy dissipation. However, \emph{+decom.} still treats AMP as an SMP, and can lead to suboptimal scheduling due to the ignorance of asymmetric computational power among cores. 
Ignoring the asymmetric communication also leads to more latency constraints violation.
Second, 
\emph{+asy-core.} adds asymmetric core awareness. 
It can always correctly determine the varying task-core affinity among tasks with different operational intensity ($\kappa$), which leads to further energy consumption reduction. 
Nevertheless, due to the ignorance of asymmetric communication effects, it is too aggressive for energy saving and violates the $L_{set}$ frequently.
Third, 
\design further adds asymmetric communication awareness (i.e., \emph{+asy-comm.}) compared to \emph{+asy-core.}.
It can model and plan well before execution, and thus prevent the latency constraint violation while ensuring the least energy consumption. 
The remaining energy dissipation by \design is marginal (i.e., about 10 \%), and is caused by the less-accurate estimation of memory accesses in our cost model. 
We plan to investigate techniques to estimate memory accesses with machine learning techniques~\cite{pmlr-v80-hashemi18a} to further enhance \design.






==> Sections/backup/6_Optimization.tex <==
\section{Optimization}
\label{sec:model}

\subsection{Rule-based Factors Tuning}


\subsection{Asymmetry-aware Cost Model to Guide the workload Scheduling}

There are a number of parameters (for example, the ratio in the data-dividing scheme) to be determined for parallelizing stream compression on AMPs. 
In this section, we develop a cost model to predict the latency and energy consumption of parallel stream compression on AMP, and then use the cost model to determine the suitable values for the parameters.
% core-mapping of parallel stream compression tasks, among the wide design space discussed in Section~\ref{subsec:revist}.

Due to the single-ISA property, the same executable binary file with different parameters can be directly shared between big cores and little cores. Moreover, there is an inter-connection -based sharing of the same memory area between the cluster of big cores and that of little cores, as introduced in Section~\ref{subsec:amp_intro}. Unfortunately, existing works~\cite{amp_partition_2019, amp_cluster_2021} only consider inter-cluster communication for task switching in operating system level, but not for specific tasks.
It is therefore desirable to have an unified model to estimate the performance of stream compression on both the big cores and the little cores in terms of both computation and communication. 
% In particular, there is lack of a model to estimate such asymmetric communication effects for parallelizing compression on AMPs.
% If we are unable to estimate the asymmetric communication for fine-grained scheduling, especially the long latency of $c2$, there can be more violation of latency constraints.


In Section~\ref{subsec:revist}, we have identified PL as a basic abstraction for stream compression on the AMP
(DD is a special case for PL). This allows us to abstract the common design issues on the cost model for
different arrangement of cores and their workload. We call this high level abstraction the abstract model. 
For a specific stream compression algorithm, we obtain its cost model by instantiating the abstract model with profiling and algorithm-specific analytic modelling (e.g., memory optimizations). 
In the remainder of this section, we first present the abstract model for PL on the AMP, and next use the tcomp32 algorithm (a simplification to 32-bit elias gamma~\cite{comp_elias} encoding) as an example of instantiating the abstract model.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Symbols and meanings.}
\label{reftab:symbols}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{|p{1.1cm}|p{6cm}|}
\hline
Variable          & \multicolumn{1}{c|}{Description}                                                                          \\ \hline
$r_i$             & Workload ratios for the big cores at Step i                                                               \\ \hline
$E$               & Total energy consumption for all cores executing all steps                                                \\ \hline
$L$               & Total latency for all cores executing all steps                                                           \\ \hline
$p_{Xcores}^i$    & The power consumption (in Watt) of executing Step i on  all Xcores (Xcores=\{ big cores, liitle cores \}) \\ \hline
$x_i$             & The number of input items (e.g., tuples) at Step i                                                        \\ \hline
$E_{Xcores}^i$    & The energy consumption of executing Step i on all Xcores                                                  \\ \hline
$L_{Xcores}^i$    & The latency of executing Step i on all Xcores                                                             \\ \hline
$C_{Xcores}^i$    & Computation latency                                                                                       \\ \hline
$In_{Xcores}^i$   & Inter-cluster communication latency                                                                       \\ \hline
$Ia_{Xcores}^{i}$ & Intra-cluster communication latency                                                                       \\ \hline
$D_{Xcores}^{i}$  & The pipelined delay of Step i                                                                             \\ \hline
$I_i$             & The average number of instructions per tuple in Step i                                                    \\ \hline
$\eta_{Xcores}^i$ & Instructions per unit time for executing Step i                                                           \\ \hline
\end{tabular}%
}
\end{table}

\textbf{Model Design}
We model the energy consumption and latency of executing a step series with PL. All terminologies used in our work is summarized in Table~\ref{reftab:symbols}.
The step series consists of $n+1$ steps, with $x_i$ items on step i ($0 \leq i \leq n$). 
The cost model predicts the energy consumption and latency of PL with workload ratios $r_i$ in Step i. 
Thus, the total energy consumption $E$ estimated to be the sum of big cores and little cores (Equation \ref{eqn:energy}), and the total latency is the longer value of them (Equation \ref{eqn:latency}). 
Moreover, the effects of every step is accumulated in both energy and latency.
\begin{align}
    T &= \max_{Xcores} (\sum_{i} T_{Xcores}^i) \label{eqn:latency} \\
    E &= \sum_{Xcores} ( \sum_{i} E_{Xcores}^i) \label{eqn:energy} \\
    Xcores &=\{Bigcores, Littlecores\} \nonumber
\end{align}

% input data
% In the following, we model the energy consumption of each task $t_i$ by using the symbol $e_i$, and its latency as $l_i$.  


%\textbf{Latency Estimation}
Next we break down the latency into four parts in Equation~\ref{eqn:latency_s}, considering 1) computational overhead $C_{Xcores}^i$, 2) communication overhead $In_i$ and $Ia_{Xcores}^{i}$ and 3) pipelined delay $D_{Xcores}^{i}$. 
\begin{align}
    L_{Xcores}^i &= C_{Xcores}^i+In_{Xcores}^i+ Ia_{Xcores}^{i}+D_{Xcores}^{i}
    \label{eqn:latency_s}
\end{align}

We estimate the computation latency to be the total execution
time for all the instructions of the step in Equation~\ref{eqn:latency_compu}. 
The number of instructions $I_i$ is irrelevant to core types due to ISA-sharing. However, big cores and little cores have different performance factors (i.e., instructions per unit time, denoted as $\eta_{Xcores}^i$). These factors can also be acquired by using to roofline models (See Section~\ref{subsec:roofline}). We assume there is a fixed $\eta_{Xcores}^i$ for each tuple, and more careful modeling which considers the dynamics will be the future work.
\begin{align}
    C_{Xcores}^i &= \frac{I_i \times r_i \times x_i}{\eta_{Xcores}^i} 
    \label{eqn:latency_compu}
\end{align}

$In_{Xcores}^i$ and $Ia_{Xcores}^{i}$ are caused by cache line exchanges, and we follow existing work~\cite{sp_briskstream} to model them. Although modeled under the same approach, they should be treated separately due to asymmetric communication effects as introduced in Section~\ref{subsec:amp_intro}. Moreover, we can ignore $Ia_{Xcores}^i$ sometimes, as such intra-cluster communication leads to much less overhead than 
inter-cluster communication $In_{Xcores}^i$.

For $D_{Xcores}^{i}$, this delay is caused by different workload ratios
in the two consecutive steps. The delay occurs when
the input data for Step i have not been generated from Step
(i-1), There are two cases depending on the workload ratio
comparison.

Case 1:
if $r_i > r_{i-1}$, we use Equation~\ref{eqn:wait_big}. The big cores may encounter
delay while the little cores prepare the input data in
Step (i-1) for the big cores in Step i. The ratio of the little cores
latency that is not pipelined with the big cores in Step (i-1) is
$\frac{1-r_i}{1-r_{i-1}}$. By subtracting this amount of latency (${L_{little \ cores}^{i-1}} \times \frac{1-r_i}{1-r_{i-1}} $ from the total little cores latency from Step 0 to Step i-1,
we get
the latency of the little cores from Step 0 to the end of the pipelined
execution area in Step i-1. The total big cores latency from Step
0 to the end of pipelined execution area with the little cores in
Step i is $\sum_{j=0}^{i} L_{big \ cores}^j$. Therefore, $D_{big \ cores}^{i}$ is the delay time on
the big cores to wait for data generated from the little cores in Step
i-1. If calculated below 0, we set $D_{big \ cores}^{i}=0$, meaning there will be no pipelined execution delay.

Case 2: if $r_i < r_{i-1}$ we use Equation~\ref{eqn:wait_little} to calculate the pipelined
execution delay for the little cores in a similar way to Case 1.
We assume
an ideal execution pipeline with the optimal IPC on each
processor, and a hash join on uniform data distributions.
\begin{align}
    D_{big \ cores}^i &= (\sum_{j=0}^{i-1} L_{little \ cores}^j - {L_{little \ cores}^{i-1}} \times \frac{1-r_i}{1-r_{i-1}})  \nonumber \\
    &- \sum_{j=0}^{i} L_{big \ cores}^j
    \label{eqn:wait_big} \\
     D_{little \ cores}^i &= \sum_{j=0}^{i-1} L_{big \ cores}^j - \nonumber \\
     &({L_{big \ cores}^{i-1}} \times \frac{1-r_{i-1}}{1-r_{i}}-\sum_{j=0}^{i} L_{little \ cores}^j)  
    \label{eqn:wait_little}
\end{align}

Finally, as specific to the pipelined stream compression, we need
to estimate the cost of intermediate results and the communication
cost between the big cores and the little cores. We estimate
the cost for two consecutive steps. If they have the same
workload ratio, we can ignore the costs on intermediate results
and the communication. Otherwise, the amount of intermediate
results can be derived from the difference of the
workload ratio between the two steps. For Step i, the number
of intermediate data items is $(r_i-r_{i-1} \times (x_i)$, assuming
a uniform distribution.


%\textbf{Energy Estimation}
We estimate the energy consumption to be the power of the core times the processing time. The power consumption $p_{Xcores}^i$ is determined by both specific cores and specific step, and it can be predicted by roofline models~\cite{roofline_energy} according to the operational intensity of the step. 
% (as introduced in Section~\ref{subsec:roofline}, by using Equations~\ref{eqn:roofline} and ~\ref{eqn:power}). 
\begin{align}
    E_{Xcores}^i &= p_{Xcores}^i \times L_{Xcores}^i \label{eqn:energy_s} 
\end{align}

The roofline models reveal the piecewise linear relationship between a software and its outcome on hardware. Considering the impacts of L1 and L2 cache, there are four segments on the AMP we studied, as presented in Algorithm~\ref{eqn:roofline}. 



First, when {$\kappa$} is low and does not put significant pressure on L1D (i.e., within the first boundary $\kappa_{L1}$), {$\eta$} or {$\zeta$} grows relatively fast with growth rate $a_{L1}$ and intercept $b_{L1}$. Second, condition $\kappa_{L1} <\kappa<= \kappa_{L2}$ means a higher {$\kappa$} that makes L1D missing frequent and have significant impacts on the core. In this case, {$\eta$} or {$\zeta$} grows slower with growth rate $a_{L2}$ and intercept $b_{L2}$. 
Third, with $\kappa$ increasing into $\kappa_{L2} <\kappa <= \kappa_{roof}$, the L2 missing has major effects and therefore changes the $a_{L2}$ and $b_{L2}$ into $a_{Exceed L2}$ and $b_{Exceed L2}$, respectively.
Fourth, after $\kappa$ reaches the last boundary $\kappa_{roof}$, the {$\eta$} or {$\zeta$} stays at the maximum value instead of increasing with $\kappa$.
\begin{align}
 \scriptsize
    \eta \text{ or } \zeta &=
    \begin{cases}
      \kappa*a_{L1}+b_{L1}&, \kappa<=\kappa_{L1}  \\
       \kappa*a_{L2}+b_{L2}&, \kappa_{L1}<\kappa<=\kappa_{L2} \\
       \kappa*a_{Exceed L2}+b_{Exceed L2}&, \kappa_{L2}<\kappa<=\kappa_{roof} \\
      \eta_{max} \text{ or } \zeta_{max}&, \kappa>\kappa_{roof} \label{eqn:roofline} 
    \end{cases} 
% \text{where}&\ \kappa_{i} = \frac{\chi_{i}}{m_{i}} 
% \label{eqn:kapa}    
\end{align}


\begin{align}
    p &=\frac{\eta}{\zeta} \label{eqn:power}
\end{align}

\begin{comment}
The performance roofline model~\cite{roofline_1st} and energy roofline model~\cite{roofline_energy} are important tools to evaluate computational platforms in performance (in instructions per unit time, denoted as $\eta$) and energy efficiency (in instructions per unit energy, denoted as $\zeta$), respectively. Both of them are determined by the intrinsic property of software, i.e., the operational intensity (which refers to instructions per memory access, denoted as $\kappa$). 


\shuhao{
It's worth noting operational intensity $\kappa$ can be Uniquely determined by specific stream compression software, and it is equal for big cores and little cores due to the ISA-sharing.
However, asymmetric cores lead to varying performance ($\eta$) and energy efficiency ($\zeta$) under the same $\kappa$, as they lead to different growth rates and intercepts in Equation~\ref{eqn:roofline}. These core-specific parameters can be acquired by using a benchmark program similar to \cite{roofline_cache}.
In addition, by considering the performance factor $\eta$ and energy efficiency factor $\zeta$ together in Equation~\ref{eqn:power}, we can estimate the \emph{power} consumption (denoted as $p$, in the unit of Watt) under given $\kappa$.
}
\end{comment}




% By physics law, energy is the production of power and time. Thus, we have Equation~\ref{eqn:energy_s} to bridge latency and energy consumption. 
% 


\textbf{Model Instantiation}
We use 3-step parallel tcomp32 as an example to illustrate the model instantiation, and algorithm details are presented in our technical report~\cite{}.
We consider fine-grained parallel compression variants
(with the granularity of 128-bit tuples).
There are four steps of model instantiation of our cost model. 


First,
% \subsection{Roofline Models}
% \label{subsec:roofline}

Second, to estimate the computation latency $C_{Xcores}^i$, we read the number of instructions
for per tuple in each step ($I_i$) can be obtained from
perf events~\cite{amp_perf}, and use the roofline model to calculate the power factor $p_{Xcores}^i$ and performance factor $\eta_{Xcores}^i$. As 4 32-bit words are processed separately for each tuple in tcomp32 and there is no lookup table, the operational intensity for each step in roofline models can be simply considered as $\frac{I_i}{4}$. 
To rule out the contingency, the $I_i$ is read after accumulated processing on a relatively large number of tuples (e.g, 10,000) and use the average value of them.

Third, we calibrate the communication overhead $In_{Xcores}^i$ and $Ia_{Xcores}^i$ per tuple with the existing
calibration method~\cite{sp_briskstream}. For some steps, the communication overhead is workload-dependent. We adopt the same approach
as profiling the number of instructions discussed above.

Forth, we can estimate the total overhead in latency $L$ and energy $E$. We can calculate $L_{Xcores}^i$ in Equation~\ref{eqn:latency_s} for $i=0,1,2$, and use them in Equation~\ref{eqn:latency} to get the $L$. The $L_{Xcores}^i$ is also used together with power factor $p_{Xcores}^i$ (acquired in the first step by roofline models) to compute 
step energy consumption $E_{Xcores}^i$ in Equation~\ref{eqn:energy_s}, which is finally sum up in Equation~\ref{eqn:energy} to predict the total energy consumption $E$.



It is worth noting that all enabled cores contribute a part to the power consumption. For instance, if the power consumption of running Step 0 on a big core is 1W as estimated in roofline models, and 2 big cores are enabled, we have $p_{big \ cores}^0=2W$.



\textbf{Model Evaluation}

%\shuhao{We only need to profile relevant statistics on an arbitrary core once for a given compression job.}
% The instantiation phase can ignore replica $t_{2}$, as it shares the same model parameters such as $\lambda$ with $t_{0}$.
%  Therefore, we only consider the pipelined $t_{0}$ and $t_{1}$ here and allow them to be mapped to the core $c$ and $c'$ of the rk3399 processor, respectively ($c,c'\in \{0,1,2,3,4,5\}$).

%First, we instantiate the performance and energy roof lines on AMP, by using a benchmark program similar to \cite{roofline_cache}, and then profile the growth rates and intercepts in Equation~\ref{eqn:roofline} for both big cores and little cores.
% In this step, a scanning of $\kappa$ is required and  do this.

% , and existing researches to this problem such as  are applicable here
% and finally fit Equation~\ref{eqn:roofline}. 
%\shuhao{Existing work such as~\cite{algo_plf0,algo_plf1} are applicable here for the piecewise linear fitting of roof lines. Be more specific. What do you mean here??}
\begin{comment}
\subsection{Model-guided Task Scheduling}
% To demonstrate the model instantiation, 
% We start with the instantiation procedure of the cost model, and then illustrate how we find an optimal scheduling plan $p_{opt}$ by the guidance of instantiated cost model. 
% We use the running example shown previously in Figure~\ref{fig:tcomp32_replica} to illustrate how we find an optimal scheduling plan $p_{opt}$.
% For simplicity, we concentrate on scheduling the pipelined $t_{0}$ and $t_{1}$ and allow them to be mapped to the core $c$ and $c'$ of the rk3399 processor, respectively ($c,c'\in \{0,1,2,3,4,5\}$).
% \subsubsection{Determine the Optimal Scheduling Plan}
% After we have completed the instantiation, 
With the instantiated cost model, we search the $p_{opt}$ by enumerating all possible plans.
For each plan $p_{enum}$ enumerated, we first predict the $l$ and $\eta$ on all of its tasks, according to Equations~\ref{eqn:roofline} and ~\ref{eqn:latency}, and then check whether constrains in Equations~\ref{eqn:toatlLat}-\ref{eqn:amountC} can be met. 
If so, we continue to predict energy consumption of tasks by Equation~\ref{eqn:epsilon} and get the $E$ of $p_{enum}$ by the accumulation of them; if not, we just ignore $p_{enum}$ and continue search. 
After the estimation, we will find the plan with minimal $E$ and meet all of the limitations, which is exactly the $p_{opt}$ we are searching for. 
We adopt dynamic programming~\cite{algo_dp_1954} to speed up the plan searching as different plans have identical scheduling targets for subsets of tasks.
\end{comment}
%Upon these calibrations are done, we can evaluate a \emph{scheduling plan} on given data set in terms of energy and latency by just inputting its $I$. During the dynamic-programming-based enumeration of \emph{scheduling plans} in Algorithm~\ref{alg:scheduler}, we use Equation~\ref{eqn:epsilon}  and~\ref{eqn:latency}  to estimate energy and latency of each \emph{task}, and then predict the corresponding behavior of the whole plan.



==> Sections/backup/6_exp.tex <==
\iffalse
% \shuhao{@Xianzhi, merge the following discussion into your experimental analysis.}
\begin{comment}
\begin{myitemize}
    \item \textbf{ILP space} (i.e., instruction density): The tcomp32 algorithm is the most instruction-bound among the three algorithms, 
    because it requires both arithemetic calculations and the \emph{AND/OR} operations.
    %\mynote{ Which is caused by unaligned I/O}. 
    The tdic32 algorithm consumes less ILP space as it does not require massive computation.
    %too much math calculation, 
    In contrast, lz4 consumes the least ILP space because it requires neither compound math calculation nor unaligned I/O.
 %   while lz4 is the least as it requires neither compound math calculation nor unaligned I/O.
    \item \textbf{MLP space} (i.e., memory-access density): 
    The lz4 algorithm is the most memory-bound algorithm because of its hash tabling and \emph{looking-back} search.
    tdic32 consumes less MLP space, as it  does not need to backward search the memory though it still maintains a hash table. The least MLP space-consumed algorithm is  tcomp32, as it involves neither the hash table nor the backward search.
\end{myitemize}
\end{comment}
\begin{comment}
\textbf{1) tcomp32} as we introduced in Section~\ref{subsec:decom_practice}. 
\textbf{2) lz4}~\cite{comp_lz4} is a widely-used LZ77-based~\cite{comp_lzFamily} compression. 
It uses a hash table to replace the traditional \emph{dictionary} of LZ77, which is illustrated in Algorithm~\ref{alg:lz4}.
%, so it is much faster than LZ77.
\textbf{3) tdic32} is a simplified variable length coding by the hybridization of two above, as it borrows the hash table from lz4 and uses a memory I/O pattern similar to tcomp32 (i.e., per 32-bit single symbol). The frequently-showed symbols are encoded with their hash index (which is always shorter). Those not found in hash table are encoded by their original values together a one-bit indicator (which means longer encoding). We present its details in Algorithm~\ref{alg:tdic32}. 

\begin{myitemize}
        \item [\textbf{Q1}] How does \design compare against alternative solutions in handling real-world work load?
    \item [\textbf{Q2}] 
    %Whether the cost model in \design is correct?
    Can the cost model in \design make correct prediction?
    \item [\textbf{Q3}] 
    What effect do different system settings have on the results of parallel compression?
    %How will different system settings affect the outcome of parallel compression?

    \item [\textbf{Q4}] 
    What effects do workload characteristics have on performance metrics?
     \item [\textbf{Q5}] 
    What are the overheads and benefits of \design's key factors (i.e., fine-grained decomposition, asymmetric core awareness, and asymmetric communication awareness)?
    
    %What are the impacts of work load characteristics on the performance metrics?

    %\item [\textbf{Q5}] How will the 6 mechanisms interact with different hardware configuration?
   %\item [\textbf{Q5}] How will our solution work on future AMP platform?
\end{myitemize}
\end{comment}
\xianzhi{copy tstream}

%To answer \textbf{Q5}, we perform sensitivity studies on the core frequencies in Section~\ref{subsec:hardware_sens}. Finally, we imagine and modelize a scaling-up AMP, the Processor-X, and conduct the simulation on it in Section~\ref{subsec:simulation} to answer \textbf{Q6}.

\fi
\section{Experimental Analysis}
\label{sec:evaluation}
The main object of our experiments is to comprehend the behavior of {\design} on AMP. Specifically, we seek answers to the following questions.
\begin{myitemize}
    \item [\textbf{Q1}] Whether the cost model in \design is correct?
    \item [\textbf{Q2}] How does \design compare against alternative solutions in handling real-world wok load?
    \item [\textbf{Q3}] How will different system settings affect the outcome of parallel compression?
    \item [\textbf{Q4}] What are the impacts of work load characteristics on the performance metrics?
    %\item [\textbf{Q5}] How will the 6 mechanisms interact with different hardware configuration?
   %\item [\textbf{Q5}] How will our solution work on future AMP platform?
\end{myitemize}

In the following, we firstly introduce our methodologies Section \ref{subsec:exp_set_up}. Then, we exam our cost model in Section \ref{sucsec:confirmation} to answer \textbf{Q1}
. We present the result of handling different real-world work load in Section \ref{subsec:e2e} to answer \textbf{Q2}. To answer \textbf{Q3}, we adjust the {$L_{set}$} from loose to tight to examine the adaptivity of each mechanism in Section \ref{subsec:system_sens}. 
In Section \ref{subsec:workload_sens}, we evaluate the impact of varying
workload configurations using the synthetic workload to answer \textbf{Q4}.
%To answer \textbf{Q5}, we perform sensitivity studies on the core frequencies in Section \ref{subsec:hardware_sens}. Finally, we imagine and modelize a scaling-up AMP, the Processor-X, and conduct the simulation on it in Section \ref{subsec:simulation} to answer \textbf{Q6}.
\subsection{Experimental Setup}
\label{subsec:exp_set_up}

\textbf{Mechanisms to be Examined.}
We will compare the following 6 mechanisms in handling the prallelized lz4, tcomp32 and tdic32 algorithms:
\begin{myitemize}
    \item \textbf{AMP-aware compression with all mechanisms (ACAM)}. The fully-functional {\design} as Section \ref{sec:overview} introduced.
    \item \textbf{Operating System scheduling (OS)}. The parallel \compress will be scheduled by the linux 5.10 kernel as threads. Since we disabled the DVFS~\cite{amp_DVFS1}  and let all cores running at highest frequency for low switching latency in running parallel compression, the major approach of the OS is the EAS.
    \item \textbf{Round Robin (R\&R)}. The compression \emph{tasks} will be scheduled under a round robin manner, i.e., sequentially mapped to each core.
    \item \textbf{Big-core Only (BO)}. \emph{Tasks} will be randomly scheduled to the little cores of rk3399 (core0 to core3), and big cores (core4 to core5) will be idle.
    \item \textbf{Little-core Only (LO)}. Parallel \compress will be randomly scheduled to the big cores of rk3399 (core4 to core5) and little cores (core0 to core3) will be idle.
    \item \textbf{\design in NUMA style (NS)}. Similar to {\textbf{ACAM}}, but use a NUMA-distance model~\cite{sp_briskstream} instead of \emph{asymmetric communication} model, so the polarity in core communication (i.e., the $\rho$ in  Equation \ref{eqn:tau_fetch}) will be ignored.
\end{myitemize}

 
 
\textbf{Performance Metrics.}
\label{subsec:performance_metrics}
Throughout this study, we focus on three important performance
metrics of streaming applications as follows. First, the
\textbf{Energy Consumption} is the factor directly to our optimization goal, and it considers the $E_{job}$ in Table \ref{reftab:symbols}\mynote{Noting we will exclude the static energy consumption by the hardware and software environment, and present the exact $E_{job}$ casuesd by studied mechanisms.}. To avoid the accidential factors, we will run 100 times of each compression job and use their averaged $E_{job}$  as the presented {energy consumption}.
Second, \textbf{Latency Violation} describes how a mechanism can meet the latency restriction in Equation \ref{eqn:toatlLat}, and the total failures (i.e., when $L_{job}>L_{set}$) of the 100 running will be recorded. 
%Third, \textbf{Core Overload} describes the assurance to Equation \ref{eqn:amountC}, and we will also sum up the the failure to this issue of all running.

Optimizing algorithms for all three performance metrics is
difficult, as these metrics are all useful in different
use cases but sometimes conflict with each other. To be practical for achieving our research goals, an optimal mechanism should have following properties:
\begin{myenumerate}
    \item When \textbf{\emph{there is}} space for energy-saving, i.e., the {$L_{set}$} by user is relatively loose, it can achieve the least {energy consumption}.
    \item It's {latency violation} should be zero \textbf{\emph{anytime}}, even when encountering a tight but possible {$L_{set}$}.
    %\item It's \textbf{\emph{Core Overload}} should also be zero \textbf{\emph{anytime}}.
\end{myenumerate}

It is worth noting that \textbf{ACAM} and \textbf{NS} lead to similar or even the same  outcome of {energy consumption}, as they share most equations in Section \ref{sec:costmodel} for estimation, and both of them use Algorithm \ref{alg:scheduler} for decision-making. However, whether considering the $\rho$ leads to different properties of {latency violation}.   

\textbf{AMP platform.}
 We use the Radxa Rockpi 4a~\cite{amp_rockpi4} single board computer (SBC), with specifications in Table \ref{tab:rockpi}.
This platform is equipped with one rk3399 AMP processor, as we introduced in Section \ref{subsec:amp_intro}. By default, each cores will run at its highest frequency for better real-time response to stream data (i.e., 1.8GHz for big cores and 1.416GHz for little cores).

\textbf{Benchmark Workload.}
\label{subsec:workload}
Four data properties including 1) \emph{vocabulary duplication}s\mynote{As the lz4, tcomp32, and tdic32 share a 32-bit reading of symbols, we can define data more than 32 bits as the \emph{vocabulary}, while that less or within 32 bit as \emph{symbol}}~\cite{comp_lzFamily}, 2) \emph{dynamic range of the symbol}~\cite{comp_baseDelta,comp_elias}, 3) \emph{symbol entropy}~\cite{comp_survey_huffman} and 4) arrival rate~\cite{comp_tersecades,sp_intra_exp} can affect the execution of \compress algorithms, and therefore have impacts on the performance of the whole system. Specifically, we consider three real-world work load including both text-stream and binary-stream, and we also include a synthetic work to comprehensively evaluate
the impact of varying workload properties. The workload used by us are as follows.
\begin{myitemize}
 \item \textbf{Sensor}~\cite{ds_sensor} is a full-text stream data generated by automated sensors. Packing in a XML format with only ascil code, its most compressible part lies in the \emph{symbol entropy}. Besides, the XML pattern can also lead to some \emph{vocabulary duplication}.
  \item \textbf{Rovio}~\cite{sp_rovio} continuously monitors the user actions of a
given game to ensure that their services work as expected, and is packed in $<64-bit\ key, 64-bit \ payload>$. Its high Key duplication according to prior work~\cite{sp_intra_exp} leads to much \emph{vocabulary duplication}.
 \item \textbf{Stock}~\cite{ds_stock} is a real-world stock exchange data set packing in  $<32-bit \ key, 32-bit\ payload>$ binary format. Unlike the \textbf{Rovio}, its key duplication is much lower so it is harder to compress.
 
  \item \textbf{Micro}~\cite{sp_intra_exp} is a synthetic workload used by prior work, and we also adapt it to tune the workload
characteristics. Specifically, different parameters in \textbf{Micro} leads to different 
vocabulary duplication, symbol entropy, dynamic range and arrival rate.
\end{myitemize}

For the simplicity, we make all workload be pre-loaded to main memory in 32-bit aligned size 9328000 byte (if not otherwise indicated), so there is no extra pre-processing in loading data. 
\subsection{Performance Model Evaluation}
\label{sucsec:confirmation}
\begin{comment}
The \model should be able to reflect the physical process of \compress without too much distortion. According to Section \ref{sec:models}, the linear or piecewise linear Equations \ref{eqn:roofline2}, \ref{eqn:tau_run} and \ref{eqn:tau_fetch} are the key to the whole model. Therefore, we examine their fitness in this subsection.

\subsubsection{The Fitness of Roof Lines (Equation \ref{eqn:roofline2})}
We check the piecewice linearity of the roof line model on AMP here, and the we use a benchmark program similar to \cite{roofline_cache} to do the \emph{scanning} of $\kappa$, which is the same as the term IPM (instructions per memory access) by existing work. After the $\kappa$ scanning, we use the results (i.e., the $\eta$ or the $\zeta$) to do least-squares-method-based piecewise fitting. The fitting results of performance roofline (i.e., $\kappa$ to $\eta$) and energy roofline (i.e., $\kappa$ to $\zeta$) are presented in Figure \ref{fig:perroof} and \ref{fig:engroof} respectively, and the unit of $\eta$ and the $\zeta$ are MINTOPS (mega integer operations per second) and MINTOPJ (mega integer operations per joule) respectively. The results show a good 
piecewice linearity for both of them.
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Fitting/FIT_of_MINTOPS.pdf}
    \caption{The fitting result of performance roofline}
    \label{fig:perroof}   
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Fitting/FIT_of_MINTOPJ.pdf}
    \caption{The fitting result of energy roofline
    }  \label{fig:engroof}   
\end{figure}
\subsubsection{The Fitness of Latency (Equation \ref{eqn:tau_run} and \ref{eqn:tau_fetch})}
We consider a two-stage and one-replica (2S1R) tdic32 \compress shown in Figure \ref{fig:dag_tdic32} as the example. In this case, we have the $\mu_{0,0,j}$ and $\mu_{1,0,j'}$
to schedule, and as all little cores (core0 to core3) and all big cores (core4 to core5) are symmetric respectively, we have four scheduling plans in total: the LL, LB, BL, BB, which mean assign $j$ and $j'$ to little core (L) or big core (B) respectively. The \textbf{Rovio} data set is used here, and we let the size of data (i.e., the $I(-1,-1)$) changing from small to large. The resulted $\tau^{run}$ and $\tau^{fetch}$  along with their fiting lines are shown in Figure \ref{fig:tao_run_tdic32} and \ref{fig:tao_fetchtdic32}. Both of them have a good linear correlation at about 99\% here, so the linear latency equations are correct.

Besides the linearity for each case, we can also find that the $\tau^{fetch}$ for \emph{inter-cluster} communication (i.e., the LB or BL in Figure \ref{fig:tao_fetchtdic32}) is always higher than \emph{intra-cluster} communication, and the LB line is specifically the highest, which confirms the polarity factor {$\rho$}.

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Verification/2s1rtdic32.pdf}
    \caption{The 2S1R tdic32 example}  \label{fig:dag_tdic32}   
\end{figure}
 
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Fitting/tdic32_tao_run.pdf}
    \caption{The fitting result of $\tau^{run}$}
    \label{fig:tao_run_tdic32}   
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Fitting/tdic32_tao_fetch.pdf}
    \caption{The fitting result of $\tau^{fetch}$}  \label{fig:tao_fetchtdic32}   
\end{figure}
\subcompact
\end{comment}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/Verification/2s1rtdic32.pdf}
    \caption{The 2S1R tdic32 example}  \label{fig:dag_tdic32}   
\end{figure}
In this section, we evaluate the accuracy of our performance
model in \design.  
%Specifically, we examine the correctness of \model in predicting the energy ($E_{job}$), latency($T_{job}$) for the whole \compress, and  core load ($W_j$) for each core. We first evaluate the estimation of a simple parallel \compress, the two-stage and one-replica (2S1R) tdic32 handling rovio \compress shown in Figure \ref{fig:dag_tdic32} as the example. In this case, only two \emph{execution units} $\mu_{0,0,j}$ and $\mu_{1,0,j'}$ are involved. We list the predicted and read value of $E_{job}$, $T_{job}$, and  $W=\sum_{j}W_j$ under four different pairs of $(j,j')$. 

Specifically, we examine the correctness of cost model in predicting the energy ($E_{job}$) for the whole compression. We first evaluate the estimation of a simple parallel compression, the two-stage and one-replica (2S1R) tdic32 handling \textbf{Rovio} compression shown in Figure \ref{fig:dag_tdic32} as the example. In this case, only two \emph{tasks} $t_0$ and $t_1$ mapped to core $j$ and $j'$ respectively are involved. We list the predicted and measured value of $E_{job}$ under four different pairs of $(j,j')$, which covers all circumstances if we treat the same type of cores equal and the same. 

To validate the overall effectiveness of our performance
model, we show the relative error associated with estimating  $E_{job}$ by our analytical model. Specifically, we have 
{$relative\_error=\frac{|E_{job}^{mes}-E_{job}^{est} |}{E_{job}^{mes}}$
}, where {$E_{job}^{mes}$} is the measured value and {$E_{job}^{est}$} is the estimated value by our model. 

The model accuracy evaluation of all algorithms under
the optimal \emph{scheduling plan} is shown
in Table \ref{tab:correctness2}. Overall, our model can have correct prediction of $E_{job}$, which also proves its correctness in latency prediction, according to Equation \ref{eqn:epsilon}. 
\begin{table}[h]
\caption{Average prediction and real value of of $E_{job}$ for 2S1R tdic32, the unit is Joule}
\label{tab:correctness}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\diagbox{variable}{$(j,j') pair$}    & (0,1) & (0,4) & (4,0) & (4,5) \\ \hline
Estimated $E_{job}$ &5.2220&4.7181&4.9286&6.3701       \\ \hline
Measured $E_{job}$  &5.4317&4.5603&4.8573&6.2628       \\ \hline
Relative error &0.0386&0.0345&0.0146&0.0171\\ \hline

\end{tabular}%
}
\end{table}

\begin{table}[h]
\caption{Average prediction and real value of $E_{job}$ for optimal \emph{scheduling plans}, the unit is Joule }
\label{tab:correctness2}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\diagbox{variable}{method}    & lz4 & tcomp32 & tdic32 \\ \hline
Estimated $E_{job}$ &4.4277&3.6933&4.1218     \\ \hline
Measured $E_{job}$  &3.8833&4.0466&4.4783    \\ \hline
Relative error &0.1402&0.0873&0.0796\\ \hline

\end{tabular}%
}
\end{table}

\begin{comment}


\begin{table}[h]
\caption{Average prediction variable and their real value, the unit is Joule for  $E_{job}$, us for $T_{job}$ , and mega integer operations per second for $W$}
\label{tab:correctness}
\resizebox{.95\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\diagbox{variable}{$(j,j') pair$}    & (0,1) & (0,4) & (4,0) & (4,5) \\ \hline
Estimated $E_{job}$ &5.3220&4.6181&4.9086&6.3701       \\ \hline
Measured $E_{job}$  &5.4317&4.4783&4.8573&6.2628       \\ \hline
Estimated $T_{job}$ &1466104&13952972&1555085&694507       \\ \hline
Measured $T_{job}$  &1460893&13960129&1544641&694055       \\ \hline
Estimated $W$ & 1481.6374& 1618.4015&1894.7542& 2916.8370      \\ \hline
Measured $W$  & 1473.7259& 1612.3751&1890.5641& 2918.6827      \\ \hline
\end{tabular}%
}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/error.pdf}
    \caption{The relative error of all algorithms}  \label{fig:errr}   
\end{figure}
\end{comment}
\subsection{End-to-end Evaluation of Real-world Data Set}
\label{subsec:e2e}
The end-to-end evaluation use 6 above mechanisms to handle the real-world workload \textbf{Sensor}, \textbf{Rovio}, and  \textbf{Stock}, with fine-grained parallel of lz4, tcomp32 and tdic32. 

\textbf{Compare the Energy Consumption}.
We present the energy consumption under relatively loose {$L_{set}$} for each method in Figure \ref{fig:eng_total}, and there is an abundant space to save energy for each mechanism. In this comparison, \design including \textbf{ACAM} and \textbf{NS} can always outperform others, and save up to 53.23\% energy (in the lz4-\textbf{Stock} case compared with \textbf{BO}). Two major causes lead to such results. First, the best scheduling plan in reality is to synthetically use both big cores and little cores. Such chance for \textbf{LO} and \textbf{BO} are never, \textbf{R\&R} and \textbf{OS} are sometimes, but \textbf{ACAM} and \textbf{NS} are \textbf{always}. 
Next, \textbf{NS} have the results similar to \textbf{ACAM}. By further analysing the system log generated by \textbf{NS}, we find its wrong predicting of latency
 does not change the energy consumption sorting order of each \emph{scheduling plan}, which explains why it can still achieve least energy consumption. 
%Next, \textbf{NS} still have the acurate modeling for energy, so it is nearly the same as \textbf{ACAM} in terms of energy consumption. The system log generated by \textbf{NS} shows that although it has wrong prediction of energy due to the polarity-unawareness in predicting $\tao_{fetch}$, which also affects the energy prediction in Equation \ref{eqn:epsilon}, it's estimation for each \emph{scheduling plan} still follows the right sorting order. Therefore, it can also choose the most energy saving plan.

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/total/energy.pdf}
    \caption{The E-to-E results of energy consumption}  \label{fig:eng_total}   
\end{figure}

\textbf{Compare the Latency Violation}.
We present the worst latency violation for each method in \ref{fig:vio_total}, and only \textbf{ACAM} and \textbf{BO} can achieve \emph{zero} violation even under the worst cases. Other mechanisms, especially the \textbf{LO} and \textbf{NS}, fail to meet some certain latency due to their insufficient allocation of cores' computation power. We will further explore the
insufficiency of \textbf{LO} and \textbf{NS} in Section \ref{subsec:system_sens}

\begin{comment}


The fail of \emph{LO} is because it can not utilize the more power big cores under tight {$L_{set}$}, while that of \emph{NS} is caused by its unawareness of asymmetry core communication. For instance, when {$L_{set}=1.8 s$}, there is some \emph{scheduling plan} with no more than 6 J energy consumption (which seems to be the 'most energy saving one'),
but its latency in reality can exceed the constrain as it involves \emph{inter-cluster} communication with high $\rho$ in Equation \ref{eqn:tau_fetch}. Unaware to the $\rho$, \textbf{NS} maintains the delusion that the {$L_{set}$} will never be exceed under such plan. 
Therefore, it repeatedly choose this plan in the 100 running, which leads to 100\% latency violation then.

How 
and \emph{NS} also thinks its latency is below 1,8s. However, as there are  in such plan, its latency in reality can exceed the constrain. By repeating such error in the 100 running, \emph{NS} produces the 100\% latency violation then. 
\end{comment}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/total/violation.pdf}
    \caption{The E-to-E results of latency violation}  \label{fig:vio_total}   
\end{figure}
\begin{comment}
\textbf{Compare the Core Overload}.
We present the worst core overload for each method in \ref{fig:overload_total}, and \textbf{ACAM} and \textbf{NS} can always prevent it due to their estimation of \emph{scheduling plans}.
Meanwhile, the \textbf{R\&R} has nearly zero overload as it is an \emph{absolutely fair} way to assign both the big cores and little cores, the \textbf{LO} has also low overload as the amount of little core is relatively abundant. However, the overexploitation of relatively rare big cores leads to high core overload in \textbf{OS} (which sometimes tries to \emph{steal} threads from little cores and reschedule them to big cores during the \emph{EAS}) and \textbf{BO} (which only uses the big cores).  
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/total/overload.pdf}
    \caption{The E-to-E results of core overload}  \label{fig:overload_total}   
\end{figure}

\end{comment}
\emph{Summary}. The end-to-end estimation in real-world workload present that the {\design} with all mechanisms (\textbf{ACAM}) outperforms other, as it leads to least energy consumption and zero latency violation.
\subsection{System Sensitivity Study}
\label{subsec:system_sens}
\textbf{Sensitivity to {$L_{set}$}}.
The trade-off between energy consumption and latency is varying to different application scenarios. When the real-time requirements is loose, users may want more energy reduction, otherwise, they may order the parallel \compress system to do its best in fast processing and avoid latency violation. Therefore, we conduct experiments on handling \textbf{Rovio} by parallel lz4 with changing $L_{set}$ in this section, and the results of performance metrics are shown in Figure \ref{fig:rovio_lz4}.

 Unlike the \textbf{OS}, \textbf{R\&R}, \textbf{BO}, \textbf{LO}, which have the relatively fixed energy consumption line, the \textbf{ACAM} is an \textbf{adaptive} method to different system parameter $L_{set}$. The \textbf{NS}, although also tries to be \textbf{adaptive}, fails to meet some \emph{critical point} of $L_{set}$ and has the terrible twitter in its violation line. This is caused by its blindness to the asymmetric core communication (i.e., the $\rho$ in Equation \ref{eqn:tau_fetch}). For instance, when {$L_{set}=1.8 s$}, there is some \emph{scheduling plan} with no more than 6 J energy consumption (which seems to be the 'optimal plan' for the least energy consumption),
but its latency in reality can exceed the constrain as it involves \emph{inter-cluster} communication with high $\rho$ in Equation \ref{eqn:tau_fetch}. Unaware of the $\rho$, \textbf{NS} maintains the delusion that the {$L_{set}$} will never be exceed under such plan. 
Therefore, it repeatedly choose this plan in the 100 running, which leads to 100\% latency violation then.
 This result reminds us the importance of asymmetric core communication again.
 
 \textbf{Sensitivity to Batch Size}.
 The batch size (i.e., $I_{job}$) can determine the base line of \textbf{Energy Consumption}, but affects much less to the \textbf{Latency violation} \mynote{As {$L_{set}$} is typically synchronously growing with batching size, and core overload is determined by intrinsic properties of data and algorithm}. Therefore, we study the energy consumption of running different batch sizes, and the tdic32-\textbf{Rovio} is tested here in Figure \ref{fig:eng_bsize}. For each mechanisms, the energy is approximately linear to the batching size, though with different growth rate. Specifically, \textbf{ACAM} and \textbf{NS} outperform others, and the energy reduction is much more significant under larger size. Back to the \model model, we can find following reasons for the explanation. First, the energy is estimated by the Equation \ref{eqn:epsilon}, where $\eta$ and $\zeta$ are irrelevant to batching size  and $\tau$ is linear to it by Equation \ref{eqn:latency} to \ref{eqn:tau_fetch}. Next, \textbf{ACAM} and \textbf{NS} have the AMP-awareness and \compress-awareness in both $\eta$ and $\zeta$, and they can always choose the least value of {$\frac{\eta}{\zeta}$} if possible.
 \begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/batchSize/ene.pdf}
    \caption{Impacts of different batch size}  \label{fig:eng_bsize}   
\end{figure}

 \textbf{Sensitivity to Core Frequencies}.
Different frequency of AMP hardware lead to different power and latency, therefore they have different impacts of the energy consumption. We set different frequencies for the lz4-\textbf{Rovio} \compress job, and demonstrate the result in Figure \ref{fig:eng_freq}. Similar to batching size, the core frequency mainly affects the energy consumption. 

The \design implemented as \textbf{ACAM} and \textbf{NS} still outperform others in changing frequencies.
And for each mechanisms, lower frequency is not equal to low energy consumption in Joule, and this is even on the total contrary for \textbf{LO}, \textbf{R\&R}, \textbf{NS} and \textbf{ACAM}. Although lower frequency can absolutely lead to low power (measured in Watt) according to state-of-art~\cite{amp_DVFS1,amp_DVFS2,amp_DVFS3}, their increased latency in \compress is even more significant and cause higher energy consumption sometimes (especially for running at little cores). This is why we should synthetically consider the roof lines and latency in Equation \ref{eqn:epsilon}. 
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/freq/ene.pdf}
    \caption{Impacts on energy consumption of different frequencies}  \label{fig:eng_freq}   
\end{figure}
\etoePic {rovio/lz4} {Impacts of changing {$L_{set}$}} {fig:rovio_lz4}

\subsection{Workload Sensitivity Study}
\label{subsec:workload_sens}
Workload characteristics of data streams being compressed vary
significantly among applications. Specifically, the different vocabulary duplication, symbol entropy can dynamic range will mainly lead to different \textbf{Energy Consumption}, while varying arrival rate of streaming data affects both the \textbf{Energy Consumption} and \textbf{Latency Violation}. In this section, we use \textbf{Micro} to tune them respectively, then record and analyze the performance metrics influenced by them.
%\mynote{The metrics hardly be affected will be skipped in our discussion}.

\textbf{The Vocabulary Duplication}.
We control the duplication of 64-bit vocabulary, and other parameters in \textbf{Micro} will be fixed. As the lz4 algorithm is most sensitive to vocabulary duplication, we choose the parallel lz4, we evaluate it here for this issue in Figure \ref{fig:v64}.

Two insights are observed here. First, a middle vocabulary duplication leads to most energy consumption for all mechanisms, due to the middle rate of both 'match' and 'mismatch' (i.e., middle {$\kappa$} ) means high {$\frac{\eta}{\zeta}$} in Equation \ref{eqn:epsilon}. 
%Next, increasing vocabulary duplication can relieve the core overload for big cores, as the software is more memory bound then, which means lower $\kappa$ and $\eta$ according to Equation \ref{eqn:kapa} and \ref{eqn:roofline2}. 
Next and most importantly, the \textbf{ACAM} can achieve least energy consumption a in dealing with changing vocabulary duplication.
\wsPic {v64} {Impacts of different vocabulary duplication} {fig:v64}

\textbf{The Symbol Entropy}.
We control the entropy of 32-bit symbol, fixing other parameters in \textbf{Micro}, and the most entropy-sensitive algorithm tdic32 is tested here in Figure \ref{fig:e32}. We can find the little cores and big cores have different or even contradict response to increasing entropy, which is caused by different task-core affinity. However, the little cores seems to be more decisive to the plans that use all cores like \textbf{R\&R}, \textbf{OS}, \textbf{NS} and \textbf{ACAM}, due to their higher quantity. Besides, it is obvious that \textbf{ACAM} is always the best in changing symbol entropy.
\wsPic {e32} {Impacts of different symbol entropy} {fig:e32}

\textbf{The Dynamic Range}.
We evaluate the most dynamic-range-sensitive algorithm tcomp32 here in Figure \ref{fig:r32}, by scanning the dynamic range of 32-bit symbol from low to high and fixing other parameters. With the growing range, the tcomp32 should do more $log2$ computation, which involves higher $\kappa$ and $\tau$. According to Equation \ref{eqn:epsilon} and \ref{eqn:roofline2}, increased $\kappa$ and $\tau$ leads to more
 energy consumption. Although \textbf{ACAM} still outperforms others, the space for energy reduction is less significant when dynamic range is high.
\wsPic {r32} {Impacts of different dynamic range} {fig:r32}

\textbf{The Arrival Rate}. In Figure \ref{fig:arr}, we adjust the arrival rate of \textbf{Micro} to several \emph{critical points}, which are the upper bound for the capacity of some \emph{scheduling plans}. Apart from this, \textbf{Micro} follows an uniform distribution and is handled by tdic32. There are three key observations: First, when the arrival rate is low (e.g., $0.6*10^6$ bytes per second), all mechanisms except the \textbf{OS} can achieve zero latency violation, perhaps due to more frequent thread switching in \textbf{OS}. Meanwhile, \textbf{ACAM} AND \textbf{NS} can achieve the least energy consumption. Next, the chances for energy saving will no longer exist when the arrival rate is more than the critical point $0.8*10^6$ bytes per second, and \textbf{NS} will over-optimize energy consumption but violate latency requirements at this point. Finally, when arrival rate is too fast at $2*10^6$, no mechanism can perform well in preventing latency violation, as the maximum computation power of the rk3399 is exceeded then. 
\begin{figure}[h]
\centering
\subfigure[Average energy consumption of processing 10M byte, 100 running]{
\includegraphics[width=0.45\columnwidth]{figures/e2e/arrivalRate/eng.pdf} 
}
\subfigure[Total latency violation of processing 10M byte, 100 running]{
\includegraphics[width=0.45\columnwidth]{figures/e2e/arrivalRate/vio.pdf} 
}
\DeclareGraphicsExtensions.
\caption{Impacts of different arrival rate}
\label{fig:arr}
\end{figure}
\begin{comment}


\subsection{Simulation: towards Future AMP}
\label{subsec:simulation}

%More and more top vendors including Intel~\cite{amp_i9_12}, AMD~\cite{amp_amd}, Qualcomm~\cite{amp_sd888}, Hisilicon~\cite{amp_kirin9000}, etc., have been using AMP to build their flag-ship processors. Meanwhile, the application filed of AMP  will extend to personal computers and even data center.

 %It's clear that AMP has a bright future, and we consider the following two aspects for the future AMP.
According to the recent AMP release by some top vendors, like the snapdragon 8 Gen 1(2021)~\cite{amp_sd8g1} by Qualcomm and the 12th generation \emph{Core} Processor~\cite{amp_i9_12} by Intel, we can consider the following two aspects for the future AMP.

\textbf{Cores with Greater Difference}. The more recent AMPs like snap dragon 8 Gen 1~\cite{amp_sd8g1} have more powerful big cores and more energy-efficient little cores than elder release like rk3399, which leads to greater differences between different types of cores. And this tendency will continue for the future. Being aware of this, we assumed a new AMP processor called Processor-X as Figure \ref{fig:processorx} depicts. This processor is nearly the same as rk3399, but has more significant difference between big cores and little cores. Specifically, we assume its performance roof lines as Figure \ref{fig:roofline_x} demonstrates. 

We then use the \textbf{Rovio} data set to simulate how will different mechanisms handle lz4, tcomp32 and tdic32 on the Process-X. The result of energy consumption is shown in Figure \ref{fig:eng_x}, which still confirms the superiority of \design. Moreover, due to the higher performance by Processor-X, the most energy reduction here is about 33\%, which is higher than rk3399 under the same case (about 26\% in Figure \ref{fig:eng_total}). 
\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/processorx/ene.pdf}
    \caption{Energy consumption on Processor-X }  \label{fig:eng_x}   
\end{figure}

\textbf{Cores with Larger Amount}. Another tendency of AMP is the growing amount for both big cores and little cores. For instance, the Intel i9-12900K processor~\cite{amp_i9_12} released in November 2021 has 8 big cores and 8 little cores, which are much more than the rk3399. Therefore, we consider to scale up the mechanisms on Processor-X in this section. For simplicity, we give the following constrains for the scaling-up:  1) we still use the two-cluster model; 2) the band width of CCI-X and the L2 size will also grow to fit into the growing number of cores, and the overhead for communication remains unchanged thus; and 3) the proportion between big cores and little cores will be unchanged.

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/processorx/en3.pdf}
    \caption{Mechanism scaling-up on Processor-X}  \label{fig:eng_xscale}   
\end{figure}
We use the tcomp32 algorithm and \textbf{Rovio} data set to examine the scaling-up of 6 mechanisms on  Processor-X, demonstrating energy consumption results in Figure \ref{fig:eng_xscale}. Since both big cores and little cores are scaled up with the same ratio, we just use the \emph{scale factor} to represent the concrete scaling up. For instance, a scale factor 2 means the targeted machine has twice amount of big cores and little cores compared with the original Processor-X in Figure \ref{fig:processorx} (i.e., with 8 little cores and 4 big cores). Due the more abundant hardware resource, the \textbf{R\&R}, \textbf{OS} and \design (i.e., the \textbf{NS} and \textbf{ACAM}) have more chances to synthetically utilize both the big cores and little cores, which leads to less energy consumption during the scaling up. Besides, the \textbf{NS} and \textbf{ACAM} have even better scaling up due to their full awareness of task-core affinity.
\end{comment}

\subsection{Simulation: towards Future AMP}
\label{subsec:simulation}

%More and more top vendors including Intel~\cite{amp_i9_12}, AMD~\cite{amp_amd}, Qualcomm~\cite{amp_sd888}, Hisilicon~\cite{amp_kirin9000}, etc., have been using AMP to build their flag-ship processors. Meanwhile, the application filed of AMP  will extend to personal computers and even data center.

 %It's clear that AMP has a bright future, and we consider the following two aspects for the future AMP.
According to the recent AMP release by some top vendors, like the snapdragon 8 Gen 1(2021)~\cite{amp_sd8g1} by Qualcomm and the 12th generation \emph{Core} Processor~\cite{amp_i9_12} by Intel, we can consider the following two aspects for the future AMP.

\textbf{Cores with Greater Difference}. The more recent AMPs like snap dragon 8 Gen 1~\cite{amp_sd8g1} have more powerful big cores and more energy-efficient little cores than elder release like rk3399, which leads to greater differences between different types of cores. And this tendency will continue for the future. Being aware of this, we assumed a new AMP processor called Processor-X as Figure~\ref{fig:processorx} depicts. This processor is nearly the same as rk3399, but has more significant difference between big cores and little cores. Specifically, we assume its performance roof lines as Figure~\ref{fig:roofline_x} demonstrates. 

We then use the {Rovio} dataset to simulate how will different mechanisms handle lz4, tcomp32 and tdic32 on the Process-X. The result of energy consumption is shown in Figure~\ref{fig:eng_x}, which still confirms the superiority of \design. Moreover, due to the higher performance by Processor-X, the most energy reduction here is about 33\%, which is higher than rk3399 under the same case (about 26\% in Figure~\ref{fig:eng_total}). 
\begin{figure}
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/processorx/ene.pdf}
    \caption{Energy consumption on Processor-X }  \label{fig:eng_x}   
\end{figure}

\textbf{Cores with Larger Amount}. Another tendency of AMP is the growing amount for both big cores and little cores. For instance, the Intel i9-12900K processor~\cite{amp_i9_12} released in November 2021 has 8 big cores and 8 little cores, which are much more than the rk3399. Therefore, we consider to scale up the mechanisms on Processor-X in this section. For simplicity, we give the following constrains for the scaling-up:  1) we still use the two-cluster model; 2) the band width of CCI-X and the L2 size will also grow to fit into the growing number of cores, and the overhead for communication remains unchanged thus; and 3) the proportion between big cores and little cores will be unchanged.

\begin{figure}
    \centering
    \includegraphics*[width=0.8\columnwidth]{figures/e2e/processorx/en3.pdf}
    \caption{Mechanism scaling-up on Processor-X}  \label{fig:eng_xscale}   
\end{figure}
We use the tcomp32 algorithm and \textbf{Rovio} dataset to examine the scaling-up of 6 mechanisms on  Processor-X, demonstrating energy consumption results in Figure~\ref{fig:eng_xscale}. Since both big cores and little cores are scaled up with the same ratio, we just use the \emph{scale factor} to represent the concrete scaling up. For instance, a scale factor 2 means the targeted machine has twice amount of big cores and little cores compared with the original Processor-X in Figure~\ref{fig:processorx} (i.e., with 8 little cores and 4 big cores). Due the more abundant hardware resource, the \textbf{R\&R}, \textbf{OS} and \design (i.e., the \textbf{NS} and \textbf{\design}) have more chances to synthetically utilize both the big cores and little cores, which leads to less energy consumption during the scaling up. Besides, the \textbf{NS} and \textbf{\design} have even better scaling up due to their full awareness of task-core affinity.
\end{comment}
\subsection{Factor analysis}
\label{subsec:factor_ana}
To understand in greater detail the overheads and benefits of various aspects of \design, we show a factor analysis in Figure~\ref{fig:factor_ene} that highlights energy dissipation and latency violation. 
%\shuhao{use $$formula here$$.}
The \emph{energy dissipation} is tested under loose $L_{set}$, and calculated by 
$$
    energy \ dissipation =
\frac{ E_{j}^{this} - E_{j}^{min}}{E_{j}^{min}}
$$
, where $E_{j}^{this}$ is the energy consumption of this method, and $E_{j}^{min}$ is the theoretical minimum energy consumption according to our cost model.
The \emph{latency violation} is under tight $L_{set}$ as defined in Section~\ref{subsec:exp_set_up}.
Specifically, we start in a pbzip2~\cite{cpmp_bzip2}-like and SMP-aware manner (denoted as \emph{simple}), then add fine-grained decomposition introduced in Section~\ref{sec:decompos} (i.e., \emph{+decom.}), next add asymmetric-core-awareness according to Section~\ref{sec:costmodel} (i.e., \emph{+asy-core., NUMA-AWARE}) and finally end by adding asymmetric-communication-awareness (\emph{+asy-comm.}), which is a fully-functional \design as illustrated in Section~\ref{sec:overview}.  The workload and algorithm for evaluation here is Rovio and tcomp32.
It is worth noting that the \emph{+asy-core.} uses a NUMA-aware modeling~\cite{sp_briskstream} for the core communications, which ignores the $\rho$ in Equation~\ref{eqn:tau_fetch}.


We have the following observations from Figure~\ref{fig:factor_ene}.
First, when decomposing a \emph{simple} method into a fine-grained manner, we can provide opportunities for synthetic utilization of big cores and little cores, which can reduce energy dissipation. However, because these methods continue to treat AMP as an SMP, these possibilities are only occasionally realized. Moreover, ignorance of extra communication overhead can increase latency violation. 
Second, by incorporating the asymmetric core awareness, 
%under the \emph{+asy-core} \cred{???} case, \shuhao{remove the extra space before ``, ''.}
we can always grasp the chances and support varying task-core affinity caused by different operational intensity $\kappa$, which leads to further energy reduction. Nevertheless, due to the thoughtlessness of asymmetric communication, we can over-optimize for energy and violate the tight $L_{set}$ frequently.
Specifically, the \emph{asy-core.} always maintains the delusion that {$L_{set}$} can never be exceeded under some plan which leads to lower energy consumption but involves more inter-cluster communication, then chooses this plan and violate {$L_{set}$} every time.
This result reminds us of the importance of asymmetric communication awareness.
%which is similar to the failure of NUMA-aware scheduling in Section~\ref{subsec:system_sens}.
Third, 
with \design, we can model and evaluate the asymmetric communication well before execution, and thus prevent the latency violation. Furthermore, the remaining energy dissipation by \design is trivial and close to the \emph{relative error} of our cost model presented in Section~\ref{sucsec:confirmation} (i.e., about 10 \%).

\iffalse
\xianzhi{The takeaways from Figure~\ref{fig:factor_ene} are as follows.
First, when decomposing the \emph{simple} into a fine-grained manner, we can provide basic opportunities for synthetic utilization of big cores and little cores, which reduce a part of energy dissipation. However, as the method still treat AMP as SMP, these chances can not be always grasped. Moreover, ignorance of extra communication overhead  leads to slight increase of latency violation. Second, under the \emph{+asy-core.} case, we can always grasp the chances and give proper support for varying task-core affinity in ILP and MLP, therefore leads to further energy reduction. Nevertheless, due to the thoughtlessness of asymmetric communication, we will over-optimize for energy and violate the tight $L_{set}$ frequently (which is similar to the failure of NUMA-aware scheduling in Section~\ref{subsec:system_sens}). Third, when upgraded into \design, we can model and evaluate the asymmetric communication well before execution, and therefore prevent the latency violation. In addition, the remaining energy dissipation by \design is trivial and close to the \emph{relative error} of our cost model presented in Section~\ref{sucsec:confirmation} (i.e., about 10 \%).}
\fi


\begin{figure}[t]
    \centering
    \includegraphics*[width=0.98\columnwidth]{figures/factor_ene.pdf}
    \caption{Factor analysis.
    % \shuhao{One space before (PC-AMP), i.e., +asy-comm. (PC-AMP). Not ``com'', should be ``comm.''}
    %\shuhao{Make this figure more specific to tcomp32. See my following descriptions accordingly.}
    }  
    \label{fig:factor_ene}   
\end{figure}

==> Sections/backup/7_RelatedWork.tex <==
\section{Related Work}
\label{sec:related}
In this section, we review the related work and reveal the limitations that motivate this work.

% \begin{comment}
% \shuhao{
% @Xianzhi. Merge the following.
% Prior researches have studied on improving the theoretical compressibility~\cite{comp_7z}, 
% reducing compressing complexity on single core~\cite{comp_survey_2017, comp_survey_huffman}, 
% accelerating compression~\cite{comp_acc}, and reducing its energy dissipation~\cite{comp_energy_2006}. 
% }
% \end{comment}

% \iffalse
% \textbf{Parallel data compression.}
% \xianzhi{Significant efforts have been devoted in parallelizing compression algorithms at earlier VLSI~\cite{comp_1985}, symmetric multicore processors (SMP)~\cite{comp_para_bzip2, comp_ndzip, comp_para_hsi}, GPU~\cite{comp_pipeline_gpu, comp_lzss_cuda, zhang2021g, comp_gpu_lossy} and FPGA~\cite{comp_lz4_fpga, comp_fp_2010}. 
%  However, neither of them is AMP-aware.  The SMP-based works assume all cores are equal and the same, lacking even the basic awareness of the asymmetry in cores and their communications. The GPU-based or FPGA-based ones are without ISA-sharing, and have more complex control of data and program, which is also unsuitable for AMP.
% }

% \cred{zf here}
% \fi


%Significant efforts have been devoted in parallelizing compression algorithms at earlier VLSI~\cite{comp_1985}, multicore processors~\cite{comp_para_bzip2}, GPU~\cite{comp_pipeline_gpu, comp_lzss_cuda} and FPGA~\cite{comp_lz4_fpga}. 

\textbf{Parallel Data Compression.} 
%Parallelization is usually a good way to reduce time overhead and improve throughput, and can exactly benefits the \compress a lot.
%\shuhao{space after ``, ''.}
% \xianzhi{
% On earlier very large-scale integration (VLSI), Gonzalez Smith et al.~\cite{comp_1985} conducted parallization work perhaps as the beginning.}
%Gonzalez Smith et al.~\cite{comp_1985} showed the parallelism both static and dynamic dictionary on dedicated Very large-scale integration (VLSI) in 1980s, which may be the earliest. 
%From 2000s and then, various parallelism work emerge with the progress of new hardware.
There are many existing works to parallelize data compression algorithms.
On the FPGA, Milward et al.~\cite{comp_2004_tpds} implemented a novel dictionary-based parallel compression implementation, Sano et al.~\cite{comp_fp_2010} achieved float-point data compression, Tian et al.~\cite{comp_waveSz} proposed parallel compression for scientifical data, and Bark et al.~\cite{comp_lz4_fpga} parallelized the lz4 algorithm.
On the GPU, the parallelization of several LZ algorithms~\cite{comp_lzFamily} have been conducted such as \cite{comp_lzss_cuda} and  \cite{comp_mpc_2015}, and Huang et al.~\cite{comp_gpu_lossy} have also parallelized trajectory-specific compression algorithms. Due to the significant difference in hardware architectures, it is unclear how can those works be applied for parallel compression on AMPs.
Researcher have also utilized the Symmetric Multicore Processors (SMPs) for parallel compression: to compress the float-point data~\cite{comp_para_pfc} and to drill the inner parallelism (in a SIMD-like manner) of LZ77~\cite{comp_paralz_2013}. Recently, Knorr et al.~\cite{comp_ndzip} achieved high-throughput of large volumes of scientific data scaling up to 24 threads, and Dua et al.~\cite{comp_para_hsi} compressed the hyperspectral images on supercomputer with a hyper-cube structure. 
Our experiments have shown that SMPs-aware parallelization results in poor performance on AMPs.
% as we discussed previously in Sections~\ref{sec::introdction} and~\ref{sec:background}.
% \begin{comment}
% %amp_web:

% Single ISA Heterogeneous Scheduling:
% Our webpage
% scheduling technique, based on big/little cores with the aid of
% DVFS, is an example of utilizing single-ISA heterogeneous
% systems for optimizing the performance versus energy tradeoff
% [35]. Nvidia’s Kal-El [21] is a single-ISA heterogeneous
% system that integrates four high-frequency cores with one lowfrequency
% core. ARM’s proposed big.LITTLE system [13]
% contains a high-performance Cortex-A15 processor and a
% lower-performance but extremely energy-efficient Cortex-A7
% processor. Without the availability of the big.LITTLE system, 
% in this paper we use the Cortex-A9 and A8 to synthesize such
% a system, and show its advantage in high-performance and
% energy-efficient mobile web browsing. Our prediction-based
% scheduling technique is similar to other recent heterogeneous
% scheduling proposals, such as PIE [30].
% \emph{
% However, instead of
% relying on (micro)architecture- and system-level statistics for
% prediction, we capture the complex behavior of webpage characteristics
% using regression modeling, and accurately predict
% the webpage load time and energy consumption.}


% amp_latency_2017:


% Petrucci et al.’s OctopusMan system is coarse grain — they allocate
% either all slowor all fast cores to an entire service, but never mix
% core types [45]. Their controller selects increasingly larger homogeneous
% con￿gurations of slow or fast cores until it meets the target
% tail latency. They do not describe a scheduler. Section 6.5 compares
% OctopusMan with EETL. EETL uses individual request progress
% and system load to deliver tighter control over power/performance
% tradeo￿s and greater energy savings.


% amp_ai, aysmo:
% AMP thread scheduling There are thread scheduling algorithms
% designed for AMP machines [3, 31, 62]. They schedule threads
% to big or little cores by monitoring their hardware behaviours or
% criticality. WASH [31] proportionally schedules threads to big and
% little cores according to the core capability. COLAB [62] makes
% coordinated core assignment and thread selection decisions based
% on the performance estimation of each thread on different cores, as
% well as identified communication patterns and bottleneck threads.
% Gomatheeshwari et al. [4] utilize a lightweight-deep neural network
% (LW-DNN) to predict the optimal cores for each workload. Compared
% with AsyMo, these works are for general thread scheduling
% at the OS or language virtual machine level. They are unknown of
% the code logic running on each thread, such as the matrix multiplication
% in this paper. Therefore, these schedulers cannot conduct
% block partition for matrix multiplication and then schedules them.
% By comparison, AsyMo partitions blocks first and then schedules
% the sub-block tasks according to the core capability.

% amp_game:
% Thread-mapping. Energy optimization can be performed
% at thread level, in which multiple threads with
% different workloads can be mapped to different types of
% cores. An MPSoC governor for mobile games proposed in
% [22] classifies threads into periodic and aperiodic ones, and
% uses two workload predictors ACR and WMA for them
% respectively. Their experimental results only report energy
% savings from the combined DVFS and thread mapping, and
% it is unclear how much is contributed by thread mapping.
% The work in [16] also explores DVFS in conjunction with
% thread migration for energy savings on big.LITTLE architectures.
% However, it only achieves 3% additional reduction in
% power consumption from thread migration. Part of the reason
% is that the Linux kernel beneath Android for multi-core
% architectures has already implemented a thread scheduling
% algorithm for load balancing, in which the cores with less
% workload will be assigned more threads for running. Given
% the limited benefits, complexities and overhead, we do
% not consider a customized thread-level scheduling in our
% current work.

% \end{comment}

% \textbf{Management of AMP}.
% The approaches to effectively manage the AMP include modeling~\cite{amp_modeling} and predicting~\cite{amp_caloree} of performance/energy, CPI stack~\cite{amp_pie_2011} considering both ILP and MLP and DVFS-collibrated scheduling~\cite{amp_DVFS3, amp_fairness_2020, amp_latency_2017}. Some classical ways, such as PID Control~\cite{amp_latency_2015}, can also aid in the feed-back regulation. 
% Recently, the performance/energy model has been merged into the popular mainline Linux from version 5.0 onwards as the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime}. 
% However, these models treat the software running on AMP as a black box due to the isolation by OS and system-level statistics, which overlooks many optimization opportunities as demonstrated in our experiments.

% a careless observation and prediction as Section~\ref{subsec:e2e} and~\ref{subsec:system_sens} presented. %\xianzhi{Besides, the energy reduction of DVFS in parallel compression is doubtful as low frequency is \emph{not inevitably}  leading  to low  energy  consumption as examined in Section~\ref{subsec:system_sens}}.
%By comparison study in section~\ref{sec:evaluation}, we have discovered the failure of such coarse grained ways.
%Specifically, they can not always consider comprehensively of user-space applications (e.g., the core communication of them). Moreover, the isolation by OS and system-level statistics 
%fail to deliver greater energy savings due to the relatively inaccurate prediction.

\textbf{Efficient Utilization of AMPs}. 
% According to the survey by SPARSH MITTAL~\cite{amp_survey_2016}, energy efficiency~\cite{amp_eng0, amp_eng1} and performance~\cite{amp_per0, amp_per1} are two major objects most relevant to ours.
%Besides, we are also inspired by the prior works in optimizing fairness~\cite{amp_scheduling_2018, amp_scheduling_2018_p2, amp_fairness_2020} to forbid the core overload.
The approaches to effectively manage the AMP include modeling~\cite{amp_modeling} and predicting~\cite{amp_caloree} of performance/energy, CPI stack~\cite{amp_pie_2011} considering both ILP and MLP and DVFS-collibrated scheduling~\cite{amp_DVFS3, amp_fairness_2020, amp_latency_2017}. The performance/energy model has been merged into the popular mainline Linux from version 5.0 onwards as the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime}.
Yu et al.~\cite{amp_scheduling_2021} recently proposed a collaborative OS scheduler addressing comprehensive multiple optimization objects on AMP. 
However, these models treat the software running on AMP as a black box due to the isolation by OS and system-level statistics, which overlooks many optimization opportunities as demonstrated in our experiments.
% But its OS level prevents the further discovery of operational intensity per task. On the contrary, we capture the complex behavior of \compress characteristics by fine-grained decomposition and modeling. 
% in Sections~\ref{sec:decompos} and~\ref{sec:costmodel}.
%
%In addition to the OS-level works above, there are a few existing researches working in user-space for the optimization in energy or latency, 
There are also a few existing user-space research projects working on energy or latency optimization on AMPs, including virtual machine~\cite{amp_vm_yinyang}, web browser~\cite{amp_webbrowser}, game governor~\cite{amp_game} and Artificial Intelligence framework~\cite{amp_ai}. Due to the different optimization objective, these works are not applicable in our context.
% Since none of them is for parallel data compression, we have problem formulation and approaches totally different from them.



\begin{comment}
And unfortunately, existing work can not cope with them well. On the one hand, state-of-art PLSC is not AMP-aware, as they are either for symmetric multicore processor (SMP)~\cite{comp_ndzip, comp_para_bzip2} or totally hybrid structure platforms (THSP) like CPU+GPU~\cite{comp_cuda_compare} or CPU+FPGA~\cite{comp_lz4_fpga}. 
The SMP-based works assume all cores are equal and the same, lacking even the basic awareness of the asymmetries. The THSP-based ones have no ISA-sharing and have more complex control of data and program, which are also unsuitable for AMP.
On the other hand, existing AMP-related studies do not consider compression. They are either in OS level~\cite{amp_DVFS2, amp_scheduling_2018, amp_scheduling_2021} (i.e., viewing the all work load as equal black-box), or for other user-space applications (e.g., game governor~\cite{amp_game}, web browser~\cite{amp_webbrowser} and Artificial Intelligence framework~\cite{amp_ai}, etc.). So they will fail to analyse the PLSC stages and replicas and schedule them to the right place. 


\textbf{Algorithms of the Lossless Compression.}  Comparison studies between different lossless compression algorithms, in terms of compression ratio, speed, etc., have done by existing researches.
Moffat et al.~\cite{comp_survey_huffman} surveyed the methods belong to huffman encoding family over near 70 years, Al-Hafeedh et al.~\cite{comp_survey_lz} studied the LZ-family algorithms by both experimental and theoretical study, and Gupta et al.~\cite{comp_survey_2017} studied both of them. Besides, the energy effects of compression have also been discussed carefully by Barr et al. ~\cite{comp_energy_2006}. As for light-weight algorithms, some works~\cite{db_comp0, db_comp1, db_comp2} have special
interests on them due to their efficiency in accelerating the data base. The primary concern of these works is the performance outcome of different algorithms, but the effects of parallelism and new hardware platforms (e.g., the FPGA, GPU, etc.) are not included. Besides, they have not considered some newly-developed algorithms like the lz4~\cite{comp_lz4}. 
In contrast to them, we study the algorithms 1) suitable for streaming data, 2) in a parallelism manner instead of single thread running, and 3) on specific new hardware (i.e., the AMP).



\textbf{Lossless Stream Compression and its Parallelization} 
Many lossless compression are put forward and compared thoroughly, Moffat et al.~\cite{comp_survey_huffman} surveyed the methods belong to huffman encoding family over near 70 years, Al-Hafeedh et al.~\cite{comp_survey_lz} studied the LZ-family algorithms by both experimental and theoretical study, and Gupta et al.~\cite{comp_survey_2017} studied both of them. Besides, the energy effects of compression have also been discussed carefully by Barr et al~\cite{comp_energy_2006}. However, not all of them are suitable for streaming data, as existing work~\cite{db_comp0, db_comp1, db_comp2, comp_tersecades} revealed that the \compress should be \emph{light-weight}, i.e., with relative low overhead. As these works focus on single thread running of algorithms, they can not improve the performance further.

Although significant speed-up and good scale can be achieved by works, their limitations are also obvious. First, they lack the comprehensive study and only focus on the parallelism of their own interested algorithms. Next, only~\cite{comp_mpc_2015} uses hybrid compression approaches including data and algorithm parallelism. Most importantly, none of them has ever touched the AMP. Different from them, we do comparison studies including several parallelism algorithms, in a fine-grained manner, and on AMP.

\textbf{AMP and its ultilization.} 
AMP was put forward for high energy-efficiency against the increased power consumption and heat dissipation on modern multicore systems~\cite{amp_2003} (firstly called as \emph{single-ISA heterogeneous
multi-core architectures} in 2003), and soon later proved its higher performance than SMP with the same size on chip~\cite{amp_2004}. Another important thing is that this research provides experimental evidences that different pieces of code have different device preference, which motivates our decomposition of the compression algorithm. After that, the performance asymmetry~\cite{amp_impacts_2005} of different cores on AMP was highlighted and became the major start-point of exploiting the AMP. As the survey by SPARSH MITTAL~\cite{amp_survey_2016}
summarized, many works are presented to harness the AMP, taking advantage of the asymmetry (in terms of energy-efficiency and performance as mentioned before) or overcoming problems caused by it (i.e., the fairness~\cite{amp_scheduling_2018, amp_scheduling_2018_p2, amp_fairness_2020} or prdictability~\cite{amp_impacts_2005} problem). Effective approaches include modeling~\cite{amp_modeling} and predicting~\cite{amp_caloree} of performance/energy, CPI stack~\cite{amp_pie_2011} considering both ILP and MLP 
simulation, and DVFS-collibrated scheduling~\cite{amp_DVFS3, amp_fairness_2020}. Some classical ways like  PID Control~\cite{amp_latency_2015} can also help in the feed-back regulation of tasks and core frequencies. By sythetically combination of those methods, Teng Yu et al.~\cite{amp_scheduling_2021} recently proposed a collaborative OS scheduler addressing
core sensitivity, thread criticality, fairness and energy
efficiency on AMP, and they demonstrate the importance of grabbing ILP and MLP once more. These works inspire us to rethink the task-core affinity in \compress, however, since they are all OS-level, they are coarse-grained in a \emph{per-task} consideration, blind to the user-space and application specific attributes (e.g., the compression algorithm and workload in our case), and spending a lot of time in prediction though not always returning accurate results. Instead, we optimize the AMP for specific user-space usage (i.e., the parallel lossless stream compression), with fine-grained (i.e., per-stage)
discovery of ILP and MLP, and make good use of the already-known information of algorithm and workload.
Although there are a few existing researches working in user-space, including virtual machine~\cite{amp_vm_yinyang}, web browser~\cite{amp_webbrowser}, game governor~\cite{amp_game} and Artificial Intelligence framework~\cite{amp_ai}, none of them is for parallel lossless stream compression. Therefore, we have problem formulation and approaches totally different from them.
\end{comment}
\begin{comment}
\emph{Summary}.The parallel-compression-aware works are not AMP-aware, while those AMP-aware are not parallel-compression-aware. Nevertheless, this work firstly maintains parallel-compression-awareness and  AMP-awareness at the same time.
\end{comment}

==> Sections/backup/8_Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
% Despite its complexity in asymmetric cores and communication, parallel data compression on AMPs is beneficial for edge computing. 
This paper introduced {\design}, a novel framework to parallelize data compression on AMPs. 
\design's superiority is gained by both fine-grained compression parallelization and model-guided asymmetry-aware scheduling strategy. Extensive experiments on a recent AMP confirm that \design significantly outperforms the state-of-the-art.
In particular, \design is able to achieve the lowest energy consumption under a given latency constraint under a wide range of workload characteristics and system configurations. 

% that achieves awareness of both types of asymmetries. 
% With fine-grained compression parallelization and model-guided asymmetry-aware scheduling, \design is able to achieve the lowest energy consumption under a given latency constraint. 
% The experiments show that \design significantly outperforms alternative solutions: \shuhao{by an order of magnitude?????}
% First, \design can save up to 53\% of the energy. 
% Second, \design ensures that the latency and energy of parallel compression are accurately modeled. 
% Third, \design can achieve an adaptive trade-off between energy savings and latency cut-off. 
% Fourth, \design can demonstrate its superiority across a range of workload characteristics and system configurations.


%Parallel data compression is beneficial for edge computing, despite its complexity in asymmetric cores and communication. This paper have introduced {\design}, a new parallelization framework of data compression on AMPs, which achieves the awareness of both two kinds of asymmetries above. Specifically, by fine-grained decomposition of compression as well as asymmetry-aware scheduling, \design  successfully reach the least energy consumption under given latency restriction. The experiments confirm that \design significantly outperforms alternative solutions up to an order of magnitude: First, \design can achieve up to 53\% energy reduction compared to alternative solutions. Second, \design have an accurate modeling of the latency and energy of parallel compression. Third, \design can achieve adaptive trade-off between energy saving and cutting-off energy. Fourth, \design can prove its superiority under varying workload characteristics and system configurations.


%We have introduced {\design}, a new parallelization framework of data compression on AMPs.
%\design successfully reach the least energy consumption under given latency restriction.
%The experiments confirm that \design significantly outperforms alternative solutions up to an order of magnitude. 

%This work have uncovered and utilized varying task-core affinity of compression on AMP in a fine-grained manner, as well as modelized  the asymmetric core communication under task pipelining. Based on these, we can expand the parallelization and optimization for other  operations like the stream online join~\cite{sp_intra_exp} on AMP. 



%Future AMP will have more cores and larger differences between different types of cores, according to  recent AMP releases by some top vendors (e.g., the snapdragon 8 Gen 1(2021)~\cite{amp_sd8g1} by Qualcomm and the 12th generation \emph{Core} Processor~\cite{amp_i9_12} by Intel, etc). These tendencies give more chances to the synthetic utilization of various kinds of cores, and makes it more profitable. Therefore, we will conduct further experiments on the up-coming AMPs as \design is indicated to be more valuable on them.



==> Sections/backup/Backup_Parallelization.tex <==
\subsection{Parallelization Strategies}
\label{subsec:algos}
To reduce the latency overhead of compression, many recent works~\cite{comp_paralz_2013,comp_para_hsi,comp_fp_2010,comp_gpu_lossy,comp_lz4_fpga} target compressing datasets in parallel. In the following, we discuss different strategies we may apply when parallelizing stream compression algorithms on a multicore edge device.
Specifically, there are two important questions to be be answered for parallelizing the stream compression: 1) how to execute the compression on infinite and incremental stream? 2) how to schedule workload into multiple cores in each execution of stream compression.
% and the common wisdom of parallelization is also presented in other stream processing operations like stream window join~\cite{sp_intra_exp}.
% We discuss the pros and cons of different parallelization strategies in this part, including the graindularity of partition/communication, and the agglomeration policy.

 \begin{figure}[t]
    \centering
    \includegraphics*[width=\columnwidth]{figures/overView_sc.pdf}
    \caption{Overview of stream compression.}
    %\shuhao{(Mark ``big'' and ``little'' cores in figure)}}  
    \label{fig:sc_comp_overview}   
\end{figure}

\subsubsection{Execution Strategies}
% In this part, we introduce two execution strategies to achieve the compressing-on-arriving requirements of stream compression, and further discuss how to handle the concurrent state update in stateful stream compression.
%Unlike the file compression or database compression where all data to be compressed are available before compression, stream compression should compress tuples during ~\emph{their arrivals}. In this part, we firstly introduce two execution strategies which can achieve the compressing-on-arriving, and
There is a common wisdom in the stream processing community of \emph{micro-batching}~\cite{sp_spark}, which can be applied to conduct the \emph{lazy stream compression} compared with the eager approach aforementioned. In this way, compression will only be conducted after enough agglomeration of tuples, which can reduce the overhead of partitioning and synchronization. As the micro-batching procedures take place in the layered cache and memory with different speed grades and capacities, a nature question arises as ``how many tuples should be batched in stream compression''. On the one hand, batching a too small number of tuples leads to frequent flush and reload. On the other hand, a larger number means we have to store tuples in slower memory storage. Therefore, it's necessary to determine a suitable size.

\textbf{Eager Execution.}
To fit into the infinite and incremental nature of stream, we can compress each tuple as soon as it arrives. In this way, only one tuple will be batched, and it can be considered as \emph{eager stream compression} in analogy with the \emph{eager stream join}~\cite{sp_intra_exp}.

\textbf{Lazy Execution.}
Such a continuous data flow-based processing model with no agglomeration seems a natural fit for handling infinite streaming inputs, but results in sub-optimal hardware utilization as there are frequency partitioning and synchronization which may\emph{ block} the ``real'' running of compression. 

\subsubsection{Shared State Implementation.}
Concurrent writing may occur in the state update (i.e., $s2$ in Algorithm~\ref{alg:stateful}) if compressing in parallel~\cite{comp_para_lzss}. Specifically, two or more cores may try to update the same part of the global state with different values,
and how to deal with the state during parallelization increases the design space of stateful stream compression.
%In this case, we can either share the state by using concurrency control like locks to avoid the conflicts, or just allow them to maintain their own state and disable the sharing. The sharing-or-not towards state increases the design space of stateful stream compression. Specifically, a global and shared state can theoretically achieve higher compressibility than separate states, as it can maintain more comprehensive recording of past tuples. However, parallelism my lost due the extra overhead of concurrency control.

\textbf{Shared state.}
We can let all cores share the single and global state, and use concurrency control like locks to avoid the conflicts. With the global sharing state, we can theoretically achieve higher compressibility than separate states, as it can maintain more comprehensive recording of past tuples. However, parallelism my lost due the extra overhead of concurrency control.

\textbf{Non-Shared state.}
We can also let each core maintain its own state and disable the sharing. This strategy can maximize the parallelisim as there is no concurrent conflict at all. However, splitting the state will loss compressibity as a core is totally unaware of the past tuples which are handled by the state of other cores. 
\subsubsection{Scheduling Strategies}
\label{subsubsec:scheduling}
We let each core in multicore edge device be scheduled a partition of stream workload for the parallel compression, the partition is assigned as a \emph{distribution ratio}. Specifically, we let $distribution\ ratio = \frac{\text{assigned workload size}}{\text{total workload size}}$.
%just some mention for the SMP
The solution is as simple as ``balanced partition and equal distribution ratio''~\cite{comp_para_bzip2} for symmetric multicore processor (SMP) case,  as all cores have equal computational power and have equal communication distance to each other.
%somehow copied from bailan ICDE.
However, when either the computational power or communication distance is not the same for all cores, the scheduling becomes \emph{a complicated art of arranging distribution ratios}, and a simple average scheduling will leads to both more latency and more energy dissipation.
%say AMP is popular, briefly

Non-equal computational power and communication distance is common at the edge according to a 2018 survey~\cite{edge_survey}, as asymmetric multicore processors (AMPs) are of increasing popularity to be applied for balancing computational power and energy consumption~\cite{amp_survey_2016}. For instance, a recent 6-core AMP RK3399~\cite{amp_rk3399} depicted in Figure~\ref{fig:rk3399} and specified in Table~\ref{tab:asymmetry} has the asymmetric properties 
as follows.

\begin{itemize}
    \item \textbf{Asymmetric computation.} Despite the sharing of ARM V8 ISA~\cite{amp_armv8}, the RK3399 involves different types of cores on the same processor: the relatively batter-saving and slower A53 cores (also called ``little core'', namely $Core0 \sim Core3$)~\cite{amp_A53ug}, and the power-hungry A72 cores (also called ``big core'', namely $Core4 \sim Core5$). They are placed at different \emph{clusters}~\cite{amp_survey_2016}, each cluster has cores under identical micro-architecture and sharing the equivalent clock frequency setting (i.e., $Cluster \ 0$ for A53 cores and $Cluster \ 1$ for A72 cores).
    \item \textbf{Asymmetric communication.} The cluster structure lead to two kinds of core communication in AMPs~\cite{amp_cluster_2021, amp_partition_2019}, i.e., \emph{intra-cluster} and \emph{inter-cluster} communication. The \emph{intra-cluster} communication (denoted as \emph{c0} in Figure~\ref{fig:rk3399}) is the direct sharing of L2 cache for cores within the same cluster, while \emph{inter-cluster} communication (denoted as \emph{c1} and \emph{c2}, respectively) represents that communication between cores went through a much slower interconnection link (i.e., CCI500). Due to the different hardware connection approach, $c0$, $c1$, $c2$ has different overhead as we summaried in Table~\ref{tab:asymmetry}.
    \iffalse
    uch a hardware architecture is conceptually similar to NUMA~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
% This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
Different from NUMA, \emph{inter-cluster} communication on AMPs further involves additional \emph{polarity} effects. 
\xianzhi{Specifically, transferring data from little cores to big cores is more costly than the reverse process.
This is because big cores are typically faster than little cores and should wait for the little cores, which increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.}
\fi
\end{itemize}

Such asymmetry especially requires a careful scheduling for better exploitation. Specifically, each step in Algorithm~\ref{alg:stateless} and ~\ref{alg:stateful} prefers the big cores or little cores to different degree in reducing latency or energy consumption.
%
This is because different stream compression steps function differently (as we illustrated in Section~\ref{subsec:intro_state}) and thus have different ~\emph{operational intensity} (i.e., instructions per memory access). According to existing works~\cite{amp_impacts_2005, amp_modeling, amp_scheduling_2021, amp_pie_2011}, software with larger operational intensity is more worthy to run on big cores, or vice verses.
In our case, a stream compression step that is more about compression-related computation such as $s1$ in Algorithm ~\ref{alg:stateful} and $s3$ in Algorithm~\ref{alg:stateful} requires a higher distribution ratio on big cores, and one that is more about memory addressing (i.e., loading tuples or outputting the compressed stream, such as $s0$) requires a lower distribution.
%
Meanwhile, we should also pay attention to the asymmetric communication effects in optimizing the latency. Specifically, when the distribution ratio of two consecutive steps is different, one core needs to fetch data from another instead of loading it from local-coupled storage (i.e., the private registers and L1D-cache). 
%Such ``remote data fetching'' would be costly if not well-scheduled.
 
\iffalse
\shuhao{Change the tone make them the default parallelism.}
Depending on how to distribute the streaming workload into parallel execution units (e.g., the processor cores), the partition and communication in parallelizing stream compression can be either coarse-grained or fine fine-grained, as illustrated in Figure~\ref{fig:parallel_grand}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/partition_communication.pdf}
    \caption{The different gurandularities of partition and communication}
    \label{fig:parallel_grand}
\end{figure}
Each step can have its own work distribution ratio on execution units. Theoretically, the PL approach can provide better exploitation of different compression behaviors in different steps, which is especially helpful to utilize asymmetric hardware resource (e.g., when using both CPU and GPU in CULZSS~\cite{comp_lzss_cuda}). For instance, to improve the energy efficiency, the memory-bounded $s0$ in Algorithm~\ref{alg:stateless} should be distributed less to the higher performance hardware compared with $s1$. However, more complicated communication is introduced to PL than DD, as one execution unit may fetch data from another due to the ratio divergence in different steps~\cite{sp_coprocessing}.
It is worth noting that concurrent writing may occur in the state update (i.e., $s2$ in Algorithm~\ref{alg:stateful}) if parallelized~\cite{comp_para_lzss}. Specifically, two or more parallel execution units (i.e., CPU/GPU cores, FPGA logic arrays, etc) may try to update the same part of the global state with different values. In this case, we can either use concurrency control like locks to avoid the conflicts, or just allow them to maintain their own state and disable the sharing. The sharing-or-not towards state increases the design space of stateful stream compression.

\textbf{Asymmetric computation.}
AMPs maintain a cluster-like structures to organize cores~\cite{amp_survey_2016}.  
Cores within the same cluster follow identical micro-architecture and share the equivalent clock frequency setting.
Despite the sharing of ARM V8 ISA~\cite{amp_armv8}, the rk3399 involves different types of cores on the same processor: the relatively batter-saving and slower A53 cores (also called ``little core'')~\cite{amp_A53ug} at cluster 0 and more powerful and power-hungry A72 cores (also called ``big core'')~\cite{amp_A72ug} at cluster 1. 

\textbf{Asymmetric communication.}
There are two kinds of core communication in AMPs~\cite{amp_cluster_2021, amp_partition_2019}, i.e., \emph{intra-cluster} and \emph{inter-cluster} communication. The \emph{intra-cluster} communication (denoted as \emph{c0} in Figure~\ref{fig:rk3399}) is the direct sharing of L2 cache for cores within the same cluster, while \emph{inter-cluster} communication (denoted as \emph{c1} and \emph{c2}, respectively) represents that communication between cores went through a much slower interconnection link (i.e., CCI500). 
Such a hardware architecture is conceptually similar to NUMA~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
% This is similar to the well-known NUMA effect~\cite{sp_briskstream} and requires one to carefully align the communication patterns among tasks being scheduled to get good performance.
Different from NUMA, \emph{inter-cluster} communication on AMPs further involves additional \emph{polarity} effects. 
\xianzhi{Specifically, transferring data from little cores to big cores is more costly than the reverse process.
This is because big cores are typically faster than little cores and should wait for the little cores, which increases the \emph{synchronization} and \emph{hand-shaking} cycles in hardware, e.g., the AMBA/AXI protocol in ARM~\cite{amp_axi}.}



We may apply data partition for the entire compression procedure. In this way, each thread is distributed with a partition of workload as assigned by a \emph{distribution ratio}. Specifically, we let $distribution\ ratio = \frac{\text{assigned workload size}}{\text{total workload size}}$ for each kind of execution unit(s).
Such a ratio is shared by all compression steps (e.g, $s0$ $\sim$ $s2$ for stateless compression in Algorithm~\ref{alg:stateless}). The shared ratio simplifies the parallelization design, and achieves low communication overhead as each execution unit only needs to fetch data from its own \emph{local-coupled} memory (e.g. the L1D cache). Due to the relatively simple implementation and low communication overhead, the DD manner is especially common in parallelizing compression on symmetric hardware such as ~\cite{comp_para_bzip2,comp_paralz_2013}.
\fi
\begin{figure}[t]
    \centering
    \includegraphics*[width=0.32\textwidth]{figures/AMP.pdf}
    \caption{The 6-core AMP rk3399.}
    %\shuhao{(Mark ``big'' and ``little'' cores in figure)}}  
    \label{fig:rk3399}   
\end{figure}

\begin{table}[t]
\centering
\caption{Hardware Specifications of RK3399. The unit of latency is ``ns per 32-bit access''.}
\vspace{+3pt}
\label{tab:asymmetry}
\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{|L{2cm}|L{1cm}|L{2cm}|L{1cm}|L{0cm}}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Asymmetric\\  cores\end{tabular}}        & \textbf{Type} & \textbf{L1 cache size}   & \textbf{Pipeline} \\ \cline{2-4} 
 & A72 & 48K I+ 32 K D                 & out-of-order     \\ \cline{2-4} 
 & A53 & 32K I+ 32K D                  & in-order \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Asymetric\\  communication\end{tabular}} & \textbf{Path} & \textbf{Description} & \textbf{Latency}  \\ \cline{2-4} 
 & c0  & intra-cluser                  & 4.4          \\ \cline{2-4} 
 & c1  & inter-cluster, cluster 1 to 0 & 8.9          \\ \cline{2-4} 
 & c2  & inter-cluster, cluster 0 to 1 & 26.3         \\ \hline
\end{tabular}%
}
\end{table}

% , and then review the existing approaches in exploiting such asymme

%We explore such dilemma through experiments in section~\ref{}.

==> Sections/backup/Related_work_0519.tex <==
\section{Related Work}
\label{sec:related}
% In this section, we review the related work and reveal the limitations that motivate this work.
% \subsection{AMP-aware Task Scheduling}



Researcher have also utilized specific architectures for parallelzing compressing.
On the FPGA, Milward et al.~\cite{comp_2004_tpds} implemented a novel dictionary-based parallel compression implementation, Sano et al.~\cite{comp_fp_2010} achieved float-point data compression, Tian et al.~\cite{comp_waveSz} proposed parallel compression for scientifical data, and Bark et al.~\cite{comp_lz4_fpga} parallelized the lz4 algorithm.
On the GPU, the parallelization of several LZ algorithms~\cite{comp_lzFamily} have been conducted~\cite{comp_lzss_cuda,comp_mpc_2015}, and Huang et al.~\cite{comp_gpu_lossy} have also parallelized trajectory-specific compression algorithms. Due to the significant difference in hardware architectures, it is unclear how can those works be applied for parallel stream compression on AMPs.



AMP thread scheduling There are thread scheduling algorithms
designed for AMP machines [3, 31, 62]. They schedule threads
to big or little cores by monitoring their hardware behaviours or
criticality. WASH [31] proportionally schedules threads to big and
little cores according to the core capability. COLAB [62] makes
coordinated core assignment and thread selection decisions based
on the performance estimation of each thread on different cores, as
well as identified communication patterns and bottleneck threads.
Gomatheeshwari et al. [4] utilize a lightweight-deep neural network
(LW-DNN) to predict the optimal cores for each workload. 
Compared with AsyMo, these works are for general thread scheduling
at the OS or language virtual machine level. They are unknown of
the code logic running on each thread, such as the matrix multiplication in this paper. Therefore, these schedulers cannot conduct
block partition for matrix multiplication and then schedules them.
By comparison, AsyMo partitions blocks first and then schedules
the sub-block tasks according to the core capability

The approaches to effectively manage the AMP include modeling~\cite{amp_modeling} and predicting~\cite{amp_caloree} of performance/energy, CPI stack~\cite{amp_pie_2011} considering both ILP and MLP and DVFS-collibrated scheduling~\cite{amp_DVFS3, amp_fairness_2020, amp_latency_2017}. 
The performance/energy model has been merged into the popular mainline Linux kernel from version 5.0 on-wards as the \emph{Energy Aware Scheduling (EAS)}~\cite{amp_realtime}.
Yu et al.~\cite{amp_scheduling_2021} recently proposed a collaborative OS scheduler addressing comprehensive multiple optimization objects on AMP. 
However, these models treat the software running on AMP as a black box due to the isolation by OS and system-level statistics, which overlooks many application-specific optimization opportunities. 
There are also a few existing user-space research projects working on energy or latency optimization on AMPs, including virtual machine~\cite{amp_vm_yinyang}, web browser~\cite{amp_webbrowser}, game governor~\cite{amp_game} and Artificial Intelligence framework~\cite{amp_ai}.
As the their application behaviors and problem formulations are different from compression, these works are not applicable in our context.


The asymmetric properties of AMPs increases the difficulty of meeting the latency constraints when parallelizing stream compression. 
% If we are unable to estimate the asymmetric communication for fine-grained scheduling, especially the long latency of $c2$, there can be more violation of latency constraints.
Unfortunately, existing works~\cite{amp_partition_2019, amp_cluster_2021} only consider inter-cluster communication for task switching in operating system level, but not for specific tasks. In particular, there is lack of a model to estimate such asymmetric communication effects for parallelizing compression on AMPs.

\begin{comment}
And unfortunately, existing work can not cope with them well. On the one hand, state-of-art PLSC is not AMP-aware, as they are either for symmetric multicore processor (SMP)~\cite{comp_ndzip, comp_para_bzip2} or totally hybrid structure platforms (THSP) like CPU+GPU~\cite{comp_cuda_compare} or CPU+FPGA~\cite{comp_lz4_fpga}. 
The SMP-based works assume all cores are equal and the same, lacking even the basic awareness of the asymmetries. The THSP-based ones have no ISA-sharing and have more complex control of data and program, which are also unsuitable for AMP.
On the other hand, existing AMP-related studies do not consider compression. They are either in OS level~\cite{amp_DVFS2, amp_scheduling_2018, amp_scheduling_2021} (i.e., viewing the all work load as equal black-box), or for other user-space applications (e.g., game governor~\cite{amp_game}, web browser~\cite{amp_webbrowser} and Artificial Intelligence framework~\cite{amp_ai}, etc.). So they will fail to analyse the PLSC stages and replicas and schedule them to the right place. 


\textbf{Algorithms of the Lossless Compression.}  Comparison studies between different lossless compression algorithms, in terms of compression ratio, speed, etc., have done by existing researches.
Moffat et al.~\cite{comp_survey_huffman} surveyed the methods belong to huffman encoding family over near 70 years, Al-Hafeedh et al.~\cite{comp_survey_lz} studied the LZ-family algorithms by both experimental and theoretical study, and Gupta et al.~\cite{comp_survey_2017} studied both of them. Besides, the energy effects of compression have also been discussed carefully by Barr et al. ~\cite{comp_energy_2006}. As for light-weight algorithms, some works~\cite{db_comp0, db_comp1, db_comp2} have special
interests on them due to their efficiency in accelerating the data base. The primary concern of these works is the performance outcome of different algorithms, but the effects of parallelism and new hardware platforms (e.g., the FPGA, GPU, etc.) are not included. Besides, they have not considered some newly-developed algorithms like the lz4~\cite{comp_lz4}. 
In contrast to them, we study the algorithms 1) suitable for streaming data, 2) in a parallelism manner instead of single thread running, and 3) on specific new hardware (i.e., the AMP).



\textbf{Lossless Stream Compression and its Parallelization} 
Many lossless compression are put forward and compared thoroughly, Moffat et al.~\cite{comp_survey_huffman} surveyed the methods belong to huffman encoding family over near 70 years, Al-Hafeedh et al.~\cite{comp_survey_lz} studied the LZ-family algorithms by both experimental and theoretical study, and Gupta et al.~\cite{comp_survey_2017} studied both of them. Besides, the energy effects of compression have also been discussed carefully by Barr et al~\cite{comp_energy_2006}. However, not all of them are suitable for streaming data, as existing work~\cite{db_comp0, db_comp1, db_comp2, comp_tersecades} revealed that the \compress should be \emph{light-weight}, i.e., with relative low overhead. As these works focus on single thread running of algorithms, they can not improve the performance further.

Although significant speed-up and good scale can be achieved by works, their limitations are also obvious. First, they lack the comprehensive study and only focus on the parallelism of their own interested algorithms. Next, only~\cite{comp_mpc_2015} uses hybrid compression approaches including data and algorithm parallelism. Most importantly, none of them has ever touched the AMP. Different from them, we do comparison studies including several parallelism algorithms, in a fine-grained manner, and on AMP.

\textbf{AMP and its ultilization.} 
AMP was put forward for high energy-efficiency against the increased power consumption and heat dissipation on modern multicore systems~\cite{amp_2003} (firstly called as \emph{single-ISA heterogeneous
multi-core architectures} in 2003), and soon later proved its higher performance than SMP with the same size on chip~\cite{amp_2004}. Another important thing is that this research provides experimental evidences that different pieces of code have different device preference, which motivates our decomposition of the compression algorithm. After that, the performance asymmetry~\cite{amp_impacts_2005} of different cores on AMP was highlighted and became the major start-point of exploiting the AMP. As the survey by SPARSH MITTAL~\cite{amp_survey_2016}
summarized, many works are presented to harness the AMP, taking advantage of the asymmetry (in terms of energy-efficiency and performance as mentioned before) or overcoming problems caused by it (i.e., the fairness~\cite{amp_scheduling_2018, amp_scheduling_2018_p2, amp_fairness_2020} or prdictability~\cite{amp_impacts_2005} problem). Effective approaches include modeling~\cite{amp_modeling} and predicting~\cite{amp_caloree} of performance/energy, CPI stack~\cite{amp_pie_2011} considering both ILP and MLP 
simulation, and DVFS-collibrated scheduling~\cite{amp_DVFS3, amp_fairness_2020}. Some classical ways like  PID Control~\cite{amp_latency_2015} can also help in the feed-back regulation of tasks and core frequencies. By sythetically combination of those methods, Teng Yu et al.~\cite{amp_scheduling_2021} recently proposed a collaborative OS scheduler addressing
core sensitivity, thread criticality, fairness and energy
efficiency on AMP, and they demonstrate the importance of grabbing ILP and MLP once more. These works inspire us to rethink the task-core affinity in \compress, however, since they are all OS-level, they are coarse-grained in a \emph{per-task} consideration, blind to the user-space and application specific attributes (e.g., the compression algorithm and workload in our case), and spending a lot of time in prediction though not always returning accurate results. Instead, we optimize the AMP for specific user-space usage (i.e., the parallel lossless stream compression), with fine-grained (i.e., per-stage)
discovery of ILP and MLP, and make good use of the already-known information of algorithm and workload.
Although there are a few existing researches working in user-space, including virtual machine~\cite{amp_vm_yinyang}, web browser~\cite{amp_webbrowser}, game governor~\cite{amp_game} and Artificial Intelligence framework~\cite{amp_ai}, none of them is for parallel lossless stream compression. Therefore, we have problem formulation and approaches totally different from them.
\end{comment}
\begin{comment}
\emph{Summary}.The parallel-compression-aware works are not AMP-aware, while those AMP-aware are not parallel-compression-aware. Nevertheless, this work firstly maintains parallel-compression-awareness and  AMP-awareness at the same time.
\end{comment}

==> Sections/backup/broken_Pre.tex <==
\section{Preliminaries}
\label{sec::preliminaries}
The special asymmetry of AMP (i.e., identical ISA together with different micro-architecture and unbalanced cache/memory structure) is usually charming
but sometimes troublesome (e.g., to ensure the thread fairness~\cite{amp_fairness_2020}). Therefore, this section introduces some technologies and experiments to further understand the asymmetry, drill the root of the charms and troubles, and act as the base of our model and optimization.
\subsection{The roof lines}
The roof line model was first put forward by Williams, etc. in this century~\cite{roofline_1st}, and soon becomes a common tool of studying the computing power of specific platforms (e.g., CPU, GPU, FPGA) due to its high-level abstraction and concise synthesis. 
Typically, an intuitive graph of roof line model sets the relative bounding of programs (i.e., memory or CPU) as the horizontal axis and the performance of platform (i.e., the number of instruction executed within a time period) as the vertical axis, so the shape of graph line is just the same as the \emph{roof}.

In addition to such model studies performance, there is an another roof line model which changes the vertical axis to the number of instruction executed within specific energy~\cite{roofline_energy}. It gives another insight of the hardware in terms of energy-efficiency, and its shape is similar to the former one.

Although the main usage of these two kinds of roof line is to evaluate the upper-bound of the device in performance or energy, they can also be used for the prediction of algorithms running on the platform. Nugteren and Corporaal have shown how to do this as the boat-hull model~\cite{roofline_boat}, which also gives us inspiration to do so. 
\subsection{Experimental roof lines on AMP}
Lopes etc.~\cite{roofline_synth} have shown that when considering the hardware resource like cache more carefully, the shape of roof line will distort but more close to the real situation of the execution of algorithms. Therefore, we review the roof lines on AMP through experiments instead of theoretical analysis, and the effects of cache, on-chip bus, etc. can be directly included.

We developed a test bench for this by keeping the memory access the same and changing the times of an accumulation\endnote{Since the hardware is under RISC architecture, accumulation is just representative enough for any other integer operations used in compression jobs. } program. Then the test bench can have a record of the execution latency (by OS API), the instructions have run (by the \emph{perf}~\cite{amp_perf} events), and the energy consumption (by reading the energy meter through USB2.0 interface), which can be used for the performance and energy roof lines with previously controlled memory access. To be inclusive, we examined both the \emph{big core} and the \emph{little core}, under all of their available frequencies. All results below are tested on the rk3399 AMP processor~\cite{amp_rk3399}, whose logical structure is shown as 
Figure \ref{fig:rk3399}. We mark the A72-based~\cite{amp_A72ug} \emph{big core} as 'B' and the A53-based~\cite{amp_A53ug} \emph{little core} as 'A' in following graphs, and the unit of frequency is GHz(for instance, the legend 'B-1.8' represents  \emph{big core} under 1.8GHz).
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/rk3399.png}
    \caption{The 6-core AMP rk3399. This is tooooo ugly.}  \label{fig:rk3399}   
\end{figure}

\subsubsection{The performance roof line}
\label{subsub:proof}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/proof.png}
    \caption{The performance roof line on AMP rk3399}  \label{fig:proof}   
\end{figure}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/speedup.png}
    \caption{The speed up of big and little on AMP rk3399}  \label{fig:pspeed}   
\end{figure}
In Figure \ref{fig:proof}, We draw the performance roof line with the horizontal axis of instructions per memory access (IPM)\endnote{The test bench use 32-bit aligned memory access, and other width like 8 or 16 bits can have a relative stable conversion relationship with it.}, the vertical axis of mega integer operations per second (MINTOPS), and both of them are in log10 scaling. To get the speed-up of \emph{big core} against \emph{little core}, we also divide their MINTOPS directly from Figure \ref{fig:proof} under the same frequency and under two different pairs of frequency\endnote{since the \emph{big core} has two more frequencies than the \emph{little core}}, which is shown as Figure \ref{fig:pspeed}, with normal scaling in vertical axis.
By these two figures, the asymmetry in performance can be learnt further in following aspects.

\textbf{The slow growth or even drop in the middle}. For all available frequencies, the performance roof line of \emph{big core} is a 3-segmentation-curve with IPM increasing: fast growth, slow growth, and saturated stage. While the fast growth and saturated stage is similar to the original and theoretical model in ~\cite{roofline_1st}, the slow growth is caused when increasing IPM leads to more often miss in L1I (i.e., too high density of instruction). When it comes to \emph{little core}, the slow growth phase is even more worse and complicated with a sudden \emph{drop}. This is because 1) the L1I of \emph{little core} A53 is smaller and 2) the in-order A53 performs worse than the out-of-order(OoO) A72 when encounter massive instructions as an instruction can \textbf{only} be executed after its prior one.

\textbf{The changing speed-up with IPM}. From a more explicit view from Figure \ref{fig:pspeed}, we find the relative gain in performance of the \emph{big core} against the \emph{little core} is \textbf{not constant}, but follows an intricacy relationship with the IPM. At the first beginning when IPM is low, the speed-up is even below 1 as the profits of OoO is not significant against the too small instruction density. Then, the compound game between pipeline structure, cache structure and instruction density caused the speed-up soar and sink (i.e., when IPM is about 300, perhaps due to the limit by L2 and CCI500). Finally, the speed-up can reach the saturated stage as both the \emph{big core} and the \emph{little core} are saturated to the high density of instructions. However, prior work on AMP always fail to grasp such changing speed-up as the OS is blind to the IPM and can only assume a fixed ratio(e.g., the different \emph{price} of cores~\cite{amp_DVFS3} or the \emph{power-coefficiency} defined in device tree~\cite{amp_linux}), which is still valid for the saturated stage but misleading otherwise.
\subsubsection{The energy roof line}
\begin{figure}
    \centering
    \includegraphics*[width=0.4\textwidth]{figures/eroof.png}
    \caption{The energy roof line on AMP rk3399}  \label{fig:eroof}   
\end{figure}
Similar to Figure \ref{fig:proof} in \ref{subsub:proof}, we draw the energy roof line in Figure \ref{fig:eroof}. And the only difference is that the vertical axis is about mega integer operations per Joule instead of MINTOPS. Similar and somehow less complex than the performance roof line, the energy roof line tells that the energy efficiency is also changing according to the IPM, which is the intrinsic properties of a given software (e.g., compression algorithm and the compressible parts of its input data).

To sum up of this section, the two kinds of roof lines help us to better grasping the asymmetry, and to understand how software (represented by IPM) influences the performance and energy-efficiency of the AMP hardware. 


==> Sections/backup/intro_backup.tex <==
section{Introduction}
\label{sec::introdction}
%First introduce data stream compression.
\begin{comment}
Making the best use of the critical resources like memory, network bandwidth, and processor cores is crucial in Internet of Things~\cite{IoT_survey2019}, as the limited space of resource is usually faced with ever-increasing demand. In the stream processing~\cite{sp_def,nebulastream} under IoT, which is an data intensive application, this need and dilemma is even more pressing as in-memory processing is strictly and eagerly required for performance concern~\cite{comp_tersecades}. 
For this reason, lossless compression (LC) on large volume of stream data, i.e., reduce the inner redundancy of it without breaking any information it carried on, is helpful to relive the stress~\cite{comp_tersecades}. 

Generally speaking, we can achieve that by 1) variable length coding approaching the entropy~\cite{comp_huffman}, 2) using \emph{dictionary} to represent the repeated sequence~\cite{comp_lzFamily} or 3) just cutting off unnecessary bits ~\cite{comp_elias,comp_baseDelta}. However, none of them comes free, and extra cost on power consumption and execution time will be generated then. 

However, nothing comes free, the LC will introduce extra cost on execution time and power consumption to the stream processing, which are tricky for 1) meeting the real-time quality-of-service and 2) meeting the energy constrains and reducing electricity billings. 
\end{comment}
%LSC is important, especially for embedded SP
Lossless compression (LC) on large volume of stream data, or lossless stream compression (LSC) for short, is aimed at reducing the inner redundancy of the data without breaking any information it carried on. This operation is of great help to boost stream processing(SP)~\cite{comp_tersecades} as it can provide more opportunities of in-memory-processing and save the bandwidth. For SP at embedded systems under Internet of things (IoT)~\cite{IoT_survey2019,nebulastream}, the LSC operation is even more necessary due to the starker contradiction between limited memory and infinite data.
%we have PLSC, but not for energy-efficiency at  embedded IoT systems. 
Starting in 1985~\cite{comp_1985} and thriving in this century,
many have explored the parallelization of LSC or generic LC to improve the performance~\cite{comp_para_bzip2,comp_ndzip,comp_para_gpu,comp_para_lzss,comp_lz4_fpga}. However, since low latency or high throughput are their major concerns, they have not give enough attention to energy-efficiency, especially that at embedded IoT systems. 

%AMP is for energy-efficiency 
The asymmetric multicore processors (AMPs) are intended to improve energy efficiency~\cite{amp_2003}, as well as guarantee or even improve the performance ~\cite{amp_2004}.
%AMP is widely used in embedded IoT
 Nowadays, top processor vendors like to apply the idea of AMP to build their flag-ship processors for edge and mobile computing (e.g. the rk3399(2016)~\cite{amp_rk3399} by Rockchip, the snapdragon-888(2020-2021)~\cite{amp_sd888} by Qualcomm and the kirin-9000(2020-2021)~\cite{amp_kirin9000} by Hisilicon) as AMPs have shown great success in fulfilling their original intention. 
 %why AMP is niubi AND what does it look like
Generally speaking, AMP means 1) identical instruction set architecture (ISA), 2) asymmetric cores (e.g., the In-Order A53~\cite{amp_A53ug} cores and Out-of-Order A72~\cite{amp_A72ug} cores)  with different performance and power and 3) asymmetric cache-memory structure to couple the asymmetric cores. Due to the widely application~\cite{amp_iot} and such insightful design, it's natural and explicit to use AMP for  PLSC on embedded SP cases.
%PLSC stages and replications

Like parallelizing other things (e.g., the stream processing engine~\cite{flink,storm}), PLSC includes 1) pipelined processing, i.e., to decompose the whole compression job into \emph{stages} and arrange them in a chain and 2) stage replications, i.e., each stage can have multiple \emph{replicas} running at the same time which only deals with a partition of all data. On concrete devices, each \emph{stage} of PLSC and its all \emph{replicas} should be assigned with specific computational hardware resource for the real execution, and this process is scheduling or core-mapping for multicore systems including AMP. The goal this paper is to schedule the PLSC on AMP for least energy consumption, with acceptable latency and no CPU overload.

%challenges
The appropriate scheduling to our goal is difficult due to following two major challenges:

\begin{enumerate}
    \item [C1] \textbf{There is a varying core affinity of each PLSC stage}. By intuition, we can map stages and replicas to In-Order cores mainly for less energy cost, and to Out-or-Order cores mainly for less time cost. However, this is not always right as the core affinity (in terms of power and performance) is stage-determined, and an arbitrary scheduling like so can lead to both energy waste and latency increase. Besides,  
     varying input data characteristics may further change the processing behavior of parallel compression tasks, which makes the evaluation of core affinity even harder.
    \item [C2] \textbf{The penalty of core communications (CC) between stages is also varying and asymmetric}. Taking the ARM'S big.LITTLE core (ABLC)~\cite{amp_official1} AMP which organize cores in \emph{clusters} for example, there are both \emph{inter-cluster} CC and \emph{intra-cluster} CC (i.e., for cores within the same \emph{cluster} or placed at different \emph{clusters} respectively). Due to the asymmetric cache-memory structure in hardware, especially the hardware path of resource sharing, the \emph{intra-cluster} CC is less costly than \emph{inter-cluster} CC. In addition, the \emph{inter-cluster} CC has \emph{polarity} itself, i.e., the cost of CC in '\emph{cluster} A to \emph{cluster} B' is different from that in '\emph{cluster} B to \emph{cluster} A', according to the performance difference of these \emph{clusters}. This kind of polarity makes CC in AMP even different from that in NUMA-architecture~\cite{sp_briskstream}, which has \emph{sockets} resemble to \emph{clusters} but without polarity in CC.
    
\end{enumerate}
And unfortunately, existing work can not cope with them well. On the one hand, state-of-art PLSC is not AMP-aware, as they are either for symmetric multicore processor (SMP)~\cite{comp_ndzip,comp_para_bzip2} or totally hybrid structure platforms (THSP) like CPU+GPU~\cite{comp_cuda_compare} or CPU+FPGA~\cite{comp_lz4_fpga}. The SMP-based works assume all cores are equal and the same, lacking even the basic awareness of the asymmetries. The THSP-based ones have no ISA-sharing and have more complex control of data and program, which are also unsuitable for AMP.
On the other hand, existing AMP-related studies do not consider compression. They are either in OS level~\cite{amp_DVFS2,amp_scheduling_2018,amp_scheduling_2021} (i.e., viewing the all work load as equal black-box), or for other user-space applications (e.g., game governor~\cite{amp_game}, web browser~\cite{amp_webbrowser} and Artificial Intelligence framework~\cite{amp_ai}, etc.). So they will fail to analyse the PLSC stages and replicas and schedule them to the right place. 
\begin{comment}

To improve the performance of LC, existing works have done a lot for  (QoS)~\cite{sp_QoS} of SP, and meet the power constrains especially for SP under IoT~\cite{IoT_survey2019,nebulastream}, we need to speedup the stream LC in an energy-efficient manner. 

Parallelization is a common way to reduce time cost, and
it have been used on LC since 1985~\cite{comp_1985}. In this century, the parallelization strategies show even greater success on symmetric multicore processors (SMP)~\cite{comp_para_bzip2,comp_ndzip}, GP-GPU~\cite{comp_para_gpu,comp_para_lzss,comp_para_lz77_gpu} and FPGA~\cite{comp_lz4_fpga}. Like parallelizing other things (e.g., the stream processing engine~\cite{flink,storm}), parallel LC includes 1) pipelined processing (i.e., to decompose the whole compression job into stages and arrange them in a chain) and 2) operator replications (i.e., each stage can have multiple execution units running at the same time which only deals with a partition of all data). These two aspects of parallelism together with the core (or ALU and other resource in FPGA) mapping of each units form a large solution space to arrange a parallel LC job.
\end{comment}

%
%Then introduce AMP

Witnessing this problem, we present a novel AMP-aware PLSC scheduling strategy as the first, which is named as \emph{Affinity and Cache Aware Mapping} (ACAM). Specifically, {\design} considers the core affinity according to a certain replica of specific compression stage handling specific data set (denoted as the \emph{execution unit})  by compression-specific analysis of algorithms along with synthetic adoption of the \emph{roof line model}~\cite{roofline_1st} on AMP, which is a fine-grained manner compared to black-box view of compression threads. In addition, we propose and use the \emph{slope model} in {\design} to address the variable and polar CC in AMP. If we define one of the ways to map \emph{stages} and their \emph{repliacas} of a PLSC algorithm to AMP cores as a \emph{scheduling plan}, {\design} can decide the best one as it can suitably determine the correlation between a \emph{scheduling plan} and its
objective value(e.g., , latency or energy). To reduce the cost of enumerate and analyzing each plan, we combine {\design}  with the dynamic programming~\cite{algo_dp_1954}.
\begin{comment}
While the models in {\design} provide a more accurate estimation of the PLSC behavior on the AMP platform, the resulting placement optimization problem is still challenging to solve. In particular, stochasticity is introduced into the problem as the objective value (e.g., energy) or weight (e.g., resource demand) of each \myeu is variable and depends on all previous decisions. 
Additionally, the placement decisions may conflict with each other and constraints on computation power are introduced into the problem. 
For instance, scheduling of an \myeu at one core may prohibit some other \myeu to be scheduled to the same core at the same time, as the accumulated workload of these \emph{execution units} will make the core overload. Therefore, we adopt the dynamic programming~\cite{algo_dp_1954} in {\design} to relieve the stress and quickly identify the optimal \emph{scheduling plan} under a given condition.

by three improvements compared to state-of-art:
\begin{itemize}
\item \textbf{Fine-grained Manner}. Placing at the user space, {\design} can directly recognize and touch every replications of every stages belonging to a whole compression job, instead of viewing the job as black boxes of abstract \emph{threads}. This is the premise to realize and use the different core-affinity. 
%This manner is illustrated in section XXX
\item \textbf{Formulaic Judgment Criterion}. Instead of arbitrarily define the affinity of stage replications, {\design} evaluate it through formulas based on the roof line model~\cite{roofline_1st}, with inspected information from its fine-grained view (e.g., the algorithm, the data size) as input, and output the concerned objective value in energy, latency and core work load. 
%Since the statistics of the same data set is relative stable, {\design} can also deal with the various data characteristics well by use the exposed attribute of \emph{data set}. 
%Our formulas are described in detail in section xxx
\item \textbf{Grasping the Different Cache Structure}. The {\design} recognize core differences not only by the micro-architecture, but also by the \emph{cluster}-like organizations the core belong to. Therefore, different size and speed of the cache, memory and bus components can be added to our formulas.  
%We achieve the awareness of this by refine formulas in section xxx, with experimental supports in xxx
\end{itemize}
When a compression job is complex and consisted of many stages (e.g., the zlib~\cite{comp_zlib} compression requires both huffman~\cite{comp_huffman} and LZ77~\cite{comp_lzFamily}), the overhead of evaluating all possible execution plans can be rather high, i.e., with the base number of replications and the power exponent determined by number of stages. Therefore, we combine {\design} with a branch and bound (B\&B) based approach to relieve the stress, defining the bounding function as energy estimated by our models and adding the evaluated latency and CPU workload as prune conditions.
\end{comment}


We implemented the {\design} on a customized embedded system, called the {\system}.
 The key design of {\system} are 1)to only include and run the software that are \emph{in need} and 2) to achieve precise and non-invasive energy measurement by special hardware. Therefore, {\system} has a software-hardware co-design which can provide {\design} with necessary support in terms of run-time libraries and power measurement methods, without adding interference or overhead to {\design}.

Based on {\system}, we conduct evaluation on AMP platform rockpi 4a~\cite{amp_rockpi4}, where we use {\design} to schedule several classic PLSC algorithms against five data sets including full-text data, binary stream data and synthetic data in experimental studies comparing with competitors. The results show that {\design} can achieve 20 \% to 40 \%
saving in energy, while always meeting the assigned maximum latency and preventing each core from overloading.

In summary, this paper makes the following contributions:
\begin{itemize}
    \item We give a formulaic definition of the energy-efficient scheduling of PLSC on AMP, with real-time limitations (section \ref{sec:problem}). 
    \item We propose a mechanism called {\design} to better schedule PLSC stages and replicas on AMP, by precisely estimating the energy, latency and core workload of them on AMP (section \ref{sec:models}). 
    \item We implement {\design} on customized embedded system {\system}, which has an anti-interference co-design and provide low-overhead energy measurement (section \ref{sec:implementation}).
    \item We carry out a comprehensive evaluation on the AMP platform, which demonstrates that {\design} outperforms alternative solutions on varying PLSC methods and stream datasets (section \ref{sec:evaluation}).
\end{itemize}

\begin{comment}
The AMPs, featuring different type of cores with different performance and   characteristics (i.e., the so-called \emph{big-cores} and \emph{little-cores}) though sharing the same instruction-set architecture (ISA), are targeted at \emph{trade-off} cases like portable costumer devices and edge devices~\cite{amp_2011,amp_official1} from the first beginning~\cite{amp_2003,amp_2004}. They are represented by ARM’s big.LITTLE core(ABLC) architecture, Intel’s hybrid Lakefield CPU and Apple’s A12-A14 bionic processors, etc., and they can enhance battery life, reduce the cost of cooling and overall improve system’s scalability and reliability in these scenarios specifically.
Due to such advanced nature and wide application~\cite{amp_iot} of AMP, they are extraordinarily capable of performing parallel lossless compression of stream data. Specifically,  Nevertheless, effectively scheduling parallel applications on AMP is another open challenge.
\end{comment}
%weakness of compression
\begin{comment}
Modern lossless data compression has a long history itself (no later than the 1950s~\cite{comp_huffman}), and its parallelsim can also date back to the 1980s~\cite{comp_1985}, but AMP-friendly lossless compression is still too far to be mature. In particular, there
are three key challenges (\textbf{C1} to \textbf{C3}) for efficiently parallelizing lossless compression on AMP.
\textbf{\emph{C1}}: a significant number of compression algorithms have been proposed and can be applied. We classify them into three groups by there weight on execution: light, medium and heavy. They are defined according to the complexity data structures and procedures: heavy weight algorithms like huffman~\cite{comp_survey_huffman} and LZ~\cite{comp_survey_lz} algorithms are often more complicated to achieve higher compression ratio, light-weight algorithms like elias-delta~\cite{comp_elias} perform fast but careless-in-space compression, and medium-weight algorithms like the recently developed lz4(~\cite{comp_lz4}) make the compromise. These three groups form a large space on the top level of algorithm choice. \textbf{\emph{C2}}: the different memory level parallelizing (MLP) and instruction level parallelizing (ILP) between different algorithms or even within the same one. Prior studies~\cite{amp_pie_2011,amp_survey_2016} have shown that the \emph{big cores} and \emph{little cores} on AMP do not have the same affinities of MLP and ILP although under the same ISA. Without a proper coupling to work load in terms of them on AMP, both energy dissipation and performance lost will happen. \textbf{\emph{C3}}: various performance metrics in real world. IoT means \emph{everything to be involved}, so there are different focuses on throughput, latency and energy cost, etc., and sometimes they can conflict
with each other. As two regulation methods have been practiced on AMP for other applications (e.g., virtual machine~\cite{amp_vm_yinyang}, artificial intelligence runtime~\cite{amp_ai} and game governer~\cite{amp_game}): the task remapping ~\cite{amp_2004} and dynamic voltage and frequency scaling (DVFS) ~\cite{amp_DVFS1}), it's worth to think about how they act in fitting the performance preferences in compression.
 
 To the best of our knowledge, this work presents the first
comprehensive experimental study on the effectiveness of parallel lossless compression
algorithms on AMP. To this end, we developed an unified benchmark framework by reimplementing five algorithms covering three kinds of weight under the same language and compiler to address \textbf{\emph{C1}}. We have a fine-grained deconstruction of these algorithms and parallelizing them in a hybrid way to address \textbf{\emph{C2}}. For \textbf{\emph{C3}}, we studied different mapping strategies and DVFS settings of AMP in dealing with the parallelized compression workload, and finally extend the price theory~\cite{amp_DVFS3} on AMP with more parallel-compression-aware policies of \emph{pricing} and \emph{marketing}.

The contributions of this paper are that we put forward and find answers to following questions:
\begin{itemize}
    \item [Q1] What do different lossless compression algorithms performs on AMP?
    \item [Q2] How to do an AMP-aware parallelism of them (i.e., drill and fit the MLP and ILP)?
    \item [Q3] How to regulate the performance metric of lossless compression further on AMP for better matching to the needs?
\end{itemize}
Moreover, our approaches which both zoom in and zoom out the algorithms together the hardware will inspire subsequent studies on other new hardware like FPGA and GPU.
\end{comment}

%remainder
\begin{comment}
\textbf{Organization.} 
 The remainder of this paper is organized as follows. 
 Section~\ref{sec:background} covers the necessary background of modern AMP and an overview of PLSC. 
 Section~\ref{sec:problem} give the problem formulation of this, followed by a detailed model design in Section~\ref{sec:models}.
 Section~\ref{sec:implementation} {discusses how we deploy {\design} and the measurement tools on concrete AMP platform.} 
 %that are optimized for shared-memory multicores. 
 We report extensive experimental results in Section~\ref{sec:evaluation}. 
 Section~\ref{sec:related} reviews related work and Section~\ref{sec:conclusion} concludes this work.
\end{comment}


==> Sections/backup/special_reserve.tex <==
If the individually mapped stages were also executed in parallel, we would have a speed-up pipeline along with more \emph{fine-grained} exposure of task-core affinity.


There is an insightful idea to further divide each stage and form a deeper pipeline, which can theoretically increase the speed-up further. However, this is not suitable for the compression algorithms that are \emph{simple} or \emph{light-weight} themselves, as extra communication overhead between \emph{too many} stages can even eliminate the acceleration and increase energy dissipation.

\begin{comment}
\begin{algorithm}[t]
\caption{The decision-making procedure of \design for the optimal scheduling plan}
\label{alg:scheduler}
\LinesNumbered 
\KwIn{ Array of all possible {scheduling plans } $[p_{0}, p_{1}, ..., p_{n-1}]$}
\KwIn{latency constraint $L_{set}$}
\KwOut{The optimal {scheduling plan} $p_{opt}$ }
$p_{opt}$ $\leftarrow$ $p_{0}$ \;
$E_{min} \leftarrow infinity$ \;
\ForEach {{scheduling plan} $p_{enum}$ enumerated from $[p_{0},p_{1},...,p_{n-1}]$ by dynamic programming\label{algo:dp0} } 
{
$L$ $\leftarrow$ estimated $L$ of $p_{enum}$ \label{algo:estiL} \;
\If{$L <L_{set}$ \label{algo:compareL}}
{
  $E_{temp}$ $\leftarrow$ estimated $E$ of $p_{enum}$ \label{algo:estiE}\;
  \If{$E_{temp} < E_{min}$ \label{algo:compareE}}
  {
     $p_{opt}$ $\leftarrow$ $p_{enum}$ \label{algo:oPlan0}\;
    $E_{min}$ $\leftarrow$ $E_{temp}$ \label{algo:oPlan1}\;
  }
}

}
\end{algorithm}

% \shuhao{Add the discussion of how to handle ``subsequent inputs''.}
With the asymmetry-aware cost model integrated and calibrated, \design determines the optimal scheduling plan by Algorithm~\ref{alg:scheduler}. As the formation of {task} leads to a large space of \emph{scheduling plans}, we adopt dynamic programming~\cite{algo_dp_1954} to reduce the complexity of enumeration (Line~\ref{algo:dp0}). 
For each \emph{scheduling plan} enumerated, the scheduler first predicts its $L$ by the cost model (Line~\ref{algo:estiL}) and compares it with the $L_{set}$ (Line~\ref{algo:compareL}). If not exceeded, the corresponding $E$  (Line~\ref{algo:estiE}) will also be estimated and compared with the current least predicted energy (Line~\ref{algo:compareE}); otherwise, we simply discard this \emph{scheduling plan}. 
After the dynamic programming is done, we can find \emph{the optimal scheduling plan} with both $L<L_{set}$ and the least $E$, according to Lines~\ref{algo:oPlan0} and~\ref{algo:oPlan1}.  
\end{comment}



The {$\eta_{i}$} can be defined and posteriorly calculated in Equation~\ref{eqn:def_eta} by literally using total instructions ($\iota_{i}$) and $l_{i}$. 
\begin{align}
\scriptsize
 \eta_{i} &=\frac{\iota_{i}}{l_{i}} \label{eqn:def_eta}
\end{align}
Similar to $\eta_{i}$, $\zeta_{i}$ follows the definition and posterior calculation in Equation~\ref{eqn:def_zeta}, but replace $e_i$ with $l_i$.
\begin{align}
\scriptsize
  \zeta_{i}&= \frac{\iota_{i}}{e_{i}}  \label{eqn:def_zeta}
\end{align}




First, if {$\kappa_{i}$} is low and does not put significant pressure on L1D (i.e., within the first boundary $\kappa_{L1}$), 
$\eta_{i}$ will just grow along with growth rate {$k_{L1}$}. Then, increasing {$\kappa_{i}$} will put 
different pressures on both L1D and L2, and leads to varying growth rate ($k_{L2}$ or or $k_{Exceed L2}$ ) and intercept ($k_{Exceed L2}$ or $b_{Exceed L2}$).
For instance, the $\kappa_{i}>\kappa_{L2}$ condition means that the L2 missing is frequent and have significant impacts. Therefore, $\eta_{i}$ is determined by $\kappa_{i}$ with 
$k_{Exceed L2}$ and $b_{Exceed L2}$ then.
Finally, there is a third boundary $\kappa_{roof}$ of $\kappa_{i}$, and $\eta_{i}$ will not grow after $\kappa_{i}>\kappa_{roof}$. Instead, it ``reaches the roof of $\eta_{max}$'' and remains unchanged.
%\begin{align}
%C &=\eta_{i}^{max} \label{eqn:cj} 
%\end{align}

It's worth noting that the concrete position of the segments (i.e., $\kappa_{L1}$, $\kappa_{L2}$ and $\kappa_{roof}$), the growth rate (i.e., $k_{L1}$, $k_{L2}$, and $k_{Exceed L2}$) and the intercept (i.e., $b_{L2}$ and $b_{Exceed L2}$) can differ for {$\eta_{i}$} and {$\zeta_{i}$}, as the pipeline structure (OoO or In-Order) of core has different response to the cache size in performance and energy. Besides, the growth rate ($k_{L2}$, and $k_{Exceed L2}$) may be negative as corresponding cache miss can \emph{slow down} the core or \emph{reduce} its energy efficiency.


==> figures/Tips.tex <==
%% This file just some irrelevant tips for figure and table 
%% This needs to delete at last



 
\autoref{fig:duck}.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/duck}
  \caption{}
  \label{fig:duck}
\end{figure}

\begin{table*}[t]
  \caption{A double column table.}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    A Wide Command Column & A Random Number & Comments\\
    \midrule
    \verb|\tabular| & 100& The content of a table \\
    \verb|\table|  & 300 & For floating tables within a single column\\
    \verb|\table*| & 400 & For wider floating tables that span two columns\\
    \bottomrule
  \end{tabular}
\end{table*}

\subsection{Tables}

  \autoref{tab:commands}.

  \autoref{tab:freq}. 

\begin{table}[hb]% h asks to places the floating element [h]ere.
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math & Frequency & Comments\\
    \midrule
    \O & 1 in 1000& For Swedish names\\
    $\pi$ & 1 in 5 & Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40\,000 & Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}
 

 
